Decentralized Stream Runtime Verification for Timed Asynchronous Networks

We study the problem of monitoring distributed systems where computers communicate using message passing and share an almost synchronized clock. This is a realistic scenario for networks where the speed of the monitoring is sufficiently slow (at the human scale) to permit efficient clock synchronization, where the clock deviations is small compared to the monitoring cycles. This is the case when monitoring human systems in wide area networks, the Internet or including large deployments. More concretely, we study how to monitor decentralized systems where monitors are expressed as stream runtime verification specifications, under a timed asynchronous network. Our monitors communicate using the network, where messages can take arbitrarily long but cannot be duplicated or lost. This communication setting is common in many cyber-physical systems like smart buildings and ambient living. Previous approaches to decentralized monitoring were limited to synchronous networks, which are not easily implemented in practice because of network failures. Even when networks failures are unusual, they can require several monitoring cycles to be repaired. In this work we propose a solution to the timed asynchronous monitoring problem and show that this problem generalizes the synchronous case. We study the specifications and conditions on the network behavior that allow the monitoring to take place with bounded resources, independently of the trace length. Finally, we report the results of an empirical evaluation of an implementation and verify the theoretical results in terms of effectiveness and efficiency.

==> eff-deceff.tex <==
\section{Efficiently vs Decentralized Efficiently Monitorability}
\label{sec:app:eff-vs-deceff}

Not every efficiently monitorable specification can be evaluated 
with finite memory in the length of the trace.
%
We show now a counter-example of a efficient monitorable specification
that illustrates that Algorithm~\ref{alg:local-algo} does not run in
bounded memory.
%
This specification is efficiently monitorable but not decentralized
efficiently monitorable.  


Consider the following efficiently monitorable specification deployed
in monitors 1 and 2 with $dist(1,2) = dist(2,1) = 2$:
{\small\begin{lstlisting}[language=LOLA] 
    @1{output num a eval = b[-1|0]} 
    @2{output num b eval = a[-1|0]}
\end{lstlisting}}
%
It is easy to observe that $a[0]$ and $b[0]$ will be resolved at $t =
0$.  Then, $a[1]$ and $b[1]$ will be resolved at $t = 2$ $a[2]$ and
$b[2]$ will be resolved at $t = 4$ $a[3]$ and $b[3]$ will be resolved
at $t = 6$ so $a[n]$ and $b[n]$ will be resolved at $t = 2n$ which is
not a constant but depends on the time of instantiation and thus it is
unbounded.

% Therefore we can elaborate a claim upon which the decentralized
% algorithm is actually Bounded Memory.
% \begin{theorem}
%   If the Network Deployment Graph is a DAG and the Dependency Graph of
%   the specification is Efficiently Monitorable, then the decentralized
%   algorithm is Bounded Memory.
% \end{theorem}
% In order to prove this we need to prove that every element in U (pair instanced stream, expression) gets resolved $\tUresolved$ in a constant amount of time.
% In order to do that we need a definition
% \begin{definition}
%   Given a specification and its $\delta$ which maps the streams to monitors, then we define $\nabla$ as the time at which a stream gets resolved. $\nabla$ tell us the time needed from a stream is instanced until it is resolved, effectively, the time the pair $(s[t],e) \in U$.
%   Formally, $\nabla(s) = max(0, max(max(0,w_{s,d} + \nabla(d) + dist(\delta(d), \delta(s)))))$ for all $d \in dependencies(s)$.
%   It is always non-negative and is defined by the sum of the future dependencies' shifts plus the nabla of those dependencies plus the distance between the monitors that compute the stream and its dependency.
% \end{definition}
% \begin{proof}
%   .
%   \qed
% \end{proof}
% %END already in efficient

\begin{example}
  \label{ex:decent-efficient}
  In this experiment (see Fig.~\ref{plot:constant-mem}) we can observe
  the bounded memory usage of the specifications independent of the
  trace length, as described in Section \ref{sec:efficient}.
  %
  What we can observe is the average among the maximum memory used for
  the combination of communication strategy (eager, lazy) and mapping
  of stream variables to nodes (centralized, decentralized).
\begin{figure}[tbh!]
  \label{plot:constant-mem}
  \centering
  \includegraphics{plots/constant_memory-crop} 
  \caption{Memory usage}
\end{figure}
\end{example}

\clearpage


==> efficient.tex <==
\section{Decentralized Efficient Monitorability}
\label{sec:efficient}
\luismitext{Add plots of network behavior in old Journal dir}
\summary{recall decentralized efficiently monitorable}
The aim of this section is to define when the local
monitors only need bounded memory to compute every output value.
%
The first thing to consider is that the specification must be 
\emph{decentralized efficiently monitorable}~\cite{danielsson19decentralized},
as we described in section~\ref{subsec:decent-eff-monitorable}.
%
%For the sake of simplicity in the explanation, we focus first on the eager communication strategy and then we explain the lazy case.
%
So, %in the case of the \emph{eager} communication strategy,
in order to
guarantee that a given storage in a local monitor for node $n$ is
bounded, one must provide an upper-bound to bound how long it takes to
resolve an instant variable for a stream that is assigned to $n$.

\subsection{General Equations for the Time to Resolve}
%
We introduce now general recursive equations that capture when an
instant variable $\InstVar{s}{k}$ is resolved.
%
In order to bound the memory, we need to bound storages $U_n$ and
$R_n$:
%, since all the other storages depend on the them:
%
\begin{itemize}
\item \textbf{Bound on $R_n$}: %Under the eager strategy
  Resolved
  values that are needed remotely are sent immediately to the remote
  nodes, so $R_n$ only contains resolved values that are needed in the
  future locally at $n$.
%
  Since decentralized efficiently monitorable specifications only
  contain (future) bounded paths (say with maximum future reference
  $b$), this upper-bound limits for how long a resolved value can
  remain in $R_n$, because after at most $b$ instants the instant
  variable that needs the value stored in $R_n$ will be instantiated.
%
  At that point, the value can be used and be immediately removed from
  $R_n$.
%
  This guarantees that $R_n$ is always upped-bounded by a constant in
  every node.
\item \textbf{Bound on $U_n$}: The size of the memory required for
  storage $U_n$ at the node $n$ responsible to resolve $s$ (that is
  $n=\mu(s)$) is proportional to the number of instantiated but
  unresolved variables.
%
  Therefore, to bound $U_n$ we need to compute the bound on the time
  it takes to resolve instant variables assigned of streams assigned
  to $n$.
\end{itemize}

These general equations that we present below depend on the duration
of messages.
%
We will later instantiate these general equations for the following
cases:
%
\begin{inparaenum}[(1)]
\item synchronous network;
\item timed-asynchronous network with an upper-bound on message
  delays for the whole trace: \globalTime; and
\item timed-asynchronous network with an upper-bound for message
  delays in a given time-horizon: \localTime.
\end{inparaenum}
%
Note that the correctness of the algorithm establishes that the output
streams $\sigma_o$ only depend on the input streams $\sigma_i$ and not
on the time at which each element of $\sigma_o$ is resolved or on the
delays of messages.
%
What we establish in this section is that the delay of messages
affects the time at which instant variables are resolved, which
affects the memory usage at the computations nodes.
%
\cesartext{Introduce $\ArrivalTime{s}{r}$ before.}
%

Recall that we assume that messages are causal and queues are FIFO as
we described in~\ref{subsec:time-async-model}.
%
Causality means that messages arrive after they are sent (that is, for
every $n$, $m$ and $t$, $\ArrivalTime{a}{b}(t) > t$) and FIFO that for
every $n$ and $m$, if $t<t'$ then
$\ArrivalTime{a}{b}(t) \leq \ArrivalTime{a}{b}(t')$.
%
We use $\TAmsgTrip(t,a,b)$ for the time it takes for a message sent
from $a$ to $b$ at time $t$ to arrive.
%
Note that $\ArrivalTime{r}{s}(t)= t + \TAmsgTrip(t,r,s)$.

We now capture the\emph{moment to Resolve} for a given instant
variable $\InstVar{s}{t}$, represented as $\MTR(\InstVar{s}{t})$,
which captures the instant of time at which $\InstVar{s}{t}$ is
guaranteed to be resolved.
%
Our definition considers two components, the delay in resolving all
local instant variables that $\InstVar{s}{t}$ may depend on, and the
remote variables that also involve message delays.
%
We use the concept of \emph{remote moment to resolve}, denoted
$\MTRrem(\InstVar{s}{t})$, as the instant at which all remote values
that $\InstVar{s}{t}$ require have arrived (or $t$ if all values
arrive before $t$).
%
\begin{align*}
& \MTR(\InstVar{s}{t}) \DefinedAs \\
& \max(\MTRrem(\InstVar{s}{t}),\{\MTR(\InstVar{r}{t+w})\;|\; \depWeightSub{s}{w}{loc}{r}\}) \\  
& \MTRrem(\InstVar{s}{t}) \DefinedAs \\
& \max(t,\{ \ArrivalTime{r}{s}(\MTR(\InstVar{r}{t+w})) \;|\;\depWeightSub{s}{w}{rem}{r} \text{ and } t+w \geq 0 \}) \\
\end{align*}
%

Note that for $\MTRrem(\InstVar{s}{t})$ only consider the those remote
instant variables for which $t+w\geq{}0$ because otherwise the
default value will be used at the moment of instantiating
$\InstVar{s}{t}$.
%
In the equation for $\MTR(\InstVar{s}{t})$ we assume the base case
$\MTR(\InstVar{s}{t})=0$ when $t<0$, because again, the default value
in the offset expression is used instead, which is known immediately.
%
It is easy to see that the first equation is equivalent to:
%
\[  \MTR(\InstVar{s}{t}) \DefinedAs 
    \max(\{\MTRrem(\InstVar{r}{t+w})\;|\; \depWeightSubStar{s}{w}{loc}{r}\}) 
\]
%
We are now ready to prove that these definitions indeed capture the time at
which $\InstVar{s}{t}$ is resolved.

%
\begin{theorem}
  Let $\Spec$ be a specification and $\mu$ a network
  placement, let $\sigma_i$ be the input trace and $\Arr$
  a network behavior.
  % 
  Then every $\InstVar{s}{t}$ is resolved at 
  $\MTR(\InstVar{s}{t})$ or before.
\end{theorem}

\begin{proof}
  The proof proceeds by induction on the evaluation graph $\EvGraph$
  induced by $\Spec$ and the length of $\sigma_i$.
  %
  \begin{itemize}
  \item Base case: inputs and other instant variables $\InstVar{s}{t}$
    that do not depend on any other instant variables.
    % 
    These are the nodes of $\EvGraph$ that do not have any outgoing
    edge.
    %
    Since $\InstVar{s}{t}$ is instantiated (and read or computed) at
    $t$, then the value is resolved exactly at $t$.
    %
    Also, $\MTR(\InstVar{s}{t})=\MTRrem(\InstVar{s}{t})=t$.
  %
  \item General case. Let $\InstVar{s}{t}$ be an arbitrary instant
    variable and assume, by inductive hypothesis, that the theorem
    holds for all instant variables lower in the $\EvGraph$.
    %
    At time $\MTRrem(\InstVar{s}{t})$ all instant variables
    $\InstVar{r}{t+w}$ from remote nodes that $\InstVar{s}{t}$ depends
    on have arrived because $\InstVar{r}{t+w}$ will be resolved at
    $\MTR(\InstVar{r}{t})$ by induction hypothesis.
    %
    Similarly, all local elements that $\InstVar{s}{t}$ depends on are
    also below in the dependency graph, so the induction hypothesis
    also applies.
    %
    Therefore, at time
    %
    \[ \max(\MTRrem(\InstVar{s}{t}),\{\MTR(\InstVar{r}{t+w})\;|\;\depWeightSub{s}{w}{loc}{r}\}\} \]
    %
    or before all elements that $\InstVar{s}{t}$ depends on will be
    known and $\InstVar{s}{t}$ will be resolved.
    %
\end{itemize}
\end{proof}

The following corollary follows from the fact that nothing that
happens after an instant variable has been resolved (either further
values in $\sigma_i$ or the network behavior) can affect the value
computed.
%
Therefore, the value and time at which $\InstVar{s}{t}$ is computed
does not depend on the future after $\MTR(\InstVar{s}{t})$.

\begin{corollary}
  For all $\InstVar{s}{t}$ there is a $t'$ such that $\InstVar{s}{t}$
  only depends on $\sigma_i$ and $\Arr$ up to $t'$.
\end{corollary}
%
\subsection{Examples}
%For Timed Asynchronous
Unrolling example, plots: arrows of when instant streams are resolved and the prediction of the eqs,...
\begin{example}
  {\footnotesize\begin{lstlisting}[language=LOLA]
    @1{input int a}
    @2{define int b = a[-1|0]
      output int c = b + a}
  \end{lstlisting}}
  We can obtain the $MTR(\InstVar{c}{1})$ as follows:
  \begin{align*}
    &MTR(\InstVar{c}{1}) = \max(\MTRrem(\InstVar{c}{1}),\MTR(\InstVar{b}{1})) = \\
    %remotes
    &= \max(\max(1,\ArrivalTime{a}{c}(\MTR(\InstVar{a}{1}))),\max(\MTRrem(\InstVar{b}{1}))) = \\
    &= \max(\max(1,\ArrivalTime{a}{c}(\MTRrem(\InstVar{a}{1}))),\\
    &       \max(\ArrivalTime{a}{b}(\MTR(\InstVar{a}{1-1})))) = \\
    &= \max(\max(1,\ArrivalTime{a}{c}(1)),\ArrivalTime{a}{b}(\MTRrem(\InstVar{a}{0}))) = \\
    &= \max(\max(1,\ArrivalTime{a}{c}(1)),\ArrivalTime{a}{b}(0)) = \\
    &= \max(\ArrivalTime{a}{c}(1),\ArrivalTime{a}{b}(0)) = \\
  \end{align*}
\end{example}

%do not include if we use \AlgorithmTADLola
%\AlgorithmProceduresLazy

\begin{example}
  \label{ex:msgs2}
  In this example we describe the message passing of Request messages
  (in red) and Response messages (in green) in
  Fig.~\ref{fig:msgs-needed}.
  %
  The need of an instanced stream value arises from its presence in
  the right side of an expression in U.
  %
  Therefore a needed value is one such that it is needed to simplify
  that expression, whereas one that is not needed does not appear in
  any expression in U.
  %
  Eager streams always send the Response message to those monitors that
  compute streams that may need their values.
  %
  Lazy streams need to be requested in order to be sent, this way only
  when it is actually needed a Request and matching Response will
  traverse the network.
  %
\qed
%
\begin{figure}[t]
%  \begin{tabular}{cc}
    \includegraphics[scale=0.8]{RE_eval} \\
    \text{(a) Eager, all streams are needed} \\
    \includegraphics[scale=0.8]{RE_lazy_needed} \\
    \text{(b) Lazy, all streams are needed} \\
    \includegraphics[scale=0.8]{RE_eval} \\
    \text{(c) Eager, rarely the streams are needed} \\
    \includegraphics[scale=0.8]{RE_lazy_notneeded} \\
    \text{(d) Lazy, rarely the streams are needed} \\
 % \end{tabular}
  \caption{Messages needed (lazy vs eager)}
  \label{fig:msgs-needed}
\end{figure}
%
\end{example}
%

\subsection{Instantiation to Synchronous}

\luismitext{Synch: calculation of TimeToResolve == Look-ahead}
\luismitext{In centralized synch(LOLA) the concept of TimeToResolve collides to Latency which is based on the offsets in the Depgraph}

The synchronous model of computation is a particular case of the
timed-asynchronous model where all message delays between two monitors
take exactly the same amount of time, a constant that is known a
priori.
%
The $\DIST(r,s)$ is used to represent the delay that every message
will take from $\mu(r)$ to $\mu(s)$, independently of the time instant
at which the message is sent.
%
We use this knowledge to simplify $\MTRrem$ for synchronous networks as follows
%
\begin{align*}
  &\MTRsynrem(\InstVar{s}{t}) \DefinedAs \max(t, \\
  &\{ \MTRsyn(\InstVar{r}{t+w}) + \DIST(r,s) \;|\;\depWeightSub{s}{w}{rem}{r}, t+w \geq 0 \})
\end{align*}
%

Recall that the \emph{time to resolve} is the time interval between
the moment at which a variable is instantiated and the instant at
which it is resolved (that is
$\TTR(\InstVar{s}{t}) = \MTR(\InstVar{s}{t}) - t)$
%
In the synchronous case we obtain:
\begin{align*}
  & \TTRsyn(\InstVar{s}{t}) = \MTRsyn(\InstVar{s}{t}) - t = \\
  &= \{\MTRsynrem(\InstVar{r}{t+w}) \;|\; \depWeightSub{s}{w}{loc}{r}\} -t = \\
  &= \max(t, \{ \MTRsyn(\InstVar{r}{t+w}) + \DIST(r,s) \;|\; \depWeightSub{s}{w}{rem}{r} \}) - t =\\
  &= \max(0,\{\TTRsyn(\InstVar{r}{t+w}) + \DIST(r,s) \;|\; \depWeightSub{s}{w}{rem}{r}\})
\end{align*}
%
Note that the value that determines the result is the
$\TTRsyn(\InstVar{s}{t})$ of the slowest remote dependency (including
resolve time and traverse through the network).
%
Additionally, we can easily show by induction in the dependency graph
that for every stream variable $s$ there is a constant $k$ such that
$\TTRsyn(\InstVar{s}{t})\leq k$, that is, $s$ always takes less than
$k$ instants to be resolved.
%
This is equivalent to the result obtained
in~\cite{danielsson19decentralized}.
%
It follows that decentralized efficiently monitorable specifications
can be monitored in constant space, that is, they are trace length
independent.

\subsection{Timed Asynchronous with \Toadv{\GlobalTime} Bounded delays}
%
An execution of timed-asynchronous monitors has \toadv{\globalTime} bounded
delays if there is an upper bound on the arrival time of every message.
%
\cesartext{Show an example of network behavior that is not globally
  bounded}
%
Formally, if there is a $d$ such that for every streams $r,s$ and for
every time $t$, $\ArrivalTime{r}{s}(t)\leq t+d$.
%
Substituting the upper-bound value $d$ in the equations for $\MTR$, we
obtain an constant upper-bound on the $\MTR$ (although this value can
be a gross over-approximation):
%
\begin{align*}
  &\MTRgrem (\InstVar{s}{t}) \leq \max(t,\{\\
  &\hspace{4em} \MTRg(\InstVar{r}{t+w}) + d \;|\;\depWeightSub{s}{w}{rem}{r}, t+w \geq 0 \})
\end{align*}
%
Note that this implies that $\InstVar{s}{t}$ can be resolved before
$\MTRg(\InstVar{s}{t})$ because we use a pessimistic upper bound.
%
In this case we can also bound the memory necessary to store in every
node to perform the monitoring process, but most of the time this
memory will not be necessary.
%
We can see an example of a \globalTime bound in figure~\ref{plot:peakTTR}.
%
\subsection{Timed Asynchronous with \Toadv{\LocalTime} Bounded delays}
%
We now take a closer look at the equations to obtain a better bound on
the time to resolve a given instant variable $\InstVar{s}{t}$, without
depending on an upper-bound of all messages in the history of the
computation.
%
The main idea to bound $\MTR(\InstVar{s}{t})$ is to consider the time
interval at which the messages that are relevant to compute
$\InstVar{s}{t}$ are sent.
%
We first define an auxiliary notion.
%
We say that a stream variable $r$ is a direct remote influence on $s$
with delay $w$, and we write $\wdirrem{s}{w}{r}$, whenever there is a
path
$\wloc{s}{w_1}{s_1}\wlocnext{w_2}{s_2}\ldots\wlocnext{w_k}{s_k}\wremnext{w_{k+1}}r$
such that:
\begin{compactitem}
\item no two nodes $s_i$ and $s_j$ are repeated (if $i\neq j$ then $s_i\neq s_j$), and
\item $w=w_1+\ldots+w_k+w_{k+1}$.
\end{compactitem}
%
Note that $\wdirrem{s}{w}{r}$ means that $\InstVar{s}{t}$ may be
influenced by remote variable $\InstVar{r}{t+w}$.
%
We define the window of interest for $\InstVar{s}{t}$ as:
\begin{align*}
  &\Win(\InstVar{s}{t}) = [\min S, \max S] \text{ where $S$ is defined as } \\
  &S  =  \{t, \MTRrem(\InstVar{r}{t+w}) \;|\; \wdirrem{s}{w}{r} \text{ and } t+w>0\}
\end{align*}
%
Note that $S$ is the set of instants at which remote instant variables
that influence $\InstVar{s}{t}$ are sent.
%
Therefore $\Win(\InstVar{s}{t})$ contains those instants at which the
remote information relevant to $\InstVar{s}{t}$ is sent.
%
We then define the worst message sent to $s$ for the computation of
$\InstVar{s}{t}$ as:
\begin{align*}
  &\dworst(\InstVar{s}{t})=\max\{t'-t\;| \\
  &\;t'=\ArrivalTime{r}{s}(t) \text{ for }  \wdirrem{s}{w}{r} \text{ and  } t\in \Win(\InstVar{s}{t}) \}.
\end{align*}
%
Note that $\dworst$ is still an over-approximation of the messages
sent in order to compute $\InstVar{s}{t}$ but it considers all those
messages and only looks at a bounded interval or time.
%
Since all the values that influence $\InstVar{s}{t}$ are sent within
$\Win(\InstVar{s}{t})$ we can bound $\MTR(\InstVar{s}{t})$ as follows:

\begin{align*}
  &\MTR(\InstVar{s}{t}) \leq \max(t,\\
  &\{\MTR(\InstVar{r}{t+w})+\dworst(\Win(\InstVar{s}{t}))\;|\;\wdirrem{s}{w}{r} \}).
\end{align*}
%
\cesartext{HERE}

%
The window ends at $\MTR(\InstVar{s}{t})$.
%
From window and bound to MTR:\\
%
Now with this window we obtain a $\WorstRoundTripWin{s}{r}{w_s}{w_e}$ inside that window and we can use it to substitute in the eqs:
%
\begin{align*}
  &\MTRrem(\InstVar{s}{t}) \DefinedAs \max(t, \\
  &\{ \MTR(\InstVar{r}{t+w}) + \WorstRoundTripWin{s}{r}{w_s}{w_e} \;|\;\depWeightSub{s}{w}{rem}{r}, t+w \geq 0 \})
\end{align*}
%
Plots showing peaks and how the MTR or TTR adapts to those peaks depending if the window includes the peak it results
in the worst MTR (same as global) or the good one if the window does not include the peak.
%
{\small\begin{figure}[tbh!]
  \centering
  \includegraphics[scale=0.7]{plots/ttr_4_peak_try-crop} 
  \caption{TTR, \globalTime and \localTime bounds for a peak delay}
  \label{plot:peakTTR}
\end{figure}}

\subsection{Pruning the Resolved Storage.}
\summary{see RV19 part where we talk about pruning and comment pruning algo~\ref{alg:prune}}
We are finally ready to prune $R_n$ because we know now when every instant variable will be resolved.
\luismitext{DANGER!!!: as we are considering eager only this whole discussion about how to prune is pointless(this whole section!!!) since with just a fire-n-forget strategy it works}
%
\begin{lemma}
  \label{lem:mtr}
  Every unresolved instant variable $\InstVar{s}{t}$ in $U_n$ is resolved at most at
  $t+\MTR(\InstVar{s}{t})$.
\end{lemma}
%
So, as soon as this moment is reached, %in the eager communication strategy,
its value will be sent to those monitors where it is needed.
%
So it can be pruned from the memory.
%
With this mechanism, we can assure that every instant variable will be in memory ($U_n, R_n$) for a bounded amount of time.
%
\noindent Lemma~\ref{lem:mtr} implies that
decentralized efficiently monitorable specifications in timed asynchronous networks can be monitored
with bounded resources.
%
The bound depends only linearly on the size of the specification,
the diameter of the network and the delays among the nodes of the network.

%\luismitext{previous to 16/02/21 below}
%\begin{definition}[d-w-window]
%  $d$-window of size $w$ means that in a window starting at $k$ endin at $k+w$
%  all msgs sent within the window arrive in $d$ instants or less (but not 0)
%   (even if they arrive outside the window) 
%   example w=4, d=2: starts at 0, ends at 3, all msgs take 1 or 2 instants to arrive, msg0 arrives at 2, msg1 at 3, msg2 at 4, msg3 at 5 , 
%   but we know nothing about msg4 or msg5...
%\end{definition}
%%
%\luismitext{ideas: 1 FIFO+positive windows="if $\InstVar{s}{t}$ can be resolved then $\InstVar{s}{t-1}$
%  can be resolved", negative(past) windows or windows that have a part in the past and part in the future}
%\begin{theorem}[Local(in time)]
%  Forall $t$ there exists a $d$-$w$-window starting at $t$ s.t. forall msgs $m$ sent between $t+w$,  $delay(m) \leq d$.
%\end{theorem}
%%
%Is there always a d-w-window? or A,k window? YES assuming Global it's trivial and assuming local it's also yes
%Calculate a sufficiently good A, k by feeding one to the equations and obtaining the other

%\subsection{The synchronous case RV19}
%In this section we identify a fragment of specifications, called
%\emph{decentralized efficiently monitorable}, for which the local
%monitors only need bounded memory to compute every output value.
%%
%To guarantee that a given storage in a local monitor for node $n$ is
%bounded, one must provide a bound on both:
%%
%\begin{inparaenum}[(1)]
%\item when a value $(u[k],c)$ in $R_n$ can be removed; and
%\item when it is guaranteed that an unresolved value from $U_n$ is
%  resolved.
%\end{inparaenum}
%%
%Note that if $s[k]$ is resolved in bounded time then all occurrences
%of $s[k]$ in $\WAIT_n$ and $\PEN_n$ are also removed in bounded time, because
%it only takes a bounded amount of time for response messages to
%arrive.
%%
%%\subsection{Pruning the Resolved Storage}
%%\label{subsec:pruning}
%\subsubsection{Pruning the Resolved Storage.}
%%
%We show now that the memory necessary in the resolve storage $R_n$ can
%be bounded (for all specifications).
%%
%If a stream $s$ is $\ISEAGER(s)$ then once $s[k]$ is resolved it is sent
%to the potentially interested remote nodes.
%%
%However, the value of $s[k]$ has to remain in $R_n$ (and in $R_m$ for
%remote nodes that receive it) until it is no longer needed.
%%
%For streams $s$ that are $\ISLAZY(s)$, the value must remain in $R_n$
%until it is guaranteed that the value will not be requested any more.
%%
%This information is captured by the notion of back reference.
%\begin{definition}
%  \label{def:back-ref}
%  Let $\varphi$ be a Lola specification with dependency graph
%  $D_\varphi$.  
%%
%  The back reference of a stream $s$ is 
%  \[
%  \Delta(s)\DefinedAs \begin{cases}
%    \max(0, \{ -k \hspace{4.885em}\;|\; r \xrightarrow{k} s\}) & \text{if \ISEAGER(s)} \\
%      \max(0, \{ -k + \DIST(r,s) \;|\; r \xrightarrow{k} s\}) & \text{if \ISLAZY(s)}
%      \end{cases}
%      \]
%\end{definition}
%
%Note that for lazy streams the request is guaranteed to be received
%after $\DIST(\mu(r),\mu(s))$ steps of the instantiation of the
%correspondent instance of $r$.
%%
%Therefore, a node responsible for $s$ will have received all requests
%for $u[k]$ at $k+\Delta(u)$.
%%
%Similarly, a fetch for $u[k]$ in $R_n$ locally at $n$ is guaranteed to
%be done no later than $k+\Delta(u)$.
%%
%Therefore, the following results holds.
%%
%\begin{lemma}
%  A value $(u[k],c)\in R_n$ will not be fetched or requested after
%  $k+\Delta(u)$.
%  \label{lem:backref}
%\end{lemma}
%%
%This implies that at every node $n$, all values of $u[k]$ can be
%removed at instant $k+\Delta(s)$, which allows to implement the
%algorithm for pruning shown in Algorithm~\ref{alg:prune}.
%%
%Therefore, the maximum size of $R_n$ needed is bounded linearly by the
%maximum $\Delta(s)$ times the number of streams.
%
%\AlgorithmPrune
%
%%\subsection{Time to resolve}
%%\label{subsec:time-resolve}
%\subsubsection{Time to resolve.}
%%
%In centralized SRV monitoring~\cite{dangelo05lola,sanchez18online} a
%specification is efficiently monitorable whenever all cycles in
%$D_\varphi$ have negative weight.
%%
%This guarantees that the online algorithm can be performed in a \emph{trace
%  length independent} way.
%%
%However, this is not true for decentralized monitoring as illustrated
%in the following example.
%%
%\begin{example}
%  \label{ex:cycles-bad}
%  Consider the following specification deployed in monitors 1 and 2
%  with $dist(1,2) = dist(2,1) = 2$:
%  {\small\begin{lstlisting}[language=LOLA] 
%      @1{output num a eval = b[-1|0]} 
%      @2{output num b eval = a[-1|0]}
%  \end{lstlisting}}
%\noindent 
%It is easy to see that $a[0]$ and $b[0]$ will be resolved at time $0$,
%$a[1]$ and $b[1]$ at time $2$, and $a[n]$ and $b[n]$ at time $2n$.
%%
%Then, $U_1$ and $U_2$ will grow to contain a number of equations that
%depends on the length the trace.
%\end{example}
%%
%We introduce the notion of \emph{decentralized efficiently
%  monitorable}, that guarantees an upper bound on the number of steps
%that it takes to resolve an equation in $U_n$.
%%
%Note that Algorithm~\ref{alg:local-algo-eager} removes an equation from
%$U_n$ and moves it into $R_n$ once it is resolved.
%%
%In turn, this also gives a bound on the duration of the elements in
%$P_n$ and $W_n$.
%%
%It follows that for decentralized efficiently monitorable
%specifications, the monitoring process requires only a constant amount
%of memory (on the size of the specification) independently of the
%length of the trace.
%
%\begin{definition}[Decentralized Efficiently monitoriable]
%  A specification $\varphi$ is decentralized efficiently monitoriable
%  whenever it is efficiently monitorable and no cycle in $D_\varphi$
%  visits two streams $r$ and $s$ assigned to different nodes
%  $\mu(r)\neq \mu(s)$.
%\end{definition}
%
%Note that since \lola is very expressive many decision problems for
%\lola specs (well-formedness, equivalence, etc) are undecidable.
%%
%However, well-definedness (which guarantee that the monitoring
%algorithm always computes a verdict), efficient monitorability and
%decentralized efficient monitorability are syntactic properties which
%are very easy to check.
%
%We now define the notion of look-ahead of a stream $s$, that bounds
%for decentralized efficiently monitorable specifications the maximum
%between the moment at which $s[k]$ is inserted in $U_n$ and $s[k]$ is
%resolved into a value.
%%
%Note that a decentralized efficiently monitorable specification can be
%decomposed into a DAG of sets of stream variables such that each set
%is mapped to a single node (because cycles in the graph must belong to
%a single node).
%%
%We use $S(s)$ for the set of streams that are grouped with $s$.
%%
%In order to define the look-ahead distance $\nabla(s)$ we use an
%auxiliary definition: $\nablaR(s)$. 
%%
%This provides an upper-bound on the time to receive from a remote node
%the value of an instant variable $r[k']$ that $s[k]$ directly depends
%on.
%%
%\begin{itemize}
%\item If $r$ is eager, this value depends on $\nabla(r)$ to guarantee
%  that $r[k']$ is known at $k'+\nabla(r)$ and the time $\DIST(r,s)$ to
%  communicate this value.
%%
%\item If $r$ is lazy, the instant at which the network node of $r$
%  sends the value of $r[k']$ is the later instant between
%  $k'+\nabla(r)$ and the reception of the request, that is
%  $k+\DIST(s,r)$.
%%
%  After receiving the request, the response takes $\DIST(r,s)$ to
%  arrive to $s$.
%\end{itemize}
%%
%Once $\nablaR$ has been determined for all edges in the dependency
%graph that leave a component $S(s)$, $\nabla(s)$ can be determined by
%the weight of the maximum simple path in $S(s)$ adding also the
%additional time to resolve the remote dependencies.
%%
%Note that the definition of $\nabla(s)$ is identical to the look-ahead
%in a centralized specification with $S(s)$ as streams that considers
%directly accessible streams $r$ at remote nodes as input streams.
%%
%Formally:
%%
%\begin{definition}[Look-ahead]
%  The remote look-ahead distance $\nablaR(s)$ of a stream $s$ is
%%
%  \( \nablaR(s) \DefinedAs \max(0,\{ \DELAY(r\xrightarrow{w}s)\;|\;
%  \mu(r)\neq\mu(s)\}\),
%%
%  where
%%
%  \[
%   \DELAY(r\xrightarrow{w}s) \DefinedAs 
% \begin{cases}
%     \DIST(r,s) + w + \nabla(r) & 
%     \text{if \ISEAGER(r)} \\
%     \DIST(r,s) + \max(w + \nabla(r),d(s,r)) & 
%     \text{if \ISLAZY(r)}
%     \end{cases}
%  \]
%%   \begin{align*}
%%   \nablaR(s) &\DefinedAs \max(0,\{ \DELAY(r\xrightarrow{w}s)\;|\; \mu(r)\neq\mu(s)\} \text{, where}\\
%%   \DELAY(r\xrightarrow{w}s)&\DefinedAs 
%% \begin{cases}
%%     \DIST(r,s) + w + \nabla(r) & 
%%     \text{if \ISEAGER(r)} \\
%%     \DIST(r,s) + \max(w + \nabla(r),d(s,r)) & 
%%     \text{if \ISLAZY(r)}
%%     \end{cases}
%%   \end{align*}
%%
%%   \[
%%   \nablaR(s) \DefinedAs \begin{cases}
%%     \max(0,\{\DIST(r,s) + w + \nabla(r) \;|\; r\xrightarrow{w}s, \mu(r)\neq\mu(s) \} & \text{if \ISEAGER(r)} \\
%% %    \max(0,\{\DIST(r,s) + \max\begin{pmatrix}w + \nabla(r)\\d(s,r)\end{pmatrix} \;|\; r\xrightarrow{w}s, \mu(r)\neq\mu(s) \} & \text{if \ISLAZY(r)}
%%     \max(0,\{\DIST(r,s) + \max(w + \nabla(r),d(s,r)) \;|\; r\xrightarrow{w}s, \mu(r)\neq\mu(s) \} & \text{if \ISLAZY(r)}
%%     \end{cases}
%%   \]
%  The look-ahead distance is
%  \(
%  \nabla(s)\DefinedAs \max(0, \{ w + \nablaR(r) \;|\; s\xrightarrow{w}^* r \text{ with $S(s)=S(r)$}\})
%  \)
%\end{definition}
%%
%\noindent The definition is well-defined because the graph is a DAG of
%components, each of which is mapped to single network node.
%%
%Intuitively, the remote look-ahead $\nablaR(s)$ captures how long it
%takes to receive information from $\mu(r)$ that is relevant to compute
%$s[k]$.
%%
%Note that if the specification is centralized, then there is a single
%component, $\nablaR(s)$ is $0$ and the look-ahead distance coincides
%with the look-ahead for centralized Lola
%evaluation~\cite{sanchez18online}.
%
%\begin{lemma}
%  \label{lem:lookahead}
%  Every unresolved $s[k]=e$ in $U_n$ is resolved at most at
%  $k+\nabla(s)$.
%\end{lemma}
%%
%\noindent Lemmas~\ref{lem:backref} and~\ref{lem:lookahead} imply that
%decentralized efficiently monitorable specifications can be monitored
%with bounded resources.
%%
%The bound depends only linearly on the size of the specification and
%the diameter of the network.


%\vfill
%\pagebreak

% \begin{theorem}
%   Every decentralized efficiently monitorable specification can be
%   monitored with bounded memory, independently on the length of the
%   trace. 
% %
%   The bound depends linearly on the size of the specification and the
%   diameter of the network.
% \end{theorem}

%%% Local Variables:
%%% TeX-master: "main.tex"
%%% TeX-PDF-mode: t
%%% End:


==> figures/Makefile <==
IPETOIPE=/home/luismigueldanielsson/ipe-7.2.7-x86_64.AppImage ipetoipe #/Applications/Ipe.app/Contents/MacOS/ipetoipe
IPELATEXDIR=latex/
IPESTYLES=styles/
PWD=/home/luismigueldanielsson/Documents/Verification/svn/ares/papers/2019-dLola/figures/
FILES= ${PWD}RE_monitors \
	${PWD}RE_eval \
	${PWD}RE_lazy_needed \
	${PWD}RE_lazy_notneeded \
	${PWD}RE_star \
	${PWD}RE_msgs \
	#spec
	 #lift1 \
	 lift2 \
	 avgcpuwin \
	 winsum \
	 reset \
	 winsumwin \
	 avgcpu

ALL=$(addsuffix .pdf, ${FILES})

all: ${ALL}

%.pdf: %.ipe
	${IPETOIPE} -pdf $<

clean:
	rm -f ${ALL}


==> figures/latex/programs.tex <==
\newcommand{\RefFigListClass}{\ref{fig:programs}(a)\xspace}
\newcommand{\RefFigMGC}      {\ref{fig:programs}(b)\xspace}
\newcommand{\RefFigSearch}   {\ref{fig:programs}(c)\xspace}
\newcommand{\RefFigLocate}   {\ref{fig:programs}(d)\xspace}
\newcommand{\RefFigAdd}      {\ref{fig:programs}(e)\xspace}
\newcommand{\RefFigRemove}   {\ref{fig:programs}(f)\xspace}

\newcommand{\RefFigListClassGhost}{\ref{fig:programs:ghost}(a)\xspace}
\newcommand{\RefFigLocateGhost}		{\ref{fig:programs:ghost}(b)\xspace}
\newcommand{\RefFigAddGhost}			{\ref{fig:programs:ghost}(c)\xspace}
\newcommand{\RefFigRemoveGhost}		{\ref{fig:programs:ghost}(d)\xspace}

\newcommand{\FigLabel}[1]{\multicolumn{1}{c}{#1}}
\newcommand{\FigLabelWide}[1]{\multicolumn{3}{c}{#1}}

%
% Figures for data structure
%
\newcommand{\ListDataStructuresBody}{
  \begin{array}{l>{\hspace{0.25em}}l<{\hspace{0.25em}}l}
	  \class & \List & \{ \Node \: \tList; \; \} \\
	  \class & \Node & \{
			\Value \: \val; \;
			\Node \: \tNext; \;
			\Lock \: \lock; \; \}
  \end{array}
}



%
% Figures for most generate cliente "decide"
%
\newcommand{\ListMGCBody}{
  \begin{algorithmic}[1]
	\Procedure{MGC}{}
	  \While {$\true$}
	  \State $e := \NondetChooseElem$
	  \State $\Nondet$
	  \State $\left[ \begin{array}{l}
		\Call \search(e) \\
		\ProgOr \\
		\Call \insertProg(e) \\
		\ProgOr \\
		\Call \remove(e)
	  \end{array} \right]$
	  \EndWhile
	\EndProcedure
  \end{algorithmic}
}



%
% Figure for "search" 
%

\newcommand{\ListSearchBody}{
  \begin{algorithmic}[1]
	\Procedure{Search}{$\Value \: e$}
	\State $\prev, \curr := \locate(e)$
    \If {$\curr.\val = e$}
    \State $\result := \true$
    \Else
    \State $\result := \false$
    \EndIf
    \State $\curr.\unlock()$
    \State $\prev.\unlock()$
    \State \tbf{return} $\result$
	\EndProcedure
  \end{algorithmic}
}



%
% Figure for "locate"
%
\newcommand{\ListLocateBody}{
  \begin{algorithmic}[1]
	\Procedure{Locate}{$\Value \: e$}
	  \State $\prev := \Head$
	  \State $\prev.\lock()$
	  \State $\curr := \prev.\tNext$
	  \State $\curr.lock()$
	  \While {$\curr.\val < e$}
		\State $\prev.\unlock()$
		\State $\prev := \curr$
		\State $\curr := \curr.\tNext$
		\State $\curr.\lock()$
	  \EndWhile
	  \State \tbf{return} $(\prev, \curr)$
	\EndProcedure
  \end{algorithmic}
}



%
% Figure for "add"
%
\newcommand{\ListAddBody}{
  \begin{algorithmic}[1]
	\Procedure{Insert}{$\Value \: e$}
	  \State $\prev, \curr := \locate(e)$
	  \If {$\curr.\val \neq e$}
		\State $\aux := \New \Node(e)$
		\State $\aux.\tNext := \curr$
		\State $\prev.\tNext := \aux$
		\State $\result := \true$
	  \Else
		\State $\result := \false$
	  \EndIf
	  \State $\prev.\unlock()$
	  \State $\curr.\unlock()$
	  \State \tbf{return} $\result$
	\EndProcedure
  \end{algorithmic}
}



%
% Figure for "remove"
%
\newcommand{\ListRemoveBody}{
    \begin{algorithmic}[1]
	  \Procedure{Remove}{$\Value \: e$}
		\State $\prev, \curr := \locate(e)$
		\If {$\curr.\val = e$}
		  \State $\aux := \curr.\tNext$
		  \State $\prev.\tNext := \aux$
		  \State $\result := \true$
		\Else
		  \State $\result := \false$
		\EndIf
		\State $\prev.\unlock()$
		\State $\curr.\unlock()$
		\State \tbf{return} $\result$
	  \EndProcedure
	\end{algorithmic}
}




%
% Figures for data structure
%
\newcommand{\DataStructuresGhostBody}{
	\begin{tabular}{cc}
		\renewcommand{\arraystretch}{0.4}
		$\begin{array}{l}
			\class \: \List \: \{ \\
			\mhs \Node \: \tList ;\\
			\hs{0.2} \fbox{ \begin{array}{l}
				\rgn \: r; \\
			\end{array}}\\
		\}
		\end{array}$ & \hs{2} $\begin{array}{l}
			\class \: \Node \: \{ \\
			\mhs \Value \: \val ;\\
			\mhs \Node \: \tNext ;\\
			\mhs \Lock \: \lock ;\\
		\}
	\end{array}$
	\end{tabular}
}

\newcommand{\DataStructuresGhostFig}{
\begin{minipage}[c]{6.5cm}
	\DataStructuresGhostBody
\label{fig:conclists:ghost}
\end{minipage}
}


%
% Figure for "locate" extended with ghost fields
%

\newcommand{\ListLocateGhostBody}{
  \begin{algorithmic}[1]
	\Procedure{Locate}{$\Value \: e$}
	  \State $\prev := \Head$
	  \State $\prev.\lock()$
	  \State $\curr := \prev.\tNext$
	  \State $\curr.lock()$
	  \While {$\curr.\val < e$}
		\State $\prev.\unlock()$
		\State $\prev := \curr$
		\State $\curr := \curr.\tNext$
		\State $\curr.\lock()$
	  \EndWhile
	  \State \tbf{return} $(\prev, \curr)$
	\EndProcedure
  \end{algorithmic}
}


%
% Figure for "add" extended with ghost fields
%
\newcommand{\ListAddGhostBody}{
  \begin{algorithmic}[1]
	\Procedure{Insert}{$\Value \: e$}
	  \State $\prev, \curr := \locate(e)$
	  \If {$\curr.\val \neq e$}
		\State $\aux := \New \Node(e)$
		\State $\aux.\tNext := \curr$
		\State $\prev.\tNext := \aux$
		\Statex $\hs{0.7}\fbox{
		  \begin{array}{l}
			l.r := l.r \cup \sreg{\aux} \\
		  \end{array}}$
		\State $\result := \true$
	  \Else
		\State $\result := \false$
	  \EndIf
	  \State $\prev.\unlock()$
	  \State $\curr.\unlock()$
	  \State \tbf{return} $\result$
	\EndProcedure
  \end{algorithmic}
}



%
% Figure for "remove" extended with ghost fields
%
\newcommand{\ListRemoveGhostBody}{
  \begin{algorithmic}[1]
	\Procedure{Remove}{$\Value \: e$}
	  \State $\prev, \curr := \locate(e)$
	  \If {$\curr.\val = e$}
		\State $\aux := \curr.\tNext$
		\State $\prev.\tNext := \aux$
		\Statex $\hs{0.7}\fbox{
		  \begin{array}{l}
			l.r := l.r - \sreg{\curr} \\
		  \end{array}}$
		\State $\result := \true$
	  \Else
		\State $\result := \false$
	  \EndIf
	  \State $\prev.\unlock()$
	  \State $\curr.\unlock()$
	  \State \tbf{return} $\result$
	\EndProcedure
  \end{algorithmic}
}


%
% Figure for data structure for proving no overtake
%
\newcommand{\DataStructuresGhostTicketBody}{
	\begin{tabular}{c>{\hspace{1cm}}c}
		\renewcommand{\arraystretch}{0.4}
		$\begin{array}{l}
			\class \: \List \: \{ \\
			\mhs \Node \: \tList ;\\
			\hs{0.2} \fbox{ \begin{array}{l}
				\rgn \: r; \\
			\end{array}} \\
		\}
		\end{array}$ & 
		$\begin{array}{l}
			\class \: \Node \: \{ \\
			\mhs \Value \: \val ;\\
			\mhs \Node \: \tNext ;\\
			\mhs \Lock \: \lock ;\\
		\}
	\end{array}$
	\end{tabular}
}

\newcommand{\DataStructuresGhostTicketFig}{
\begin{minipage}[c]{5cm}
	\DataStructuresGhostTicketBody
\label{fig:struct-cl-ticket}
\end{minipage}
}



%
% Figure for "locate" extended with ghost fields for proving no overtake
%

\newcommand{\ListLocateGhostTicketBody}{
  \begin{algorithmic}[1]
	\Procedure{Locate}{$\Value \: e$}
	  \State $\prev := \Head$
	  \State $\prev.\lock()$
	  \Statex $\hs{0.7}\fbox{
		\begin{array}{l}
		  \myTicket := \ticket \\
		  \ticket := \ticket + 1 \\
		\end{array}}$
	  \State $\curr := \prev.\tNext$
	  \State $\curr.lock()$
	  \While {$\curr.\val < e$}
		\State $\prev.\unlock()$
		\State $\prev := \curr$
		\State $\curr := \curr.\tNext$
		\State $\curr.\lock()$
	  \EndWhile
	  \State \tbf{return} $(\prev, \curr)$
	\EndProcedure
  \end{algorithmic}
}




\newcommand{\RefFigSkiplistClass}{\ref{fig:programs}(a)\xspace}
\newcommand{\RefFigInsert}{\ref{fig:programs}(b)\xspace}

%
% Figures for data structure
%
\newcommand{\SkiplistDataStructuresBody}{
	\begin{array}{l>{\hspace{0.25em}}l>{\hspace{0.25em}}llll}
		\class & \SkipList & \{ &
			\NodeP & \head; \; \\
			&&& \NodeP & \tail; \\
			&&& \Tint & \maxLevel; \\
			&&& \TSet{\Addr} & @\reg; & \} \\
		\class & \Node & \{ &
			\Value & \val;		\\
			&&& \Key & \key;	\\
			&&& \TArray \langle \NodeP \rangle & \fNext; \\
			&&& \Tint & @\level; & \}
%			&&& \TArray \langle \NodeP \rangle \: \lock; & \}
  \end{array}
}


\newcommand{\SkiplistInsertBody}{
%  \framebox[\textwidth]{
	\begin{algorithmic}[1]
	\Statex
	\Procedure{Insert}{$\SkipList \: sl$, $\Value \: \newval$}
	\MState {$\Tvector\tuple{\NodeP} \upd[0..K-1]$}
			{$\mrgn \: m_r := \emptyset$}{8}{0}
	\State $lvl := \randomLevel(K)$
	\State $\NodeP \pred := sl.\head$
	\MState {$\pred.\locks[K-1].\lock()$}
			{$m_r := m_r \cup \{ (\pred, K-1) \}$}{8}{0}
	\State $\NodeP \curr := \pred.\fNext[K-1]$
	\MState {$\curr.\locks[K-1].\lock()$}
			{$m_r := m_r \cup \{ (\curr, K-1) \}$}{8}{0}
	\For {$i:=K-1$ downto $0$}
		\If {$i < K -1$}
			\MState {$\pred.\locks[i].\lock()$}
					{$m_r := m_r \cup \{ (\pred, i) \}$}{8}{2}
			\If {$i \geq lvl$}
				\MState {$\curr.\locks[i+1].\unlock()$}
						{$m_r := m_r - \{ (\curr, i+1) \}$}{8}{3}
				\MState {$\pred.\locks[i+1].\unlock()$}
						{$m_r := m_r - \{ (\pred, i+1) \}$}{8}{3}
			\EndIf
			\State $\curr := \pred.\fNext[i]$
			\MState {$\curr.\locks[i].\lock()$}
					{$m_r := m_r \cup \{ (\curr, i) \}$}{8}{2}
		\EndIf
		\While {$\curr.\val < \newval$}
			\MState {$\pred.\locks[i].\unlock()$}
					{$m_r := m_r - \{ (\pred, i) \}$}{8}{2}
			\State $\pred := \curr$
			\State $\curr := \pred.\fNext[i]$
			\MState {$\curr.\locks[i].\lock()$}
					{$m_r := m_r \cup \{ (\curr, i) \}$}{8}{2}
		\EndWhile
		\State $\upd[i] := \pred$
	\EndFor
	\State $\bool \: \valueWasIn := (\curr.\val = \newval)$

	\If {$\valueWasIn$}
		\For {$i := 0$ to $lvl$}
			\MState {$\upd[i].\fNext[i].\locks[i].\unlock()$}
					{$m_r := m_r - \{ (\upd[i].\fNext[i], i)\}$}
						{8}{2}
			\MState {$\upd[i].\locks[i].\unlock()$}
					{$m_r := m_r - \{ (\upd[i], i) \}$}{8}{2}
		\EndFor
	\Else
		\State $x:=\CreateNode(lvl, \newval)$
		\For {$i:=0$ to $lvl$}
			\State $x.\fNext[i] := \upd[i].\fNext[i]$
			\MState {$\upd[i].\fNext[i] := x$}
					{$sl.r := sl.r \cup \{ (x, i) \}$}{8}{2}
			\MState {$x.\fNext[i].\locks[i].\unlock()$}
					{$m_r := m_r - \{ (x.\fNext[i], i) \}$}
						{8}{2}
			\MState {$\upd[i].\locks[i].\unlock()$}
					{$m_r := m_r - \{ (\upd[i], i) \}$}{8}{2}
		\EndFor
	\EndIf
	\State $\tbf{return } \lnot \valueWasIn$
	\EndProcedure
	\end{algorithmic}
%      }
}




==> figures/latex/theories.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TLLpL Signature
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\TLLpLSignature}{
\centering
\begin{tabular}{r>{\vspace{-.5\baselineskip}}p{10.5cm}}
\hline
\textbf{Signature:} & \sigCells \\
\textbf{Sorts:} & \sCell, \sElem, \sAddr, \sThId \\
\textbf{Functions:} &
			\begin{array}{p{1.6cm}cl}
			\fError & : & \sCell \\
			\fMkcell & : & \sElem \times \sAddr \times \sThId \to \sCell \\
			\_.\fData & : & \sCell \to \sElem \\
			\_.\fNext & : & \sCell \to \sAddr \\
			\_.\fLockID & : & \sCell \to \sThId \\
			\_.\fLock & : & \sCell \to \sThId \to \sCell \\
			\_.\fUnlock & : & \sCell \to \sCell \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigMemory \\
\textbf{Sorts:} & \sMem, \sAddr, \sCell\\
\textbf{Functions:} &
			\begin{array}{p{1.6cm}cl}
			\fNull & : & \sAddr \\
			\_[\_] & : & \sMem \times \sAddr \to \sCell \\
			\fUpd & : & \sMem \times \sAddr \times \sCell \to \sMem \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigReach \\
\textbf{Sorts:} & \sMem, \sAddr, \sPath \\
\textbf{Functions:} &
			\begin{array}{p{1.6cm}cl}
			\fEpsilon & : & \sPath \\
			\lbrack \_ \rbrack & : & \sAddr \to \sPath \\
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{1.6cm}cl}
			\pAppend & : & \sPath \times \sPath \times \sPath \\
			\pReach & : & \sMem \times \sAddr \times \sAddr \times \sPath \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigSets \\
\textbf{Sorts:} & \sAddr, \sSet \\
\textbf{Functions:} &
			\begin{array}{p{1.6cm}cl}
			$\emptyset$ & : & \sSet \\
			\{ \_ \} & : & \sAddr \to \sSet \\
			$\cup$, $\cap$, $\setminus$ & : & \sSet \times \sSet \to \sSet
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{1.6cm}cl}
			$\in$ & : & \sAddr \times \sSet \\
			$\subseteq$ & : & \sSet \times \sSet
			\end{array} \\
\hline
\textbf{Signature:} & \sigSetsT \\
\textbf{Sorts:} & \sThId, \sSetT \\
\textbf{Functions:} &
			\begin{array}{p{1.6cm}cl}
			\stEmpty & : & \sSetT \\
			\stSingle{\_} & : & \sThId \to \sSetT \\
			\stCup, \stCap, \stSubst & : & \sSetT \times \sSetT \to \sSetT
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{1.6cm}cl}
			\stIn & : & \sThId \times \sSetT \\
			\stSubset & : & \sSetT \times \sSetT
			\end{array} \\
\hline
\textbf{Signature:} & \sigBridge \\
\textbf{Sorts:} & \sMem, \sAddr, \sSet, \sPath \\
\textbf{Functions:} &
			\begin{array}{p{1.6cm}cl}
			\fPathToSet & : & \sPath \to \sSet \\
			\fAddrToSet & : & \sMem \times \sAddr \to \sSet \\
			\fGetp & : & \sMem \times \sAddr \times \sAddr \to \sPath \\
			\fFirstLocked & : & \sMem \times \sPath \to \sAddr
			\end{array} \\
\hline
\end{tabular}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TLLpL Interpretations
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\TLLpLInterpretations}{
\centering
\begin{tabular}{r>{\vspace{-.5\baselineskip}}p{10.5cm}}
\hline
\textbf{signature:} & \sigCells \\
\textbf{interpretation:} &
		\begin{compactitem}
		\item $\fMkcell (e, a, k) =
			\langle e, a, k \rangle$
		\item $\langle e, a, t \rangle.\inter{\fData}{\Ai} = e$
		\item $\langle e, a, t \rangle.\inter{\fNext}{\Ai} = a$
		\item $\langle e, a, t \rangle.\inter{\fLockID}{\Ai} = t$
		\item $\langle e, a, t \rangle.\inter{\fLock}{\Ai}(t') =
			\langle e, a, t' \rangle$
		\item $\langle e, a, t \rangle.\inter{\fUnlock}{\Ai} =
			\langle e, a, \oslash \rangle$
		\item $\inter{\fError}{\Ai}.\inter{\fNext}{\Ai} =
			\inter{\fNull}{\Ai}$
		\end{compactitem} \\
		& for each
			$e \in \Ais{\sElem}$,
			$a \in \Ais{\sAddr}$,
			$k \in \Ais{\sThId}$
			and $t, t' \in \Ais{\sThId}$ \\
\hline
\textbf{Signature:} & \sigMemory \\
\textbf{Interpretation:} &
		\begin{compactitem}
		\item $m\inter{[a]}{\Ai} = m(a)$
		\item $\inter{\fUpd}{\Ai}(m,a,c) = m_{a \mapsto c}$
		\item $\inter{m}{\Ai}(\inter{\fNull}{\Ai}) = \inter{\fError}{\Ai}$
		\end{compactitem} \\
		& for each
			$m \in \Ais{\sMem}$,
			$a \in \Ais{\sAddr}$ and
			$c \in \Ais{\sCell}$ \\
\hline
\textbf{Signature:} & \sigReach \\
\textbf{Interpretation:} &
		\begin{compactitem}
		\item $\inter{\fEpsilon}{\Ai}$ is the empty sequence
		\item $\inter{[i]}{\Ai}$ is the sequence containing $i \in 
			\Ais{\sAddr}$ as the only element
		\item $\left(\left[i_1,\ldots, i_n\right], \left[j_1, \ldots, 
			j_m\right], \left[i_1,\ldots, i_n, j_1,
				\ldots, j_m\right]
			\right) \in \inter{\pAppend}{\Ai}$ iff

			\mhs $i_k$ and $j_l$ are all distinct
		\item $\left(m, i, j, p\right) \in \inter{\pReach}{\Ai}$ iff
			\begin{compactitem}
				\item $i=j$ and $p = \fEpsilon$, or
				\item there exist addresses $i_1, \ldots, i_n \in
						\Ais{\sAddr}$ such that:
			\end{compactitem}
		\end{compactitem} \\
		& \hs{1.5} $\begin{array}{l>{\hspace{1em}}l}
			\trm{(a) } p = [i_1, \ldots, i_n] &
			\trm{(c) } m(i_r).\inter{\fNext}{\Ai} = i_{r+1}$,
				for $1 \leq r < n \\
			\trm{(b) } i_1 = i &
			\trm{(d) } m(i_n).\inter{\fNext}{\Ai} = j
		\end{array}$ \\
\hline
\textbf{Signature:} & \sigSets \\
\textbf{Interpretation:} &
		\begin{compactitem}
		\item The symbols $\emptyset$, $\{ \_ \}$, $\cup$, $\cap$,
				$\setminus$, $\in$ and $\subseteq$ are interpreted according
				to their standard interpretation over sets of addresses.
		\end{compactitem}\\
\hline
\textbf{Signature:} & \sigSetsT \\
\textbf{Interpretation:} &
		\begin{compactitem}
		\item The symbols $\stEmpty$, $\stSingle{\_}$, $\stCup$, $\stCap$,
				$\stSubst$, $\stIn$ and $\stSubset$ are interpreted according
				to their standard interpretation over sets of thread
				identifiers.
		\end{compactitem}\\
\hline
\textbf{Signature:} & \sigBridge \\
\textbf{Interpretation:} &
		\begin{compactitem}
		\item $\inter{\fAddrToSet}{\Ai}(m, i) = \big\{ j \in \Ais{\sAddr} 
			\:|\: \exists p \in \Ais{\sPath}$
				s.t. $(m,i,j,p) \in \pReach \big\}$

		\item $\inter{\fPathToSet}{\Ai}(p) = \{ i_1, \ldots, i_n\}$ for $p = 
			[i_1, \ldots, i_n] \in \Ais{\sPath}$

		\item $\inter{\fGetp}{\Ai}(m,i,j) =
			\begin{cases}
				p & \text{if } (m,i,j,p)
					\in \inter{\pReach}{\Ai} \\
				\fEpsilon & \text{otherwise}
			\end{cases}$
		\end{compactitem} \\
		
		& \hs{1} for each $m \in \Ais{\sMem}$,
		$p \in \Ais{\sPath}$ and $i,j \in \Ais{\sAddr}$ \\

		& \begin{compactitem}
		\item $\inter{\fFirstLocked}{\Ai}\left(m,[a_1, \ldots, 
			a_n]\right) =
			\left\{
			\begin{array}{ll}
			a_k &
			\trm{if there is } 1 \leq k \leq n \trm{ such that } \\
			& \trm{for all } 1 \leq j < k,
				m[a_j].\fLockID = \oslash \\
			& \trm{and } m[a_k].\fLockID \neq \oslash \\
			\fNull & \trm{otherwise }
			\end{array}
			\right.$
		\end{compactitem} \\
		& \hs{1} for each $m \in \Ais{\sMem}$ and
			$a_1, \ldots a_n \in \Ais{\sAddr}$ \\
\hline
\end{tabular}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TLLpL PATH Auxiliary functions
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ListTPathFig}{
\renewcommand{\arraystretch}{1.1}
\centering
\begin{tabular}{|c|}
\hline
$\fApp : \sSeq \times \sSeq \to \sSeq$ \\
\hline
$\fApp (\fNil, l) = l$ \\
$\fApp(\fCons(a,l), l') = \fCons(a, \fApp(l, l'))$ \\
\hline
\hline
$\fSeqToSet : \sSeq \to \sSet$ \\
\hline
$\fSeqToSet (\fNil) = \emptyset$ \\
$\fSeqToSet (\fCons(a,l)) = \{ a \} \cup \fSeqToSet(l)$ \\
\hline
\hline
$\fIsPath : \sSeq$ \\
\hline
$\fIsPath(\fNil)$ \\
$\fIsPath(\fCons(a, \fNil))$ \\
$\{a\} \nsubseteq \fSeqToSet(l) \land \fIsPath(l) \Impl
	\fIsPath(\fCons(a,l))$ \\
\hline
\hline
$\fLast : \sSeq \to \sAddr$ \\
\hline
$\fLast(\fCons(a, \fNil)) = a$ \\
$l \neq \fNil \Impl \fLast(\fCons(a, l)) = \fLast(l)$ \\
\hline
\hline
$\pIsReach : \sMem \times \sAddr \times \sAddr$ \\
\hline
$\pIsReach(m, a, a)$ \\
$m[a].\fNext = a' \land \pIsReach(m, a', b) \Impl \pIsReach(m, a, b)$ \\
\hline
\hline
$\pIsReachP : \sMem \times \sAddr \times \sAddr \times \sSeq$ \\
\hline
$\pIsReachP(m, a, a, \fNil)$ \\
$m[a].\fNext = a' \land \pIsReachP(m, a', b, p) \Impl
	\pIsReachP(m, a, b, \fCons(a, p))$ \\
\hline
\hline
$\fFirstMarked : \sMem \times \sSeq \times \sAddr$ \\
\hline
$\fFirstMarked (m, \fNil, \fNull)$ \\
	\Impl
	\fFirstMarked(m, p, j)$ \\
	\land
	\fFirstMarked(m, q, i) \Impl \fFirstMarked(m, p, i)$ \\
\hline
\end{tabular}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TLLpL Auxiliary Functions
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ListAuxiliaryFunctions}{
\renewcommand{\arraystretch}{1.1}
\centering
\begin{tabular}{|c|}
\hline
$\List : \sMem \times \sAddr \times \sSet$ \\
\hline
$\begin{array}{lcl}
	\List(h,a,r) & \Iff & \fNull \in \fAddrToSet(h, a)
		\land r = \fPathToSet(\fGetp(h, a, \fNull)) \\
\end{array}$\\
\hline
\hline
$\fa : \sMem \times \sAddr \to \sPath$ \\
\hline
$\fa(h,n) = \begin{cases}
		\fEpsilon & \trm{if } n = \fNull \\
		\fGetp(h, h[n].\fNext, \fNull) & \trm{if } n \neq \fNull \\
		\end{cases}$ \\
\hline
%
% Begin: Function removed to reduce space
%
\hline
$\fb : \sMem \times \sAddr \times \sAddr \times \sPath$ \\
\hline
$\begin{array}{lclll}
\fb(h, n, m, p) & \Iff & (n = \fNull \land p = \fEpsilon) \quad \lor \\
		& & \big(n \neq \fNull \land \pReach(h,n,m,\tilde{p})
			& \land & m=\fNull	\Impl \pAppend(p, \fNull, \tilde{p}) \\
		& & & \land & m\neq \fNull \Impl \pAppend(p,[m],\tilde{p}) \big)
\end{array}$ \\
\hline
%
% End: Function removed to reduce space
%
\hline
$\LastMarked : \sMem \times \sPath \to \sAddr$ \\
\hline
$\LastMarked(m, p) = \fFirstLocked(m, \fRev(p))$ \\
\hline
\hline
$\NoMarks : \sMem \times \sPath$ \\
\hline
$\NoMarks(m,p) \Iff \fFirstLocked(m,p) = \fNull$ \\
\hline
\hline
$\SomeMark : \sMem \times \sPath$ \\
\hline
$\SomeMark(m,p) \Iff \fFirstLocked(m,p) \neq \fNull$ \\
\hline
\end{tabular}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TSLK Signature - Table One
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\TSLKSignatureOne}{
\centering
\begin{tabular}{r>{\vspace{-.5\baselineskip}}p{9cm}}
\hline
\textbf{Signature:} & \sigLevelK \\
\textbf{Sorts:} & \sLevelK \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			0,1, \ldots, \K-1 & : & \sLevelK \\
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			$<$  & : & \sLevelK \times \sLevelK \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigOrd \\
\textbf{Sorts:} & \sOrd \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\fZero, \fInfty & : & \sOrd \\
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			\pOrd & : & \sOrd \times \sOrd \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigCells \\
\textbf{Sorts:} & \sCell, \sElem, \sOrd, \sLevelK, \sAddr \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\fError & : & \sCell \\
			\fMkcell & : & \sElem \times \sOrd \times \sAddr^{\K}
							\to \sCell \\
			\_.\fData & : & \sCell \to \sElem \\
			\_.\fKey & : & \sCell \to \sOrd \\
			\_.\fNext \lbrack \_ \rbrack & : & \sCell \times \sLevelK
							\to \sAddr \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigMemory \\
\textbf{Sorts:} & \sMem, \sAddr, \sCell \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\fNull & : & \sAddr \\
			\fRd & : & \sMem \times \sAddr \to \sCell \\
			\fUpd & : & \sMem \times \sAddr \times \sCell \to \sMem \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigReach \\
\textbf{Sorts:} & \sMem, \sAddr, \sLevelK, \sPath \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\fEpsilon & : & \sPath \\
			\lbrack \_ \rbrack & : & \sAddr \to \sPath \\
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			\pAppend & : & \sPath \times \sPath \times \sPath \\
			\pReachK & : & \sMem \times \sAddr \times \sAddr
							\times \sLevelK \times \sPath \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigSets \\
\textbf{Sorts:} & \sAddr, \sSet \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			$\emptyset$ & : & \sSet \\
			$\{ \_ \}$ & : & \sAddr \to \sSet \\
			$\cup$, $\cap$, $\setminus$ & : & \sSet \times \sSet
								\to \sSet \\
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			$\in$ & : & \sAddr \times \sSet \\
			$\subseteq$ & : & \sSet \times \sSet \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigBridge \\
\textbf{Sorts:} & \sMem, \sAddr, \sLevelK, \sSet, \sPath \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\fPathToSet & : & \sPath \to \sSet \\
			\fAddrToSetK & : & \sMem \times \sAddr \times \sLevelK
							\to \sSet \\
			\fGetpK & : & \sMem \times \sAddr \times \sAddr
							\times \sLevelK \to \sPath \\
			%\fThreadSubset & : & \sMem \times \sAddr \times \sAddr
							%\times \sLevelK \to \sSetT
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			\pOrdList & : & \sMem \times \sPath \\
			\end{array} \\
\hline
\end{tabular}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TSLK Signature - Table Two
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\TSLKSignatureTwo}{
\centering
\begin{tabular}{r>{\vspace{-.5\baselineskip}}p{9cm}}
\hline
\textbf{Signature:} & \sigSetsT \\
\textbf{Sorts:} & \sThId, \sSetT \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\stEmpty & : & \sSetT \\
			\stSingle{\_} & : & \sThId \to \sSetT \\
			\stCup, \stCap, \stSubst & : & \sSetT \times \sSetT
								\to \sSetT \\
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			\stIn & : & \sThId \times \sSetT \\
			\stSubset & : & \sSetT \times \sSetT \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigMrgn \\
\textbf{Sorts:} & \sMrgn, \sAddr, \sLevelK \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\mrgnEmpty & : & \sMrgn \\
			\mrgnSingle{\_, \_} & : & \sAddr \times \sLevelK \to \sMrgn \\
			\mrgnCup, \mrgnCap, \mrgnMinus & : & \sMrgn \times \sMrgn
							\to \sMrgn \\
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			\mrgnIn & : & \sAddr \times \sLevelK \times \sMrgn \\
			\mrgnSubset & : & \sMrgn \times \sMrgn \\
			\mrgnDisj & : & \sMrgn \times \sMrgn \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigAArray \\
\textbf{Sorts:} & \sAArray, \sThId, \sAddr \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\aarrRd{\_}{\_} & : & \sAArray \times \sThId \to \sAddr \\
			\aarrUpd{\_}{\_}{\_} & : &
					\sAArray \times \sThId \times \sAddr \to \sAArray \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigLArray \\
\textbf{Sorts:} & \sLArray, \sThId, \sLevelK \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\larrRd{\_}{\_} & : & \sLArray \times \sThId \to \sLevelK \\
			\larrUpd{\_}{\_}{\_} & : &
					\sLArray \times \sThId \times \sLevelK \to \sLArray \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigBridge \\
\textbf{Sorts:} & \sMem, \sAddr, \sLevelK, \sSet, \sPath \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\fPathToSet & : & \sPath \to \sSet \\
			\fAddrToSetK & : & \sMem \times \sAddr \times \sLevelK
							\to \sSet \\
			\fGetpK & : & \sMem \times \sAddr \times \sAddr
							\times \sLevelK \to \sPath \\
			\fFirstLockedK & : & \sMem \times \sPath \times \sLevelK
							\to \sAddr \\
			%\fThreadSubset & : & \sMem \times \sAddr \times \sAddr
							%\times \sLevelK \to \sSetT
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			\pOrdList & : & \sMem \times \sPath \\
			\end{array} \\
\hline
\end{tabular}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TSLK Interpretations
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\TSLKInterpretations}{
\centering
\begin{tabular}{p{11cm}}
\hline \\
\textbf{Signature:} $\sigCells$ \\
\textbf{Interpretations:} \\
  \hspace{1.5em}
  \begin{tabular}{p{10cm}}
    \begin{compactitem}
		\item $\inter{\fMkcell}{\Ai} (e, k, \vect{a}) =
			\langle e, k, \vect{a} \rangle$
		\item $\inter{\fError}{\Ai}.\inter{\fNext}{\Ai} =
			\inter{\fNull}{\Ai}$
		\item $\langle e, k, \vect{a} \rangle
				.\inter{\fData}{\Ai} = e$
		\item $\langle e, k, \vect{a} \rangle
				.\inter{\fKey}{\Ai} = k$
		\item $\langle e, k, \vect{a} \rangle
				.\inter{\fNext}{\Ai}[j] = a_j$
		\end{compactitem} \\
    for each
			$e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$\vect{a} \in \Ais{\sAddr}^{\K}$ and
			$j \in \Ais{\sLevelK}$ \\
  \end{tabular} \\ \\
\hline \\
\textbf{Signature:} $\sigMemory$ \\
\textbf{Interpretations:} \\
  \hspace{1.5em}
  \begin{tabular}{p{10cm}}
		\begin{compactitem}
		\item $\inter{\fRd}{\Ai}(m,a) = m(a)$
		\item $\inter{\fUpd}{\Ai}(m,a,c) = m_{a \mapsto c}$
		\item $\inter{m}{\Ai}(\inter{\fNull}{\Ai}) = \inter{\fError}{\Ai}$
		\end{compactitem} \\
    for each
      $m \in \Ais{\sMem}$,
			$a \in \Ais{\sAddr}$
      and $c \in \Ais{\sCell}$ \\
  \end{tabular} \\ \\
\hline \\
\textbf{Signature:} $\sigReach$ \\
\textbf{Interpretations:} \\
  \hspace{1.5em}
  \begin{tabular}{p{10cm}}
    \begin{compactitem}
    \item $\inter{\fEpsilon}{\Ai}$ is the empty sequence
		\item $\inter{[i]}{\Ai}$ is the sequence containing $i \in
					\Ais{\sAddr}$ as the only element
		\item $\left(\left[i_1 \,..\, i_n\right], 
				\left[j_1\,..\,j_m\right],
				\left[i_1\,..\,i_n, j_1\,..\,j_m\right]\right)
					\in \inter{\pAppend}{\Ai}$ iff $i_k\neq j_l$
		\item $(m, \aInit, \aEnd, l, p) \in \inter{\pReachK}{\Ai}$
				iff $\aInit=\aEnd$ and $p = \fEpsilon$, or
				there exist addresses $a_1, \ldots, a_n \in \Ais{\sAddr}$
				such that:
		\end{compactitem}
		\hs{1.4} $\begin{array}{ll}
			\trm{(a) } p = [a_1\,..\,a_n]  \phantom{aaaa}&
			\trm{(c) } m(a_r).\inter{\fNext}{\Ai}[l]
						= a_{r+1}, \;\;\text{for}\;\;\;r < n \\
			\trm{(b) } a_1 = \aInit &
			\trm{(d) } m(a_n).\inter{\fNext}{\Ai}[l] = \aEnd
    \end{array}$ \\
  \end{tabular} \\ \\
\hline \\
\textbf{Signature:} $\sigBridge$ \\
\textbf{Interpretations:} \\
  \hspace{1.5em}
  \begin{tabular}{p{10cm}}
    \begin{compactitem}
		\item $\inter{\fPathToSet}{\Ai}(p)
					= \{ a_1, \ldots, a_n\}$ for $p
					= [a_1, \ldots, a_n] \in \Ais{\sPath}$
		\item $\inter{\fAddrToSetK}{\Ai}(m, a, l)
					= \big\{a' \in \Ais{\sAddr} | \exists p \in \Ais{\sPath}$ 
						. $(m,a,a',l,p) \in \pReachK
						\big\}$
		\item $\inter{\fGetpK}{\Ai}(m,\aInit,\aEnd,l) =
			\begin{cases}
				p & \text{if } (m,\aInit,\aEnd,l,p)
					\in \inter{\pReachK}{\Ai} \\
				\fEpsilon & \text{otherwise}
			\end{cases}$
    \end{compactitem} \\
    \hs{1} for each
      $m \in \Ais{\sMem}$,
			$p \in \Ais{\sPath}$,
			$l \in \Ais{\sLevelK}$
			and $\aInit, \aEnd \in \Ais{\sAddr}$ \\
    \begin{compactitem}
    \item $\inter{\pOrdList}{\Ai}\left(m,p \right)$
			iff
			\begin{compactitem}
				\item $p=\fEpsilon$, or
				\item $p = \lbrack a \rbrack$, or
				\item $p = [a_1\,..\, a_n]$ with $n \geq 2$ and
						$m(a_i).\inter{\key}{\Ai} \pOrd
						m(a_{i+1}).\inter{\key}{\Ai}$
						for all $1 \leq i < n$,
						for any $m \in \Ais{\sMem}$
			\end{compactitem}
		\end{compactitem} \\
  \end{tabular} \\ \\
\hline \\
\end{tabular}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TSLK PATH Auxiliary functions
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\SkiplistTPathFig}{
\renewcommand{\arraystretch}{1.1}
\centering
\begin{tabular}{l}
	\hline
	$\fApp : \sSeq \times \sSeq \to \sSeq$ \\
	$\fApp (\fNil, l) = l$ \\
	$\fApp(\fCons(a,l), l') = \fCons(a, \fApp(l, l'))$ \\
	\hline
	$\fSeqToSet : \sSeq \to \sSet$ \\
	$\fSeqToSet (\fNil) = \emptyset$ \\
	$\fSeqToSet (\fCons(a,l)) = \{ a \} \cup \fSeqToSet(l)$ \\
	\hline
	$\fIsPath : \sSeq$ \\
	$\fIsPath(\fNil)$ \\
	$\fIsPath(\fCons(a, \fNil))$ \\
	$\{a\} \nsubseteq \fSeqToSet(l) \land \fIsPath(l) \Impl
		\fIsPath(\fCons(a,l))$ \\
	\hline
	$\fLast : \sSeq \to \sAddr$ \\
	$\fLast(\fCons(a, \fNil)) = a$ \\
	$l \neq \fNil \Impl \fLast(\fCons(a, l)) = \fLast(l)$ \\
	\hline
	$\pIsReachK : \sMem \times \sAddr \times \sAddr \times \sLevelK$ \\
	$\pIsReachK(m, a, a, l)$ \\
	$m[a].\fNext[l] = a' \land \pIsReachK(m, a', b, l)
		\Impl \pIsReachK(m, a, b, l)$ \\
	\hline
	$\pIsReachKP : \sMem \times \sAddr \times \sAddr \times \sLevelK
		\times \sSeq$ \\
	$\pIsReachKP(m, a, a, l, \fNil)$ \\
	$m[a].\fNext[l] = a' \land \pIsReachP(m, a', b, l, p)
		\Impl \pIsReachP(m, a, b, l, \fCons(a, p))$ \\
%	\hline
%	$\fFirstMarked : \sMem \times \sSeq \times \sLevelK \times \sAddr$ \\
%	\hline
%	$\fFirstMarked (m, \fNil, l, \fNull)$ \\
%	$p \neq \fNil \land p = \fCons(a, q)
%		\land m[a].\fLockID[l] \neq \oslash
%			\Impl \fFirstMarked(m, p, l, a)$ \\
%	$p \neq \fNil \land p = \fCons(a, q)
%		\land m[a].\fLockID[l] = \oslash
%			\land \fFirstMarked(m, q, l, b)
%				\Impl \fFirstMarked(m, p, l, b)$ \\
%	\hline
	\hline
	$\pOrdPath : \sMem \times \sSeq$ \\
	$\pOrdPath(h, \fNil)$ \\
	$h[a].\fNext[\fLevel{0}] = a' \land h[a].\fKey \pOrd h[a'].\fKey
		\land p = \fCons(a, q) \land \pOrdPath(h, q)
			\Impl \pOrdPath(h, p)$ \\
	\hline
	%\hline
	%$\pContAtLevelK : \sMem \times \sAddr \times \sAddr \times \sLevelK
		%\times \sAddr \times \sAddr \times \sLevelK \times \sSetT$ \\
	%\hline
	%$\begin{pmatrix}
	%\begin{array}{p{2.5em}cp{7em}c}
	%\center$a = U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	%\center$l = 0$ & \land & \center$\contained$
	%\end{array}
	%\end{pmatrix}
		%\Impl \pContAtLevelK(h, L, U, H, a, a, 0, \stSingle{t}) $ \\
	%$\begin{pmatrix}
	%\begin{array}{p{2.5em}cp{7em}c}
	%\center$a = U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	%\center$l = 0$ & \land & \center$\lnot \contained$
	%\end{array}
	%\end{pmatrix}
		%\Impl \pContAtLevelK(h, L, U, H, a, a, 0, \stEmpty)$ \\
	%$\begin{pmatrix}
	%\begin{array}{p{2.5em}cp{7em}c}
	%\center$a = U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	%\center$l > 0$ & \land & \center$\contained$
	%\end{array}
	%\end{pmatrix}
		%\land \pContAtLevelK(h,L,U,H,L,U,l-1,s)
		%\Impl \pContAtLevelK(h, L, U, H, a, a, l-1,
									%s \stCup \stSingle{t})$ \\
	%$\begin{pmatrix}
	%\begin{array}{p{2.5em}cp{7em}c}
	%\center$a = U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	%\center$l > 0$ & \land & \center$\lnot \contained$
	%\end{array}
	%\end{pmatrix}
		%\land \pContAtLevelK(h,L,U,H,L,U,l-1,s)
		%\Impl \pContAtLevelK(h, L, U, H, a, a, l-1, s)$ \\

	%$\begin{pmatrix}
	%\begin{array}{p{2.5em}cp{7em}c}
	%\center$a \neq U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	%\center$a \neq a'$ & \land & \center$\contained$ & \land \\
	%& & \center$h[a].\fNext = a'$
	%\end{array}
	%\end{pmatrix}
		%\land \pContAtLevelK(h,L,U,H,a',b,l,s)
		%\Impl \pContAtLevelK(h, L, U, H, a, b, l,s \stCup \stSingle{t})$\\
	%$\begin{pmatrix}
	%\begin{array}{p{2.5em}cp{7em}c}
	%\center$a \neq U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	%\center$a \neq a'$ & \land & \center$\lnot \contained$ & \land \\
	%& & \center$h[a].\fNext = a'$
	%\end{array}
	%\end{pmatrix}
		%\land \pContAtLevelK(h,L,U,H,a',b,l,s)
		%\Impl \pContAtLevelK(h, L, U, H, a, b, l,s)$\\
	%\hline
\end{tabular}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TSLK PATH Auxiliary functions
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\TSLKPathExtension}{
\renewcommand{\arraystretch}{1.1}
\centering
\begin{array}{l}
	\begin{pmatrix}
	\begin{array}{p{2.5em}cp{7em}c}
	\center$a = U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	\center$l = 0$ & \land & \center$\contained$
	\end{array}
	\end{pmatrix}
		\Impl \pContAtLevelK(h, L, U, H, a, a, 0, \stSingle{t}) \\
	\begin{pmatrix}
	\begin{array}{p{2.5em}cp{7em}c}
	\center$a = U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	\center$l = 0$ & \land & \center$\lnot \contained$
	\end{array}
	\end{pmatrix}
		\Impl \pContAtLevelK(h, L, U, H, a, a, 0, \stEmpty) \\
	\begin{pmatrix}
	\begin{array}{p{2.5em}cp{7em}c}
	\center$a = U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	\center$l > 0$ & \land & \center$\contained$
	\end{array}
	\end{pmatrix}
		\land \pContAtLevelK(h,L,U,H,L,U,l-1,s)
		\Impl \pContAtLevelK(h, L, U, H, a, a, l-1,
									s \stCup \stSingle{t}) \\
	\begin{pmatrix}
	\begin{array}{p{2.5em}cp{7em}c}
	\center$a = U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	\center$l > 0$ & \land & \center$\lnot \contained$
	\end{array}
	\end{pmatrix}
		\land \pContAtLevelK(h,L,U,H,L,U,l-1,s)
		\Impl \pContAtLevelK(h, L, U, H, a, a, l-1, s) \\

	\begin{pmatrix}
	\begin{array}{p{2.5em}cp{7em}c}
	\center$a \neq U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	\center$a \neq a'$ & \land & \center$\contained$ & \land \\
	& & \center$h[a].\fNext = a'$
	\end{array}
	\end{pmatrix}
		\land \pContAtLevelK(h,L,U,H,a',b,l,s)
		\Impl \pContAtLevelK(h, L, U, H, a, b, l,s \stCup \stSingle{t}) \\
	\begin{pmatrix}
	\begin{array}{p{2.5em}cp{7em}c}
	\center$a \neq U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	\center$a \neq a'$ & \land & \center$\lnot \contained$ & \land \\
	& & \center$h[a].\fNext = a'$
	\end{array}
	\end{pmatrix}
		\land \pContAtLevelK(h,L,U,H,a',b,l,s)
		\Impl \pContAtLevelK(h, L, U, H, a, b, l,s)\\
\end{array}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   Translation Examples
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\tslkExampleSkiplist}{
\begin{tabular}{p{14em}>{\hspace{1em}}p{24em}}

\hline
Original term & \TSLK term \\
\hline \\

\begin{array}{c}
	\pOrdList(h, sl, 0)
\end{array} &
\begin{array}{lcl}
	\overbrace{p = \fGetpK(h, \head, \fNull, 0)}^{\sigBridge} & \land &
	   \overbrace{\pOrdList(h,p)}^{\sigBridge}
\end{array} \\\\

\hline \\

\begin{array}{c}
	h[sl].\tail.\fNext[0] = \fNull \\
	\land \cdots \land \\
	h[sl].\tail.\fNext[3] = \fNull \\
\end{array} &
\begin{array}{lcccc}
	\overbrace{c_{\tail} = h[\tail]}^{\sigMemory} & \land &
		\overbrace{a_{\tail_0} = c_{\tail}.\fNext[0]}^{\sigCells} & \land&
		\overbrace{a_{\tail_0} = \fNull}^{\sigAddr} \\
	& \land & \vdots & \land & \vdots \\
	&&	\overbrace{a_{\tail_3} = c_{\tail}.\fNext[3]}^{\sigCells} & \land&
		\overbrace{a_{\tail_3} = \fNull}^{\sigAddr} \\
\end{array} \\\\

\hline

\begin{array}{ll}
	\SubList( h,& sl.\head, sl.\tail, 1, \\
				& sl.\head, sl.\tail, 0) \\
	\multicolumn{2}{c}{\land \cdots \land} \\
	\SubList(h, & sl.\head, sl.\tail, 3, \\
				& sl.\head, sl.\tail, 2) \\
\end{array} &
\begin{array}{cccc}
	\overbrace{p_{\tail_0} = \fGetpK(h, \head, \tail, 0)}^{\sigBridge}
					& \land & \cdots & \land \\
	\overbrace{p_{\tail_3} = \fGetpK(h, \head, \tail, 3)}^{\sigBridge}
					& \land \\
		\overbrace{s_{\tail_0} = \fPathToSet(p_{\tail_0})}^{\sigBridge}
					& \land & \cdots & \land \\
		\overbrace{s_{\tail_3} = \fPathToSet(p_{\tail_3})}^{\sigBridge}
					& \land \\
		\overbrace{s_{\tail_1} \subseteq s_{\tail_0}}^{\sigSets}
					& \land & \cdots & \land \\
		\overbrace{s_{\tail_3} \subseteq s_{\tail_2}}^{\sigSets}
\end{array} \\\\
\hline
\end{tabular}
}



\newcommand{\tslkExamplePreconditions}{
\begin{tabular}{p{11.5em}>{\hspace{1em}}p{26.3em}}

\hline
Original term & \TSLK term \\
\hline \\

\begin{array}{c}
	x.\fKey = \newval
\end{array} &
\begin{array}{ccc}
	\overbrace{c_x = h[x]}^{\sigMemory} & \land &
	   \overbrace{c_x.\fKey = \newval}^{\sigCells}
\end{array} \\\\

\hline \\

\begin{array}{c}
	\prev.\fKey < \newval
\end{array} &
\begin{array}{cccc}
	\overbrace{c_{\prev} = h[\prev]}^{\sigMemory} & \land &
	\overbrace{c_{\prev}.\fKey = k_{\prev}}^{\sigCells} & \land \\
	\overbrace{k_{\prev} \pOrd \newval}^{\sigOrd} & \land &
	\overbrace{k_{\prev} \neq \newval}^{\sigOrd}
\end{array} \\\\

\hline \\

\begin{array}{c}
	\prev.\fNext[i].\fKey > \newval
\end{array} &
\begin{array}{cccc}
	\overbrace{a_{\fNext} = c_{\prev}.\fNext[i]}^{\sigCells} & \land &
	\overbrace{c_{\fNext} = h[a_{\fNext}]}^{\sigMemory} & \land \\
	\overbrace{k_{\fNext} = c_{\fNext}.\fKey}^{\sigCells} & \land \\
	\overbrace{\newval \pOrd k_{\fNext}}^{\sigOrd} & \land &
	\overbrace{\newval \neq k_{\fNext}}^{\sigOrd}
\end{array} \\\\

\hline \\

\begin{array}{c}
	\prev.\fNext[i] = x.\fNext[i]
\end{array} &
\begin{array}{ccc}
	\overbrace{a_{\fNext_x} = c_x.\fNext[i]}^{\sigCells} & \land &
	\overbrace{a_{\fNext} = a_{\fNext_x}}^{\sigAddr}
\end{array} \\\\

\hline \\

\begin{array}{c}
	\prev.\fLockID[i] = j
\end{array} &
\begin{array}{ccc}
	\overbrace{t_{\prev} = c_{\prev}.\fLockID[i]}^{\sigCells} & \land &
	\overbrace{t_{\prev} = j}^{\sigThId}
\end{array} \\\\

\hline \\

\begin{array}{c}
	x.\fNext[i].\fLockID[i] = j
\end{array} &
\begin{array}{cccc}
	\overbrace{c_{\fNext_x} = h[a_{\fNext_x}]}^{\sigMemory} & \land &
	\overbrace{t_{\fNext_x} = c_{\fNext_x}.\fLockID[i]}^{\sigCells}
			& \land \\
	\overbrace{t_{\fNext_x} = j}^{\sigThId}
\end{array} \\\\

\hline \\

\begin{array}{c}
	(x,i) \notin r
\end{array} &
\begin{array}{ccccc}
	\overbrace{\empty = \mrgnEmpty}^{\sigMrgn} & \land &
	\overbrace{x_{i_{\mathit{set}}} = \mrgnSingle{x,i}}^{\sigMrgn}
			& \land &
	\overbrace{\empty = r \mrgnCap x_{i_{\mathit{set}}}}^{\sigMrgn}
\end{array} \\\\

\hline \\

\begin{array}{c}
	0 \leq i \leq 3
\end{array} &
\begin{array}{l}
	\text{We must generate four different scenarios to be} \\
	\text{combined with the conjunction of the remaining literals.}\\
	\text{These scenarios are:} \\
	\begin{array}{c>{\hspace{1em}}ccc>{\hspace{3em}}c>{\hspace{1em}}ccc}
	1. & \overbrace{0 < i}^{\sigLevelK} & \land &
		\overbrace{i < 3}^{\sigLevelK} &
	3. & \overbrace{0 = i}^{\sigLevelK} & \land &
		\overbrace{i < 3}^{\sigLevelK} \\
	2. & \overbrace{0 < i}^{\sigLevelK} & \land &
		\overbrace{i = 3}^{\sigLevelK} &
	4. & \overbrace{0 = i}^{\sigLevelK} & \land &
		\overbrace{i = 3}^{\sigLevelK} \\
	\end{array}
\end{array} \\\\

\hline
\end{tabular}
}


\newcommand{\tslkExampleTransformation}{
\begin{tabular}{p{15.5em}>{\hspace{1em}}p{22em}}

\hline
Original term & \TSLK term \\
\hline \\

\begin{array}{c}
	\AT_{43}^{[j]} \land {\AT'}_{44}^{[j]}
\end{array} &
\begin{array}{ccccccc}
	\overbrace{\AT_{j_{43}}}^{\sBool} & \land &
	\overbrace{\lnot \AT_{j_{44}}}^{\sBool} & \land &
	\overbrace{{\lnot \AT'}_{j_{43}}}^{\sBool} & \land &
	\overbrace{{\AT'}_{j_{44}}}^{\sBool}
\end{array} \\\\

\hline \\

\begin{array}{c}
	\prev'.\fNext[i] = x
\end{array} &
\begin{array}{ccc}
	\overbrace{a_{\fNext_{\new}} = c_{\prev_{\new}}.\fNext[i]}^{\sigCells}
			& \land &
	\overbrace{a_{\fNext_{\new}} = x}^{\sigAddr}
\end{array} \\\\

\hline \\

\begin{array}{c}
	\prev'.\fKey = \prev.\fKey
\end{array} &
\begin{array}{ccc}
	\overbrace{k_{\prev_{\new}} = c_{\prev_{\new}}.\fKey}^{\sigCells}
			& \land &
	\overbrace{k_{\prev} = k_{\prev_{\new}}}^{\sigOrd}
\end{array} \\\\

\hline \\

\begin{array}{c}
	\prev'.\fData = \prev.\fData
\end{array} &
\begin{array}{cccc}
	\overbrace{e_{\prev} = c_{\prev}.\fData}^{\sigCells}
			& \land &
	\overbrace{e_{\prev_{\new}} = c_{\prev_{\new}}.\fData}^{\sigCells}
			& \land \\
	\overbrace{e_{\prev} = e_{\prev_{\new}}}^{\sigElem}
\end{array} \\\\

\hline \\

\begin{array}{c}
	\prev'.\fNext[0] = \prev.\fNext[0] \\
	\land \cdots \land \\
	\prev'.\fNext[i-1] = \prev.\fNext[i-1] \\
	\land \\
	\prev'.\fNext[i+1] = \prev.\fNext[i+1] \\
	\land \cdots \land \\
	\prev'.\fNext[3] = \prev.\fNext[3]
\end{array} &
\begin{array}{cccc}
	\overbrace{a_{\prev_0} = c_{\prev}.\fNext[0]}^{\sigCells}
			& \land & \cdots & \land \\
	\overbrace{a_{\prev_{i-1}} = c_{\prev}.\fNext[i-1]}^{\sigCells}
			& \land \\
	\overbrace{a_{\prev_{i+1}} = c_{\prev}.\fNext[i+1]}^{\sigCells}
			& \land & \cdots & \land \\
	\overbrace{a_{\prev_{3}} = c_{\prev}.\fNext[3]}^{\sigCells}
			& \land \\
	\overbrace{a_{\prev_{\new_0}}
				= c_{\prev_{\new}}.\fNext[0]}^{\sigCells}
			& \land & \cdots & \land \\
	\overbrace{a_{\prev_{\new_{i-1}}}
				= c_{\prev_{\new}}.\fNext[i-1]}^{\sigCells}
			& \land \\
	\overbrace{a_{\prev_{\new_{i+1}}}
				= c_{\prev_{\new}}.\fNext[i+1]}^{\sigCells}
			& \land & \cdots & \land \\
	\overbrace{a_{\prev_{\new_{3}}}
				= c_{\prev_{\new}}.\fNext[3]}^{\sigCells}
			& \land \\
	\overbrace{a_{\prev_{\new_0}} = a_{\prev_0}}^{\sigAddr}
			& \land & \cdots & \land \\
	\overbrace{a_{\prev_{\new_{i-1}}} = a_{\prev_{i-1}}}^{\sigAddr}
			& \land \\
	\overbrace{a_{\prev_{\new_{i+1}}} = a_{\prev_{i+1}}}^{\sigAddr}
			& \land & \cdots & \land \\
	\overbrace{a_{\prev_{\new_{3}}} = a_{\prev_{3}}}^{\sigAddr}
			& \land \\
	\overbrace{h' = \fUpd(h, \prev, c_{\prev_{\new}})}^{\sigMemory}
\end{array} \\\\

\hline
\end{tabular}
}


\newcommand{\lukSignature}{
\begin{array}{lclllcll}
	\sigPair & = & \big( & \{ & \multicolumn{3}{l}{ \sPair, \sThId} & \}, 
			\\
			& & & \{ & \fPair{\_}{\_} &:& \sThId \times \sThId \to\sPair\\
			& & & \{ & & & & \} \; \big) \\ \\
	\sigSetPair & = & \big( & \{ & \multicolumn{3}{l}{\sSetPair, \sPair} & 
			\}, \\
			& & & \{ & \spEmpty & : & \sSetPair, 						\\
			& & &    & \spSingle{\_} & : & \sPair \to \sSetPair,		\\
			& & &    & \spCup & : & \sSetPair \times \sSetPair
						\to \sSetPair,									\\
			& & &    & \spCap & : & \sSetPair \times \sSetPair
						\to \sSetPair,									\\
			& & &    & \spSubst & : & \sSetPair \times \sSetPair
						\to \sSetPair							  & \},	\\

			& & & \{ & \spIn & : & \sPair \times \sSetPair				\\
			& & & 	 & \spSubset & : & \sSetPair \times \sSetPair & \}
			\; \big) \\ \\
	\sigLUK & = & \big( & \{ & \multicolumn{3}{l}{
				\sMem, \sAArray, \sLArray, \sThId, \sSetT,
				\sPair, \sSetPair} & \}, \\
			& & & \{ & \fLUKSubset & : &
				\sMem \times \sAArray \times \sAArray \times \sLArray 
					\times \sAddr \times \sAddr \times \sLevelK
					\to \sSetT \\
			& & &	 & \fInterLUK & : &
				\sMem \times \sAArray \times \sAArray \times \sLArray 
					\times \sSetT \to \sSetPair \\
			& & &	 & \fEmptyLUK & : &
				\sMem \times \sAArray \times \sAArray \times \sLArray 
					\times \sAddr \times \sAddr \times \sLevelK
					\to \sSetT \\
			& & &	 & \fMinLUK & : &
				\sMem \times \sAArray \times \sSetT \to \sThId	& \} \\
			& & & \{ & & & & \} \; \big) \\
\end{array}
}

\newcommand{\lukInterpretation}{
\begin{array}{rcl>{\hspace{-0.5em}}l>{\hspace{-0.5em}}c>{\hspace{-0.2em}}cclll}
\inter{\fLUKSubset}{\Ai}(m,L,U,H,a_1,a_2,l) & = &
		& \big\{ &
			t' & \in & \Ais{\sThId} &|&
				a_1 \leq L(t') \text{ and } U(t') \leq a_2 \text{ and } \\
		&&&&&&&&	(H(t') < l \text{ or } H(t') = l) & \big\} \\ \\

\inter{\fInterLUK}{\Ai}(m,L,U,H,g) & = &
		& \big\{ &
			\fPair{t_1}{t_2} & \in & \Ais{\sPair} &|&
				t_1 \in g \text{, } t_2 \in g \text{, } \\
		&&&&&&&&	\intersects(t_1, t_2) \text{ and } t_1 \neq t_2
		& \big\} \\ \\

\inter{\fEmptyLUK}{\Ai}(m,L,U,H,a_1,a_2,l) & = &
		& \big\{ &
			t' & \in & \Ais{\sThId} &|&
				t' \in \inter{\fLUKSubset}{\Ai}(m,L,U,H,a_1,a_2,l) \\
		&&&& \multicolumn{5}{l}{
				\text{and }
					\inter{\fLUKSubset}{\Ai}(m,L,U,H,L(t'),U(t'),H(t'))
					= \emptyset}
		& \big\} \\ \\

\inter{\fMinLUK}{\Ai}(m,U,g) & = &
		\multicolumn{8}{l}{
		\left\{\begin{array}{>{\hspace{0.3em}}l>{\hspace{2em}}l}
				\oslash & \text{if } g = \emptyset \\
				t_i & \text{if } g = \{t_1, \ldots, t_q\} \text{, }
					i \in 1..q \text{ and} \\
				& \hspace{1em} \text{forall } j \in 1..q \;
					U(t_j) \leq U(t_i)
		\end{array}\right.}
\end{array}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TSL Signature - Table
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\TSLSignature}{
\centering
\begin{tabular}{r>{\vspace{-.5\baselineskip}}p{9cm}}
\hline
\textbf{Signature:} & \sigLevel \\
\textbf{Sorts:} & \sLevel \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			$0$ & : & \sLevel \\
			$s$ & : & \sLevel \to \sLevel \\
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			$<$  & : & \sLevel \times \sLevel \\
			\end{array} \\
\hline
%\textbf{Signature:} & \sigOrd \\
%\textbf{Sorts:} & \sOrd \\
%\textbf{Functions:} &
%			\begin{array}{p{2cm}cl}
%				\fZero & : & \sOrd \\
%				\fInfty & : & \sOrd \\
%			\end{array} \\
%\textbf{Predicates:} &
%			\begin{array}{p{2cm}cl}
%			\pOrd	& : & \sOrd \times \sOrd \\
%			\end{array} \\
%\hline
\textbf{Signature:} & \sigArray \\
\textbf{Sorts:} & \sArray, \sLevel, \sAddr \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\fArrayRd{\_}{\_} &:& \sArray \times \sLevel \to \sAddr \\
			\fArrayUpd{\_}{\_}{\_} & : &
				\sArray \times \sLevel \times \sAddr \to \sArray \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigCells \\
\textbf{Sorts:} & \sCell, \sElem, \sOrd, \sArray, \sAddr, \sLevel \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\fError & : & \sCell \\
			\fMkcell & : & \sElem \times \sOrd \times \sArray \times \sLevel
												\to \sCell \\
			$\_.\fData$ & : & \sCell \to \sElem \\
			$\_.\fKey$ & : & \sCell \to \sOrd \\
			$\_.\fArr$ & : & \sCell \to \sArray \\
			$\_.\fMax$ & : & \sCell \to \sLevel \\
			\end{array} \\
\hline
%\textbf{Signature:} & \sigMemory \\
%\textbf{Sorts:} & \sMem, \sAddr, \sCell \\
%\textbf{Functions:} &
%			\begin{array}{p{2cm}cl}
%			\fNull & : & \sAddr \\
%			\fRd & : & \sMem \times \sAddr \to \sCell \\
%			\fUpd & : & \sMem \times \sAddr \times \sCell \to \sMem
%			\end{array} \\
%\hline
\textbf{Signature:} & \sigReach \\
\textbf{Sorts:} & \sMem, \sAddr, \sPath \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\fEpsilon & : & \sPath \\
			\lbrack \_ \rbrack & : & \sAddr \to \sPath
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			\pAppend & : & \sPath \times \sPath \times \sPath \\
			\pReach & : & \sMem \times \sAddr \times \sAddr \times \sLevel
											\times \sPath \\
			\end{array} \\
\hline
%\textbf{Signature:} & \sigSets \\
%\textbf{Sorts:} & \sAddr, \sSet \\
%\textbf{Functions:} &
%			\begin{array}{p{2cm}cl}
%			$\emptyset$ & : & \sSet \\
%			$\{ \_ \}$ & : & \sAddr \to \sSet \\
%			$\cup$, $\cap$, $\setminus$ & : & \sSet \times \sSet \to \sSet
%			\end{array} \\
%\textbf{Predicates:} &
%			\begin{array}{p{2cm}cl}
%			\pAppend & : & \sPath \times \sPath \times \sPath \\
%			\pReach & : & \sMem \times \sAddr \times \sAddr \times \sLevel
%											\times \sPath \\
%			\end{array} \\
%\hline
\textbf{Signature:} & \sigBridge \\
\textbf{Sorts:} & \sMem, \sAddr, \sSet, \sPath, \sLevel\\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\fPathToSet & : & \sPath \to \sSet \\
			\fAddrToSet & : & \sMem \times \sAddr \times \sLevel
				\to \sSet \\
			\fGetp & : & \sMem \times \sAddr \times \sAddr \times
				\sLevel \to \sPath \\
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			\pOrdList & : & \sMem \times \sPath \\
			\pSkiplist & : & \sMem \times \sSet \times \sLevel \times \sAddr
												\times \sAddr \\
			\end{array} \\
\hline
\end{tabular}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TSL Interpretations
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\TSLInterpretations}{
\centering
\begin{tabular}{p{11cm}}
\hline \\
\textbf{Signature:} $\sigLevel$ \\
\textbf{Interpretations:} \\
  \hspace{1.5em}
  \begin{tabular}{p{10cm}}
		\begin{compactitem}
			\item $\inter{0}{\Ai} = 0$
			\item $\inter{s}{\Ai}(l) = s(l)$
		\end{compactitem} \\
		for each
			$l \in \Ais{\sLevel}$ \\
	\end{tabular} \\ \\
\hline \\
\textbf{Signature:} $\sigArray$ \\
\textbf{Interpretations:} \\
  \hspace{1.5em}
  \begin{tabular}{p{10cm}}
		\begin{compactitem}
			\item $\fArrayRdInter{A}{l}{\Ai} = A(l)$
			\item $\fArrayUpdInter{A}{l}{a}{\Ai} = A_{\mathit{new}}$, where
				$A_{\mathit{new}}(l) = a$ and
				$A_{\mathit{new}}(i) = A(i)$ for $i \neq l$
		\end{compactitem} \\
		for each
			$A, A_{\mathit{new}} \in \Ais{\sArray}$,
			$l \in \Ais{\sLevel}$ and
			$a \in \Ais{\sAddr}$ \\
	\end{tabular} \\ \\
\hline \\
\textbf{Signature:} $\sigCells$ \\
\textbf{Interpretations:} \\
	\hspace{1.5em}
  \begin{tabular}{p{10cm}}
		\begin{compactitem}
		\item $\inter{\fMkcell}{\Ai} (e, k, \vect{a}, l) =
						\langle e, k, A, l \rangle$
		\item $\inter{\fError}{\Ai}.\inter{\fArr}{\Ai}(l) = \inter{\fNull}{\Ai}$
		\item $\langle e, k, A, l \rangle.\inter{\fData}{\Ai} = e$
		\item $\langle e, k, A, l \rangle.\inter{\fKey}{\Ai} = k$
		\item $\langle e, k, A, l \rangle.\inter{\fArr}{\Ai} = A$
		\item $\langle e, k, A, l \rangle.\inter{\fMax}{\Ai} = l$
		\end{compactitem} \\
		for each
			$e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$A \in \Ais{\sArray}$,
			and $l \in \Ais{\sLevel}$ \\
	\end{tabular} \\ \\
\hline \\
\textbf{Signature:} $\sigReach$ \\
\textbf{Interpretations:} \\
	\hspace{1.5em}
  \begin{tabular}{p{10cm}}
		\begin{compactitem}
		\item $(m, \aInit, \aEnd, l, p) \in \inter{\pReach}{\Ai}$
			iff $\aInit=\aEnd$ and $p = \fEpsilon$, or
		there exist addresses $a_1, \ldots, a_n \in \Ais{\sAddr}$ such 
		that:
		\end{compactitem} \\
		\hs{1.4} $\begin{array}{ll}
			\trm{(a) } p = [a_1\,..\,a_n]  \phantom{aaaa}&
			\trm{(c) } m(a_r).\inter{\fArr}{\Ai}(l)
				= a_{r+1}, \;\;\;\text{for}\;\;\;r < n \\
			\trm{(b) } a_1 = \aInit &
			\trm{(d) } m(a_n).\inter{\fArr}{\Ai}(l)
				= \aEnd
		\end{array}$ \\
	\end{tabular} \\ \\
\hline \\
\textbf{Signature:} $\sigBridge$ \\
\textbf{Interpretations:} \\
	\hspace{1.5em}
	\begin{tabular}{p{10cm}}
		\begin{compactitem}
		\item $\inter{\fAddrToSet}{\Ai}(m, a, l)
					= \big\{a' \in \Ais{\sAddr} | \exists p \in \Ais{\sPath}$ .  
						$(m,a,a',l,p) \in \pReach
						\big\}$
		\item $\inter{\fGetp}{\Ai}(m,a_i,a_e,l) =
			\begin{cases}
				p & \text{if } (m,a_i,a_e,l,p)
					\in \inter{\pReach}{\Ai} \\
				\fEpsilon & \text{otherwise}
			\end{cases}$
		\item $\inter{\pSkiplist}{\Ai}(m, r, l, a_i, a_e)$ iff
				$\begin{bmatrix}
					\begin{array}{cl}
						\inter{\pOrdList}{\Ai}(m, \inter{\fGetp}{\Ai}(m, a_i, a_e, 0))
								& \land \\
						r = \inter{\fPathToSet}{\Ai}(\inter{\fGetp}{\Ai}(m,a_i,a_e,l)) & \land \\
						0 \leq l \land
						\forall a \in r \;.\;
							m(a).\inter{\fMax}{\Ai} \leq l & \land \\
						m(a_e).\inter{\fArr}{\Ai}(l) = \inter{\fNull}{\Ai}
							& \land \\
						\big( 0 = l_{\fMax} \big) \; \lor \\
							\big(\exists l_p \;.\; \inter{s}{\Ai}(l_p) = l \land
								\;\forall\; i \in 0, \ldots, l_p \;.\; \\
								\hspace{1em} m(a_e).\inter{\fArr}{\Ai}(i)
									= \inter{\fNull}{\Ai} \; \land \\
								\hspace{1em}
									\inter{\fPathToSet}{\Ai}(
										\inter{\fGetp}{\Ai}(m, a_i, a_e,
											\inter{s}{\Ai}(i))) \subseteq \\
								\hspace{2em} \inter{\fPathToSet}{\Ai}(
										\inter{\fGetp}{\Ai}(m, a_i, a_e, i)) \big)
					\end{array}
				\end{bmatrix}$
		\end{compactitem} \\
		for each
      $m \in \Ais{\sMem}$,
			$p \in \Ais{\sPath}$,
			$r \in \Ais{\sSet}$,
			$l \in \Ais{\sLevelK}$
			and $a, a_i, a_e \in \Ais{\sAddr}$ \\
	\end{tabular} \\ \\
\hline \\

\end{tabular}
}



==> missing.tex <==
\section{Missing proofs}
\label{sec:app:missing}

\newcounter{backup}

\setcounter{backup}{\value{theorem}}
\setcounter{theorem}{\value{thm-convergence}}

\begin{theorem}
  All of the following hold for every instant variable $u[k]$:
  \begin{compactenum}
  \item[\textup{(1)}] If $\ISLAZY(u)$ then all request messages for $u[k]$
    are eventually responded.
    \item[\textup{(2)}] If $\ISEAGER(u)$ then a response message for
      $u[k]$ is eventually sent.
    \item[\textup{(3)}] The value of $u[k]$ is eventually resolved.
    \item[\textup{(4)}] The value of $u[k]$ is $c$ if and only if $(u[k],c)\in R$ at
      some instant.
  \end{compactenum}
\end{theorem}


\setcounter{theorem}{\value{backup}}

\begin{proof}
  Let $M$ be a length of a computation and $\sigma_I$ be an input of
  length $M$.
%
  Note that $(1)$ to $(4)$ above are all statements about instant
  variables $u[k]$, which are the nodes of the evaluation graph
  $G_{\varphi,M}$.
%
  We proceed by induction on $G_{\varphi,M}$ (which is acyclic because
  $D_\varphi$ is well-formed).
%
  \begin{itemize}
  \item \textbf{Base case}: The base case are vertices of the
    evaluation graph that have no outgoing edges, which are either
    instant variables that correspond to inputs or to defined
    variables whose instant equation does not contain other instant
    variables.
    %
    Statement $(3)$ follows immediately for inputs because at instant
    $k$, $s[k]$ is read at node $\mu(k)$.
    % 
    For output equations that do not have variables, or whose
    variables have offsets that once instantiated become negative or
    greater than $M$, the value of its leafs is determined either
    immediately or at $M$ when the offset if calculated.
    %
    At this point, the value computed is inserted in $R$, so $(4)$
    also holds at $\mu(u)$.
    % 
    Note that $(4)$ also holds for other nodes because the response
    message contains $u[k]=c$ if and only if $(u[k],c)\in R_n$, where
    $\mu(u)=n$.
    %
    If $s$ is eager, then the response message is inserted exactly at
    the point it is resolved, so $(3)$ implies $(2)$.
    %
    Finally, $(1)$ also holds at the time of receiving the request
    message or resolving $u[k]$ (whatever happens later).
%
  \item \textbf{Inductive case}: Consider an arbitrary $u[k]$ in the
    evaluation graph $G_{\varphi,M}$ and let
    $u_1[k_1],\ldots,u_l[k_l]$ the instant variables that $u[k]$
    depends on.
    % 
    These are nodes in $G_{\varphi,M}$ that are lower than $u[k]$ so
    the inductive hypothesis applies, and $(1)$-$(4)$ hold for these.
    %
    Let $n=\mu(u)$.
    %
    At instant $k$, $u[k]$ is instantiated and inserted in $U_n$. 
    %
    At the end of cycle $k$, lazy variables among $u_1[l_1]\ldots
    u_l[ul]$ are requested.
    %
    By induction hypothesis, at some instant all these requests are
    responded by $(1)$.
    %
    Similarly, the values of all eager variables are calculated and
    sent as well (by $(2)$ and $(3)$).
    %
    At the latest time of arrival, the equation for $u[k]$ has no more
    variables and it is evaluated to a value, so $(3)$ holds and $(4)$
    holds at $n$.
    %
    At this point, if $\ISEAGER(u)$ then the response message is sent
    (so $(2)$ holds for $u[k]$) and if $\ISLAZY(u)$ then all requests
    (previously received in $\PEN_n$ or future requests) are answered,
    so $(1)$ also holds.
  \end{itemize}
%
  This finishes the proof.
  \qed
\end{proof}

\setcounter{backup}{\value{theorem}}
\setcounter{theorem}{\value{thm-correctness}}

\begin{theorem}
  %\label{thm:correctness}
  Let $\varphi$ be a specification, $S:\tupleof{\varphi,\topo,\mu}$ be
  a decentralized SRV problem, and $\sigma_I$ an input.
  %
  Then $(\sigma_I,\OUTPUT(\sigma_I))\models \varphi$.
\end{theorem}

\setcounter{theorem}{\value{backup}}

\begin{proof}
  Let $\sigma_O$ be the unique evaluation model such that
  $(\sigma_I,\sigma_O)\models \varphi$ (we use $\sigma_O(s)$ for the
  output stream for stream variable $s$ and $\sigma_O(s)(k)$ for its
  value in the $k$-th position).  
%
  We need to show that for every $s$ and $k$,
  $\Osem{s}(k)=\sigma_O(s)(k)$.
%
  We again proceed by induction on the evaluation graph $G_{\varphi,M}$.
  %
  \begin{itemize}
  \item \textbf{Base case:}
    For inputs the value follows immediately. 
    % 
    The other basic case corresponds to output variables $s$ at
    instants at which these that do not depend on other variables
    (because all occurrences of offsets, if any, fall off the trace).
    %
    The evaluation of the value is performed by $\mu(s)$, and it
    satisfies the equation $e_s$ of $s$, not depending on any value of
    any other stream. 
    %
    Therefore, it satisfies that $\Osem{s}(k)=\sem{e_s[k]}=\sigma_O(s)(k)$,
    as desired
  \item \textbf{Inductive case:} 
%
    Let $s$ be an arbitrary stream variable and $k$ an arbitrary
    instant within $0$ and $M-1$ and assume that all instant variables
    $u[k']$ that $s[k]$ can reach in the evaluation graph satisfy the
    inductive hypothesis.
    %
    Let $n$ be the node in charge of computing $s$.
    %
    By Theorem~\ref{thm:convergence}, all the values are eventually
    received by $n$ and in $R_n$, and by IH, these values are the same
    as in the denotational semantics, that is
    $\Osem{u}(k')=\sigma_O(u)(k')$.
    %
    The evaluation of $s[k]$ corresponds to computing $\sem{e_s}$,
    which uses the semantics of the expression (according to
    Section~\ref{sec:lola}).
    %
    A simple structural induction on the expression $e_s$ shows that
    the result of the evaluation, that is the value assigned to
    $s[k]$, is $\sem{e_s}_{\sigma}(k)=\sigma_O(s)(k)$, as desired.
  \end{itemize}
  This finishes the proof.
  \qed
\end{proof}



%
% OLD MISSING PROOFS
%

% \section{Missing Proofs}
% \label{sec:app:proofs}



% % Cesar: commented because I erase this lemma from the main body
% %\setcounter{backup}{\value{lemma}}
% %\setcounter{lemma}{\value{lem-L4}}

% \begin{lemma}[Every message arrives]
%   Let $m\ =\ (req,\ \si,\ V_s,\ V_d)\ or\ m'\ =\ (res,\ \si,\ c,\ V_s,\ V_d)\ \in\ Q_v$ for some node $V$ and time $t$.\\
%   then $M\ \in\ Q_{V_{d_{t'}}}$ for some $t'\ =\ t\ +\ k$ where $h$ is the height of $\si$ in $\varphi$ and \\
%   $k\ =\ len(l)$ and $l\ =\ RT_v(V_s,\ V_d)$ \\
% \end{lemma}

% \begin{proof}
%   By Induction on l:
%   \paragraph{Base case:}
%   \begin{align*}
%     k\ &=\ 0\\
%     RT_V (V_s,\ V_d)\ =\ (V_x,\ 0,\ [])\ &\produce\ V_x\ =\ V\ \And\ m\ \in\ Q_V\ \And\ t'\ =\ t
%   \end{align*}
%   \paragraph{IH}
%   $m\ \in\ Q_{V_{dt'}}\ \And\ t'\ =\ t\ +\ k,\ k\ =\ len(RT_v(V_s,\ V_d))$
%   \begin{align*}
%     Proof\ for\ k\ +\ 1\ &=\ len(RT_v(V_1,\ V_d)),\\
%     RT_v(V_1,\ V_d)\ =\ V_y\ :\ l\\
%     RT_V\ (V_s,\ V_d)\ &=\ (V_x,\ k\ +\ 1,\ V_y\ :\ l)\\
%     where\ l\ &=\ U_1\ :\ [U_2, ..., U_k]\\
%     \produce\\
%     m\ \in\ Q_{V_yt'}\ &t'\ =\ t\ +\ 1\ By\ \ref{Ph1},\ IH\\
%     RT_V(V_s,\ V_d)\ &=\ (V_1,\ k,\ l)\ By\ Fact1\\
%     \produce\\
%     m_2\ \in\ &Q_{V_dt"}\ t"\ =\ t'\ +\ k\ By\ IH\\
%     then\quad t"\ &=\ t'\ +\ k\ =\ t\ +\ k\ +\ 1\\
%   \end{align*}
% %
%   This finishes the proof.
% %  
%   \qed
% \end{proof}

% %\setcounter{lemma}{\value{backup}}

% \setcounter{backup}{\value{lemma}}
% \setcounter{lemma}{\value{lem-acyclic-eval-graph}}

% \begin{lemma}
%   \label{lem:acyclic-eval-graph}
%   Let $\varphi$ be a spec $G_{\varphi}$ a dependency graph and (V,E an Evaluation Graph for [0..N]) then (V, E ) is acyclic.
%   This is an acyclic directed graph (unweighted).\\
%   Consequently, every node $s[n]$ has a longest finite path.\\
% \end{lemma}
% \begin{proof}
%   By contradiction.
%   Suppose there is a cycle, then there must be a SCC in the dependency graph of weight 0.\\
%   But we do not allow 0 weighted cycles for well-formed specifications in the dependency graph, as in \cite{lola}. So this is a contradiction.
% \end{proof}

% \setcounter{lemma}{\value{backup}}

% \setcounter{backup}{\value{theorem}}
% \setcounter{theorem}{\value{thm-convergence}}
% \begin{theorem} [Convergence V]
%   \label{thm:convergence}
%   Every request produces a response\\
%   and\\
%   Every $\si_t$ is eventually resolved\\
%   and\\
%   Every time a response is sent $\Impl$ $\si_t$ is resolved to $c$, $(\si_t, c)\ \in R_v$\\
%   Formally:\\
%   Let $s_t$ be a stamped stream and let $V = \de(s)$\\
%   Let $V_{src}$ be an arbitrary node and\\
%   \paragraph{(1)}  let $\{req, s_t, V_{src}, V\}$ be a msg in state $\Si_t$\\
%   then, for some $t' > t$ there is a $c$ and a msg $\{res, s_t, c, V, V_{src}\}$ in state $\Si_{t'}$\\
%   \paragraph{(2)} Also, for every $t"$ for which $s_t \in U_V$ there is $t''' > t"$ for which $s_t \in R_V$\\
%   The proof will be done by structural induction, thus, a well-ordering is defined over $\rho$:\\
% \end{theorem}
% \begin{proof}
%   By induction on $\rho$
%   \paragraph{(1)}  Let us show that (1) holds for inputs:\\
%   Let $(req,\ i_{i}[t-x_i],\ V_s,\ V)\ \in\ Q_V[t']$ and $\de(i_i) = V,\ x_i\ \in\ \Int $By \ref{L4}\\
%   $\rho(i_i[n]) = 0$
%   As it is an input, $i_{i}[t-x_i]\ \in\ R_V[t"]\, t" = t-x_i$ By line 17\\
%   Then $(res,\ i_{i}[t-x_i],\ v_i,\ V,\ V_s)$ will be sent by line 20\\
%   Then $(res,\ i_{i}[t-x_i],\ v_i,\ V,\ V_s)\ \in\ Q_{V_s}[t'''] $ by \ref{L4}  
  
%   \paragraph{Base case $\rho(s_i[n]) = 0$}
%   Proof (2) holds:\\
%   $s[t]\ =\ f\ (s[t-y|d],\ i_1[t-x_1|d],...,\ i_i[t-x_i|d],\ r_{1}[t-k_{1}|d_1],..., \ r_{j}[t-k_{j}|d_j])$\\
%   As $\rho(s[t]) = 0$ then $\rho(r_1) = ... = \rho(r_{j}[t-k_{j}|d_j]) = 0$\\
%   But $s[t]$ can only depend on subexpressions $r_1, ..., r_j$ such that \\
%   $r_{1}[t-k_{1} | d_1],..,\ r_{j}[t-k_{j} | d_j] < s[t]$ in the given well-founded order.\\
%   Thus, they are either inputs or streams whose all subexpressions are simplified to default values, to comply with the order.\\
%   Those that will be simplified are those that meet $t+k < 0\ or\ t+k > N$ 
%   Then $\ r_{1}[t-k_{1} | d_1],..., \ r_{j}[t-k_{j} | d_j] = d_1, ..., d_j$ By line 19\\
%   Note that V need not send messages to know the default values $d_1, ..., d_j$\\\
%   If an input it is resolved in V\\
%   $i_1[t-x_1],...,\ i_i[t-x_i]\ \in\ R_{v}[t"]$ by line 17\\
%   If it is resolved to default values $s[t]$ is resolved, so:\\
%   $s[t]\ \in\ R_V[t"]$ By line 19\\
%   (2) holds.
  
%   Proof (1) holds based on (2) holds:\\
%   let $msg =(req, s[t], V, V_s),\ \de(s) = V_s,\ msg\ \in\ Q_{V_s}[t'],\ t' <= t + d$ by \ref{L4}\\
%   and $h(s) = 0$\\
%   Then $s[t]$ is resolved at some time in the future\\
%   $s[t]\ \in R_{V_s}[t"] t" > t'$ By (2)\\
%   Then a response is sent back to $V$\\
%   $(res, s[t],v, V_s, V)$ By line 20\\
%   which is received at $t'''$\\
%   $(res, s[t],v, V_s, V) \in Q_V[t'''],\ t''' <= t" + d$ By \ref{L4}\\
%   (1) and (2) hold for base case.\\
  
%   \paragraph{IH :$\rho(r[n]) < \rho(s[n])$}  
%   Assuming $\rho(r[n]) < \rho(s[n])$ for an arbitrary $t$\\
%   Prove (2) assuming (1) for $\rho(r[n]) < \rho(s[n]$\\
%   let $s[t]\ =\ f\ (s[t-y],\ i_1[t-x_1],...,\ i_i[t-x_i],\ r_{1}[t-k_{1} | d_1],..., \ r_{j}[t-k_{j} | d_j])$\\
%   And considering \\
%   $x_{1..i}\ \in\ \Int$\\
%   $k_{1..j}\ \in\ \Int$\\
%   $y\ \in\ \Nat$\\
%   $r_{1..j} < s[t]$ in the above specified order\\
%   Then requests are sent to the other nodes $(req, r_{1}[t-k_{1} | d_1],..., \ r_{j}[t-k_{j} | d_j], V, V_{1..j})$ By line 21\\
%   Those requests produce responses that return\\
%   $(res, r_{1}[t-k_{1} | d_1],..., \ r_{j}[t-k_{j} | d_j],c_1, ..., c_j, V_{1..j}, V)\ \in\ Q_V[t"] by (1)$\\
%   So, both subexpressions and inputs are resolved waiting enough:\\
%   $(r_{1..j}, c_{1..j})\ \in\ R_V[t"]$\\
%   $(i_{1..i}, v_{1..i})\ \in\ R_V[t'''],\ t''' = t + max_{i=1..i}(t-x_i)$\\
%   So, s[t] is resolved eventually in the future\\
%   $s[t]\ \in\ R_V[t^{IV}],\ t^{IV} = max(t", t''') = max (t", t + max_{i=1..i}(t-x_i))$\\
%   (2) holds.\\
  
%   Proof (1) assuming (2) h,t\\
%   Let $msg = (req, s[t],V, V_s)\ \in\ Q_{V_s}$ By \ref{L4}\\
%   let   $s[t]\ =\ f\ (s[t-y],\ i_1[t-x_1],...,\ i_i[t-x_i],\ r_{1}[t-k_{1} | d_1],..., \ r_{j}[t-k_{j} | d_j])$\\
%   then $s[t]$ is eventually resolved\\
%   $(s[t], c)\ \in\ R_{V_s}[t'], t' > t$ By (2)\\
%   then a response can be emitted\\
%   $(res, s[t], c, V, V_s)$ By line 20\\
%   at last, the response arrives at its destination\\
%   $(res, s[t], c, V, V_s)\ \in\ Q_{V}[t"], t" <= t' + d$ By \ref{L4}\\
%   (1) and (2) hold for inductive case.
% \end{proof}

% \setcounter{theorem}{\value{backup}}

% %redundant with next one
% %\setcounter{backup}{\value{theorem}}
% %\setcounter{theorem}{\value{thm-correctness-strict-d}}
% %
% %\begin{theorem}[Correctness of strict decentralised]
% %  \label{thm:correctness-cent-decent-strict}
% %  prove the evaluation is equal by proving the parameters feed to both functions are equal.
% %  Let $f (I, \varphi, t)$  be the decentralised version,
% %  let $g (I, \varphi, t)$  be the centralised version,
% %  let us prove that $f = g$
% %  Decentralised evaluation consist on the evaluation of subexpressions and those of inputs
% %  $eval_d(I,s,t) = f(eval_d(I, r_j, t'), eval_d(I, i_i, t'))$
% %  Analogously, for the centralised version:
% %  $eval_c(I,s,t) = f(eval_c(I, r_j, t'), eval_c(I, i_i, t'))$
% %\end{theorem}
% %
% %\setcounter{theorem}{\value{backup}}

% \setcounter{backup}{\value{theorem}}
% \setcounter{theorem}{\value{thm-correctness-c-d-eval}}
% \begin{theorem} [Theorem correctness of decentralised and centralised with evaluation]
%   \label{thm:correctness-cent-decent-eval}
%   The centralised and decentralised algorithms using the evaluation simplification yield the same outputs for any input.
%   Let $\form$ be a well defined specification and $I$ an input of size $N$. Let $O_{ce}$ be the outputs of the centralised evaluation and $O_{de}$ the outputs of the decentralised evaluation with the topology $\topo$. Then $O_{ce} = O_{de}$.
% \end{theorem}

% \begin{proof}
%   Let $E$ be the evaluation graph of $\varphi$, let $I$ be the input and let $\rho$ be the evaluation distance of $E$. We show by induction on $\rho(v^t)$ that $O_c(v_t) = O_d(v_t)$
%   \paragraph{Base case}[$\rho = 0$]
%   let $s[t]\ =\ f\ (s[t-y|d],\ i_1[t-x_1|d],...,\ i_i[t-x_i|d],\ r_{1}[t-k_{1}|d_1],..., \ r_{j}[t-k_{j}|d_j])$ be the stream expression\\
%   And this expression is the same for the centralised and decentralised algorithms.
%   As $\rho(s[t]) = 0$ then $\rho(r_1) = ... = \rho(r_{j}[t-k_{j}|d_j]) = 0$\\
%   But $s[t]$ can only depend on subexpressions $r_1, ..., r_j$ such that \\
%   $r_{1}[t-k_{1} | d_1],..,\ r_{j}[t-k_{j} | d_j] < s[t]$ in the given well-founded order.\\
%   Thus, they are either inputs or streams whose all subexpressions are simplified to default values, to comply with the order.\\
%   Those that will be simplified are those that meet $t+k < 0\ or\ t+k > N$ 
%   Then $\ r_{1}[t-k_{1} | d_1],..., \ r_{j}[t-k_{j} | d_j] = d_1, ..., d_j$ By line 19\\
%   Note that V need not send messages to know the default values $d_1, ..., d_j$\\\
  
%   If an input:\\
%   if it will be resolved in a remote node, a request is sent by line 21\\
%   that request will arrive at its destination by lemma 1 \ref{L4}\\
%   then it is processed and as it is an input at some time t' it will be resolved\\
%   then a response can be emitted with the value in R by line 20\\
%   then the response arrives at V with the pair $(i[t], c)$ by lemma 1 \ref{L4}\\
%   so it is resolved in V\\
%   Alternatively, the input is received at some time in V.\\
  
%   Either case :\\
%   $i_1[t-x_1],...,\ i_i[t-x_i]\ \in\ R_{v}[t"]$ with their respective values by line 17 or by Convergence 2\\
%   So, by applying all its parameters, $s[t]$ is resolved in the decentralised with evaluation version:\\
%   $(s[t], c)\ \in\ R_{V_d}[t"]$ By line 19\\
  
%   On the other hand the centralised with evaluation algorithm will resolve $s[t]$ at instant $t'$
%   where $t' = max_i (t-x_i)$. At said moment both the default values $d_1, ..., d_j$ and the inputs $(i_1,c_1), ..., (i_i, c_i)$ are available to evaluate the expression of $s[t]$.
%   $(s[t], c)\ \in\ R_{V_d}[t"]$ By line 19\\
%   Because applying the same expression (function) over the same arguments yield the same result.
  
%   \paragraph{IH :$\rho(r[n]) < \rho(s[n])$}  
%   Assuming that for $\rho(r[n]) < \rho(s[n])$ the value of $r[n]_{cs}$ is equal to $r[n]_{ce}$ for an arbitrary $t$\\
%   Prove $s[t]_{ce} = s[t]_{cs}$ assuming their subexpressions are resolved and equal for $\rho(r[n]) < \rho(s[n])$\\
%   let $s[t]\ =\ f\ (s[t-y],\ i_1[t-x_1],...,\ i_i[t-x_i],\ r_{1}[t-k_{1} | d_1],..., \ r_{j}[t-k_{j} | d_j])$\\
%   And considering \\
%   $x_{1..i}\ \in\ \Int$\\
%   $k_{1..j}\ \in\ \Int$\\
%   $y\ \in\ \Nat$\\
%   $r_{1..j} < s[t]$ in the above specified order\\
%   all params are resolved to the same values as in the centralised with evaluation algorithm by IH 
%   So, s[t] is resolved eventually in the future to a constant $c$
%   $s[t]\ \in\ R_V[t^{IV}],\ t^{IV} = max(t", t''') = max (t", t + max_{i=1..i}(t-x_i))$\\
  
%   On the other hand the centralised version will resolve it by evaluating the expression of $s[t]$ applying all its parameters, both inputs and subexpressions.
%   Thus, $s[t]\ \in\ R_V,$\\
%   And as the inputs for the expression are equal to those of the decentralised version, and all the subexpressions with lesser $\rho$ are resolved to the same values in both algorithms, we can conclude that the value of $s[t]$ obtained by the centralised and decentralised algorithms are equal. For every $s[t]$.
  
% \end{proof}

% \setcounter{theorem}{\value{backup}}

% \setcounter{backup}{\value{lemma}}
% \setcounter{lemma}{\value{lem-simpl-two}}
% \begin{lemma}
%   \label{lem:simpl-two}
%   For every $t, \si_1$ and $\si_2$\\
%   $t \si_1 \si_2 \eqval \simpl(\simpl(t\si_1)\si_2)$\\
% \end{lemma}
% \begin{proof}
%   We first show that
%   \begin{equation}
%     \text{if $t \eqval t'$ then for every $\si$ such that $t\si \eqval t'\si$}
%     \label{eq:sigma-eqval}
%   \end{equation}
%   Let $\si_2$ be an arbitrary substitution from $Val(Vars(t\si) \Union Vars(t'\si))$.\\That is a substitution of the remaining variables after substituting $\si$\\
%   then ($\si\si_2$) is a substitution from $Val(Vars(t) \Union Vars(t'))$, all variables present in $t$ or $t'$.\\
%   Since $t \eqval t'$, then\\
%   $Eval(t\si\si_2) = Eval (t'\si\si_2)$, or in other words\\
%   $Eval((t\si)\si_2) = Eval ((t'\si)\si_2)$ this implies $t\si \eqval t'\si$.
%   Hence, (\ref{eq:sigma-eqval}) holds.
  
%   Now, first $t\si_1 \eqval t\si_1$ by reflexivity.\\
%   Then $t\si_1 \eqval simpl\ t\si_1$ by definition of admissible simplifiers\\
%   It follows that $t\si_1\si_2 \eqval (simpl t\si_1)\si_2.$\\
%   Then by Fact \ref{eq:Atwo} $t\si_1\si_2 \eqval\ simpl((simpl\ t\si_1)\si_2)$ as desired.
% \end{proof}

% \setcounter{lemma}{\value{backup}}

% \setcounter{backup}{\value{lemma}}
% \setcounter{lemma}{\value{lem-simpl-distr}}
% \begin{lemma} [Simplification distributive property]
%   \label{lem:simpl-distr}
%   Let $t$ be a term,  let $\si_0, ..., \si_n$ be substitutions from $Val(Vars(t))$,\\
%   Let $t_0, ...,t_n$ be defined as follows: $t_0 = t,\ t_{i+1} = simpl(t_i\si_i)$\\
%   then\\
%   $t_n \eqval simpl(t\si_1...\si_n)$\\
%   then 
%   $t_n \eqval simpl(t\si_0 ... \si_{n-1})$
% \end{lemma}
% \begin{proof}
  
%   We show by induction on $n$ that $t_n \eqval t\si_0, ..., \si_{n-1}$.
%   IH: $t_{n-1} \eqval t\si_0, ..., \si_{n-2}$
%   Now by ``simpl preserves equivalence'' \ref{eq:Atwo} and by ``substitution to both members preserves equivalence'' \ref{eq:sigma-eqval} then
%   $simpl (t_{n-1}\si_{n-1}) \eqval t\si_0, ..., \si_{n-2}\si_{n-1}$
%   Now $t_n = simpl(t_{n-1}\si_{n-1})$ and by reflexivity $t_n \eqval simpl(t_{n-1}\si_{n-1})$
%   Hence, $t_n \eqval t\si_0, ..., \si_{n-1}$ follows.
%   Now applying ``simpl preserves equivalence'' we obtain the desired result.
% \end{proof}

% \setcounter{lemma}{\value{backup}}

% \setcounter{backup}{\value{lemma}}
% \setcounter{lemma}{\value{lem-subs-simpl-ground}}
% \begin{lemma}Let $t[x_1,...,x_n]$ be a term, and simpl a simplifier.
%   \label{lem:subs-simpl-ground}
%   Let $\si$ be a partial substitution of $X$ such that $simpl(t\si) = c$. Then, for every $\si_{rest}, simpl(t\si\si_{rest}) = c$
%   In particular if $t\si\si_{rest}$ is ground, $Eval(t\si\si_{rest}) = c$
% \end{lemma}
% \begin{proof}
%   $t\si \eqval simpl(t\si) \eqval c$
%   Consequently,     $t\si\si_{rest} \eqval simpl(t\si\si_{rest}) \eqval c\si_{rest}$, and $c\si_{rest} \eqval c$
%   Finally, since $t\si\si_{rest}$ is ground $Eval(t\si\si_{rest}) = d$, which satisfies $d \eqval c$
% \end{proof}

% \setcounter{lemma}{\value{backup}}

% \setcounter{backup}{\value{theorem}}
% \setcounter{theorem}{\value{thm-correctness-c-simpl-c-strict}}
% \begin{theorem}[Theorem correctness of centralised with simplification and centralised strict]
%   \label{thm:correctness-cent-simpl-cent-strict}
%   The centralised with evaluation and the centralised with simplification algorithms yield the same outputs for any input.
%   Let $\form$ be a well defined specification and $I$ an input of size $N$. Let $O_{ce}$ be the outputs of the centralised evaluation and $O_{cs}$ the outputs of the centralised with simplification. Then $O_{ce} = O_{cs}$.
% \end{theorem}

% \begin{proof}
%   Let $E$ be the evaluation graph of $\varphi$ and $I$ and let $\rho$ be evaluation distance of $E$. We show by induction on $\rho(v_t)$ that for all $O_{ce}(v_t) = O_{cs}(v_t)$
%   \paragraph{Base case}[$\rho = 0$]
%   let $s[t]\ =\ f\ (s[t-y|d],\ i_1[t-x_1|d],...,\ i_i[t-x_i|d],\ r_{1}[t-k_{1}|d_1],..., \ r_{j}[t-k_{j}|d_j])$ be the stream expression\\
%   And this expression is the same for both algorithms.\\
%   As $\rho(s[t]) = 0$ then $\rho(r_1) = ... = \rho(r_{j}[t-k_{j}|d_j]) = 0$\\
%   But $s[t]$ can only depend on subexpressions $r_1, ..., r_j$ such that \\
%   $r_{1}[t-k_{1} | d_1],..,\ r_{j}[t-k_{j} | d_j] < s[t]$ in the given well-founded order.\\
%   Thus, they are either inputs or streams whose all subexpressions are simplified to default values, to comply with the order.\\
%   Those that will be simplified are those that meet $t+k < 0\ or\ t+k > N$ \\
%   Then $\ r_{1}[t-k_{1} | d_1],..., \ r_{j}[t-k_{j} | d_j] = d_1, ..., d_j$ By line 19\\
%   Note that V need not send messages to know the default values $d_1, ..., d_j$\\
%   If an input it is received at some time in V.\\
%   $i_1[t-x_1],...,\ i_i[t-x_i]\ \in\ R_{v}[t"]$\\
%   As both inputs and the default values are resolved, so by applying all its parameters to its expression, $s[t]$ is resolved in the centralised with evaluation to a value $c$.\\
%   $(s[t], c)\ \in\ R_{V_d}[t"]$ By line 19\\
  
%   But, at some time $t'''$ such that $t''' \leq t"$ the centralised with simplification simplifies the expression of $s[t]$ to its value $d$.\\
%   Then by lemma \ref{lem:subs-simpl-ground} we could substitute the remaining parameters $\si_{rest}$ in the expression on $s[t]$ at $t'''$ and evaluate the expression, obtaining the same output $c$, thus we can conclude that $c = d$.
  
%   \paragraph{IH :$\rho(r[n]) < \rho(s[n])$}
%   Assuming centralised with evaluation and centralised with simplification yield the same outputs for $\rho(r[n]) < \rho(s[n])$ for an arbitrary $t$\\
%   Prove $s[t]_{cs} = s[t]_{ce} $ assuming their subexpressions are resolved and equal for $\rho(r[n]) < \rho(s[n]$\\
%   let $s[t]\ =\ f\ (s[t-y],\ i_1[t-x_1],...,\ i_i[t-x_i],\ r_{1}[t-k_{1} | d_1],..., \ r_{j}[t-k_{j} | d_j])$\\
%   And considering \\
%   $x_{1..i}\ \in\ \Int$\\
%   $k_{1..j}\ \in\ \Int$\\
%   $y\ \in\ \Nat$\\
%   $r_{1..j} < s[t]$ in the above specified order\\
%   So, s[t] is resolved eventually in the future to a constant $c$\\
%   $s[t]\ \in\ R_V[t^{IV}],\ t^{IV} = max(t", t''') = max (t", t + max_{i=1..i}(t-x_i))$\\
%   On the one hand the centralised version will resolve it by evaluating the expression of $s[t]$ applying all its parameters, both inputs and subexpressions. As follows :
%   $Eval(t, s1, ...,sn) = c$ where $s_1, ..., s_n$ are pairs of substitutions of the form $(stream, const)$
%   Thus, $s[t]\ \in\ R_V,$\\
  
%   Nevertheless, the centralised with simplification algorithm may obtain the output of the expression in some time $t' \leq t$ by applying some of the parameters of the expression. As follows:\\
%   $simpl(t, si0) = d$.
%   Then by lemma \ref{lem:subs-simpl-ground} we could substitute the remaining parameters $\si_{rest}$ in the expression on $s[t]$ at $t'''$ and evaluate the expression, obtaining the same output $c$, thus we can conclude that $c = d$.
  
% \end{proof}

% \setcounter{theorem}{\value{backup}}

% \setcounter{backup}{\value{theorem}}
% \setcounter{theorem}{\value{thm-correctness-d-simpl-d-strict}}
% \begin{theorem}[Theorem correctness of decentralised with simplification and decentralised with strict]
%   \label{thm:correctness-decent-simpl-decent-strict}
%   The decentralised with evaluation and the decentralised with simplification algorithms yield the same outputs for any input.
%   Let $\form$ be a well defined specification and $I$ an input of size $N$ and let $\Tau$ be the topology for both algorithms. Let $O_{de}$ be the outputs of the decentralised with evaluation and $O_{ds}$ the outputs of the decentralised with simplification. Then $O_{de} = O_{ds}$.
% \end{theorem}
% \begin{proof}
%   Let $E$ be the evaluation graph of $\varphi$ and $I$ and let $\rho$ be evaluation distance of $E$. We show by induction on $\rho(v_t)$ that $O_{ds}(v_t) = O_{de}(v_t)$
%   \paragraph{Base case}[$\rho = 0$]
%   let $s[t]\ =\ f\ (s[t-y|d],\ i_1[t-x_1|d],...,\ i_i[t-x_i|d],\ r_{1}[t-k_{1}|d_1],..., \ r_{j}[t-k_{j}|d_j])$ be the stream expression\\
%   And this expression is the same for the decentralised with simplification and decentralised strict algorithms.\\
%   As $\rho(s[t]) = 0$ then $\rho(r_1) = ... = \rho(r_{j}[t-k_{j}|d_j]) = 0$\\
%   But $s[t]$ can only depend on subexpressions $r_1, ..., r_j$ such that \\
%   $r_{1}[t-k_{1} | d_1],..,\ r_{j}[t-k_{j} | d_j] < s[t]$ in the given well-founded order.\\
%   Thus, they are either inputs or streams whose all subexpressions are simplified to default values, to comply with the order.\\
%   Those that will be simplified are those that meet $t+k < 0\ or\ t+k > N$ \\
%   Then $\ r_{1}[t-k_{1} | d_1],..., \ r_{j}[t-k_{j} | d_j] = d_1, ..., d_j$ By line 19\\
%   Note that V need not send messages to know the default values $d_1, ..., d_j$\\
%   If an input it is resolved in V\\
%   if it will be resolved in a remote node then a request is sent by line 21\\
%   that request will arrive at its destination by     \ref{L4}\\
%   then it is processed and as it is an input at some time t' it will be resolved\\
%   then a response can be emitted with the value in R by line 20\\
%   then the response arrives at V with the pair $(i[t], c)$\\
%   so it is resolved in V\\
%   Alternatively, the input is received at some time in V.\\
%   Either case :\\
%   $i_1[t-x_1],...,\ i_i[t-x_i]\ \in\ R_{v}[t"]$ by line 17\\
%   If it is resolved to default values $s[t]$ is resolved, so by applying all its parameters, $s[t]$ is resolved in decentralised with evaluation:\\
%   As follows :
%   $Eval(t, s1, ...,sn) = c$ where $s_1, ..., s_n$ are pairs of substitutions of the form $(stream, const)$
%   Then $(s[t], c)\ \in\ R_{V_d}[t"]$ By line 19\\
  
%   Nevertheless, the decentralised with simplification algorithm may obtain the output of the expression in some time $t' \leq t$ by applying some of the parameters of the expression.\\
%   As follows:\\
%   $simpl(t, si0) = d$.
%   Then by lemma \ref{lem:subs-simpl-ground} we could substitute the remaining parameters $\si_{rest}$ in the expression on $s[t]$ at $t'''$ and evaluate the expression, obtaining the same output $c$, thus we can conclude that $c = d$.
  
%   \paragraph{IH :$\rho(r[n]) < \rho(s[n])$}
%   Prove $s[t]_d = s[t]_c $ assuming their subexpressions are resolved and equal for $\rho(r[n]) < \rho(s[n]$\\
%   let $s[t]\ =\ f\ (s[t-y],\ i_1[t-x_1],...,\ i_i[t-x_i],\ r_{1}[t-k_{1} | d_1],..., \ r_{j}[t-k_{j} | d_j])$\\
%   And considering \\
%   $x_{1..i}\ \in\ \Int$\\
%   $k_{1..j}\ \in\ \Int$\\
%   $y\ \in\ \Nat$\\
%   $r_{1..j} < s[t]$ in the above specified order will be resolved eventually to the same values that in the decentralised with simplification by IH\\
%   So, s[t] is resolved eventually in the future to a constant $c$ by applying all its parameters.\\
%   $s[t]\ \in\ R_V[t^{IV}],\ t^{IV} = max(t", t''') = max (t", t + max_{i=1..i}(t-x_i))$????\\ 
  
%   On the other hand the decentralised with simplification version will resolve it by evaluating the expression of $s[t]$ applying some its parameters but will yield the same result by P2.\\
%   Thus, $s[t]\ \in\ R_V,$\\
%   Considering that the needed inputs for the expression are equal as those of the decentralised version with evaluation, and all the needed subexpressions with lesser $\rho$ are resolved to the same values in both algorithms by IH.\\
%   Then $simpl(t, si0) = d$ follows.
%   Then by lemma \ref{lem:subs-simpl-ground} we could substitute the remaining parameters $\si_{rest}$ in the expression on $s[t]$ at $t'''$ and evaluate the expression, obtaining the same output $c$, thus we can conclude that $c = d$.
% \end{proof}


% \setcounter{theorem}{\value{backup}}

% \setcounter{backup}{\value{lemma}}
% \setcounter{lemma}{\value{lem-oracle}}
% \begin{lemma}[Oracle]
%   \label{lem:oracle}
%   Let there be an Oracle which injects the value of a stream in $R_V$ for a given node $V$.
%   The value injected by the oracle is the same as the value that the algorithm would obtain applying the expression of the stream to all its parameters.
%   Just as in the centralised LOLA.
% \end{lemma}
% \begin{proof}
%   By contradiction.\\
%   Suppose there is a stream for which the value guessed by the Oracle differs from that obtained by the system.\\
%   Given that all its substreams are well calculated and that the Oracle guesses the correct value of the stream.\\
%   Then, the only possibility is that the application of the stream expression with all its parameters performed the algorithm was incorrect. This is a contradiction.
% \end{proof}

% \setcounter{lemma}{\value{backup}}

% \setcounter{backup}{\value{lemma}}
% \setcounter{lemma}{\value{lem-back-ref}}
% \begin{lemma}[Back Reference (TTL)]
%   \label{lem:back-ref}
%   Let $s[t]$ be and instanced stream $s$ at time $\tick$, then
%   there will be no Request message for $s[t]$ received at $\delta(s)$ after $t+bref(s)$
% \end{lemma}
% \begin{proof}
% Let $r_i$, $s$ be streams s.t. $r_i \xrightarrow{w_i} s$ then\\
%   at $t_i' = t - w$ $r_i \in U_{\delta(r_i)}$ By Instantiation phase (line 19) and\\
%   at $t_i'' = t_i' + dist(\delta(r_i), \delta(s))$ a $Msg\{Req, s, \delta(r_i), \delta(s)\}$ arrives at $\delta(s)$ By lemma \ref{L4} and\\
%   at $t_{max} = Max(0, Max(t_i''))$ the last request message for $s$ arrives at $\delta(s)$.
% \end{proof}

% \setcounter{lemma}{\value{backup}}


==> old_solution.tex <==
\section{Decentralized Stream Runtime Verification}
\label{sec:solution}

In this section we describe our solution to the decentralized SRV
problem.
%
Given a well-formed \lola specification, the decentralized online
algorithm that we present in this paper will incrementally compute a
value for each output stream variable.
%
The starting point of the solution is to map each stream of the
specification to a node in the network. 
%
Input streams correspond to the ability of the node to read a new
value of the input in every instant, and output streams correspond to
the responsibility of the node to compute values of the stream.
%
Each node will run a local monitor, that will collaborate with other
monitors by exchanging messages to perform the global monitoring
tasks.
%
There is no shared memory between the computational nodes.
%
The main \emph{correctness} criteria is that we prove is that the
output produced by our network of cooperating monitors is the same as
the output that a centralized solution produces.
%
Even though the streams of outputs are identical, the decentralized
algorithm may compute an output value at a different time instant than
the centralized version, due to the different location of the inputs
and the delays and reorders produced by the communication.
%
We study this effect both theoretically in this section, and
empirically in Section~\ref{sec:empirical}.
%
Additionally, we study other non-functional aspects like the number of
messages exchanged or the memory requirements that each local monitor
needs to maintain.

%
% Structure:
% 3. Decentralized Stream Runtime Verification
%  Intro (above)
% 3.2 Configuration (static mappings) and Deployment
% 3.3 Network
% 3.4 Dynamics (state and transition, both local and global)
% 3.5 Local Algorithm (Operational Semantics)
% 3.6 Correctness

\subsection{Decentralized SRV Problem Description}
\label{subsec:problem}

A network topology $\topo:\tupleof{N,E}$ is given by a number of nodes
$N:\{1,\ldots,n\}$ and a set of directed edges $E\subseteq N\times N$
representing communication links between the nodes.
%
We assume that the graph is connected.
%
A route between two nodes $n$ and $m$ is list of nodes
$[n_0,\ldots,n_k]$ such that consecutive nodes are neighbours
(i.e. $E(n_i,n_{i+1})$), no node is repeated, $n=n_0$ and $m=n_k$.
%
We statically fix routes between every two nodes with the following
properties:
\begin{itemize}
\item If two nodes $n,m$ are neighbours then they communicate directly
  (that is $[n,m]$ is the route from $n$ to $m$).
\item If $n$ appears in a route $[l\ldots n\ldots m]$ then the route
  from $n$ to $m$ is the sub-list $[n\ldots m]$
\end{itemize}
%
This kind of properties can be enforced by calculating a spanning
tree, and imply that routing tables can be encoded by remembering at
each node $n$ only the next hop knowing the destination $m$.
%
We use $\NEXT_n(m)$ for the next hop in the routing table of $n$ for
messages with destination $m$.
%
We use $\DIST(n,m)$ for the number of hops between nodes $n$ and $m$
given a network and topology and routing table.
%
This is precisely the number of routing operations that are needed to
send a message between $n$ and $m$.

Given a a specification $\varphi(I,O)$ and a network topology
$\topo:\tupleof{N,E}$ a \emph{stream assignment} is a map $\mu:I\cup
O\Into N$ that assigns to every stream variable a network node.
%
The node $\mu(s)$ for an input stream variable $s$ is the location in
the network where $s$ is sensed in every clock tick.
%
The node $\mu(t)$ for an out stream variable $t$ is the location whose
local monitor is responsible for resolving the values of $t$.

\begin{definition}
  A decentralized SRV problem $\tupleof{\varphi,\topo,\mu}$ is given
  by a specification $\varphi$, a topology $\topo$ and a stream
  assignment $\mu$.
\end{definition}








%%%%
%%%% This subsection must go
%%%%
\subsection{Goals of the solution}
\label{sec:goals}
%The goals of this solution are the following: %JUST FORMAL DEFINITIONS

\paragraph{Performance}
%
We consider different aspects to evaluate the performance criteria.
% 
The number of messages with monitoring purposes traversing the network
should be minimized, as well as the network bandwidth and the CPU
usage of any given node.
%
Decentralized monitoring should minimize the delay between the time
all variables for a formula are present in the system and the time a
verdict or a result for the formula is returned to the user.
%
%Ideally, we would like this delay to be zero, meaning that the system emits a verdict in the same tick when all the needed values are in R.
%
%This ideal is met in centralized Lola for efficiently monitorable specifications.
%
%But in decentralized solutions this is not achievable as observations may be performed in remote nodes.
%
%Additionally, decentralized monitoring algorithms may impose additional delays.
%
%\paragraph{Number of messages}
%The number of messages is defined as $\sum m_{ij}$ where $i$ is the identifier of the node and $j$ is the identifier of the message sent by the $i$-th node. These messages with monitoring purposes
%traversing the network should be minimized.
%\paragraph{Bandwidth}
%Decentralized monitoring should minimize the network bandwidth usage as much as possible. Formally, $\sum_i payload_i$ where $i$ represents the number of messages and $payload_i$ represent the number
%of bits of payload that the message $i$ carries. We will use standard sizes such as 4 bytes for an integer, 8 bytes for a double, one bit for a boolean and for data structures we will count the number
%of elements and multiply by the size of each individual element and so forth, resulting in measuring the size in the total number of bits used.
%\paragraph{CPU} 
%Decentralized monitoring should minimize the CPU usage of a given node, so that the monitoring overhead is kept low at each computing node. We want the computation to be as evenly distributed among
%the monitors as possible in order not to overload some monitors while other are idle.Formally, let $s_e$ be the number of simplifications until a certain expression in Unresolved is resolved, let
%$mon_m = sum_{expression} s_e$ be the number of simplifications that a single monitor perform in a cycle and let $allCycle = \sum_{monitor} mon_m $ is the total number of simplifications performed in
%a cycle in all monitors, then for all $m$ . $mon_m \approx \frac{allCycle}{numMonitors}$.
%\paragraph{Verdict delay}
%Decentralized monitoring should minimize the delay between the time all variables for a formula are present in the system and the time a verdict or a result for the formula is returned to the
%user. Formally, let $t$ be the time at which every needed input to the specification $s$ are present in the system, and let $t_1$ such that $t_1 \ge t$ be the time in which $s$ is resolved to a value,
%that is a final verdict.We would like to minimise $t_1 - t$. Ideally, we would like this delay to be zero, meaning that the system emits a verdict in the same tick it has all the needed values. This
%ideal is met in centralized Lola for efficiently monitorable specifications. But in decentralized solutions this is not achievable as observations may be performed in remote nodes. Additionally,
%decentralized monitoring algorithms may impose additional delays.

\subsection{Message passing}
\label{ass:msg-passing}
Messages considered in this work will arrive always at their destination exclusively(i.e. unicast communication) and there will not be duplicates nor delays in the transmition.
%
A message sent at time $t$ will be available at destination at $t + 1$.
%All messages will be timestamped as well as carry a sequence number. This sequence number $seq$ will be the number of messages sent by monitor $M_i$.
%Having these two numbers supposedly allow for a total order to be enforced on the messages even though they could arrive with an unbounded delay.(THIS IS ANOTHER SCENARIO)
Messages can be of one of these three types: Request
%: $req_{seq}\{\subform_t, V_{src}, V_{dest}\}$
,Response %: \label{response}  $res_{seq}\{\subform_t = c, V_{src}, V_{dest}\}$
or Trigger.%:\label{trigger} $trigger_{seq}\{\subform_t, V_{src}, V_{dest}\}$ See \ref{trigger}.
%
%\begin{itemize}
%\item{Request:} $req_{seq}\{\subform_t, V_{src}, V_{dest}\}$
%\item{Response:} \label{response}  $res_{seq}\{\subform_t = c, V_{src}, V_{dest}\}$
%\item{Trigger:} \label{trigger} $trigger_{seq}\{\subform_t, V_{src}, V_{dest}\}$ See \ref{trigger}
%\end{itemize}
%explain how U evolves before this example DONE in intro
%
%EXAMPLE placement
%
\subsection{Distributing monitors}
\label{dist-mon}
%
In this section we analyze the core of the solution presented in this work.
%
We use a network of monitors that cooperate in order to resolve the output of the monitors created from a given formula on an input trace.
%
%We describe with detail all the concepts and components needed for our solution to behave and achieve the properties that we desire.
%
Intuitively, we distribute the formula in subformulas that are
assigned to monitors, which in turn are deployed in the nodes of the
topology.
%
The input trace is observed in multiple nodes. %, in contrast to a centralized observation.
%
At each cycle, each monitor reads the input and the incoming messages, then with their already resolved subformulas, the monitor tries to simplify the unresolved subformulas assigned to it.
%
After the simplification stabilizes, the resolved subformulas obtained are sent to the interested nodes in accordance to the communication strategies (see Section~\ref{commstrategies}).
%
Repeating this process leads to the correct evaluation of the formula over the input as it is proved in the Section~\ref{sec:simplification}.
%
Formally, we will have a set of monitors $M = {m_1, ..., m_m}$, a topology $\topo$, a specification $\form$ and an input trace of events $I$.
%
We want our solution to be a function $L~:~M\times\topo\times\form\times I ~\produce ~ type$ whose result is that of computing the specification in the monitors of the topology over an input trace of
events.
%
%In the case of Boolean specifications, the output type will be Boolean, and for any other specification type, the output type will be the corresponding one.

\paragraph{Local Monitor}
A Local Monitor is a process running in a computation node that communicates with neighbouring local monitors of the system through message passing.
%
No shared memory is assumed in our system.
%
A monitor $M$ can be modelled as $M:\tupleof{I, Q, E, U, R, Pen, O, \topo, \deploy, \Tracelen, \EvalStreams, \Triggers}$.
%
A monitor receives the set of Input variables at time $\tick$ in $I$ from the trace of observations that are in the scope of this Monitor, of the form $i[\tick] = c$ for $i \in I$ and will store them in $R$.
%
%At that time the value $c$ of the variable $i[\tick]$ is accessible for the monitor without the need to communicate with any other node.
%
A monitor receives messages in $Q$ from its neighbouring nodes accordingly to the messages described in Section~\ref{ass:msg-passing}.
%
A monitor stores the subexpressions that are assigned to it in $E$.
%
These expressions are instantiated and placed in $U$ for every valid tick of the clock.
%
These expressions have the form $\subform[\tick] = \ga[\tick]$ simplified up to the best knowledge of this node at the present tick.
%
$\ga[\tick]$ is an expression of the type of the stream that is not a constant.
%
As we will see, when $\ga[\tick]$ becomes a constant $c$, the equation $\subform[\tick] = c$ is resolved and moved to $R$.
%
A monitor stores resolved equations in $R$, of the form $\subform[\tick] = c$ where $c$ is a constant of the data type.
%
This corresponds to values that the monitor has been able to resolve.
%
A monitor stores requested streams and triggers in Pen, in order to respond them when they get resolved.
%
\begin{definition} [Local expressions]
  \label{def:local-exp}
  Let $\subform[\tick]$ be a local expression that is (part of) a formula. Let $\tick$ be a specific time, then $\subform[\tick]$ is either on $U_t$ or in $R_t$ (but not in both).
\end{definition}
\begin{definition} [Global as composition of local]
  \label{def:global-comp-local}
  Let $\mu$ be the global state of the decentralized version of LOLA and $\nu_i$ the state of the local monitor $M_i$,
  then $\mu\ =\ \prod\ \nu_i$
\end{definition}

%
A monitor has the set of messages to be sent in the tick in $O$.
%
%These messages match the patterns described in Section~\ref{ass:msg-passing}.

We consider static non changing connected topologies.
%
%In such a topology, modelled as a connected graph, a routing table can be built such that it contains the shortest path between every pair of nodes.
%
The information about the system topology as an adjacency matrix will be stored in $\topo$. 
%
$\topo$ is specific for each node and relates any destination node ($V_d$) to next-hop node ($V_n$).
\begin{fact}[Route Table and distance]
  \label{fact:route-table}
  For every $V$, $V_d$, let $RT_V(V_d) = [U_1,...,\ U_k]$ the list of monitors in the shortest path from $V$ to $V_d$
  then $U_1$ is the next-hop monitor, $U_k\ =\ V_d$ and $k\ =\ len(l)$ the length of the path
  where $l\ =\ U_1\ :\ RT_{U_1}(V_d)$
\end{fact}

\newcounter{lem-L4}
\setcounter{lem-L4}{\value{lemma}}
\begin{lemma}[Every message arrives]
  \label{lem:L4}
  Let $m\ =\ (req,\ \subform,\ V_s,\ V_d)\ or\ m'\ =\ (res,\ \subform,\ c,\ V_s,\ V_d)\ \in\ Q_v$ for some node $V$ and time $\tick$.
  then $M\ \in\ Q_{V_{d_{t'}}}$ for some $\tickp'\ =\ \tickp\ +\ \tickoffp$ where $h$ is the height of $\subform$ in $\form$ and 
  $\tickoffp\ =\ len(l)$ and $l\ =\ RT_v(V_d)$
\end{lemma}
%\begin{proof}  By Induction on $\tickoffp$:\\
%  \textbf{Base case:}$\tickoffp =\ 0$\\
%  If the distance between the nodes is zero the list of the nodes of the path is empty $RT_V(V_d)\ =\ []$. Then $V = V_d \And\ m\ \in\ Q_V\ \And\ \tickp'\ =\ \tickp$\\
%  \textbf{Induction Hypothesis (IH)}
%  This lemma holds when $m\ \in\ Q_{V_{d\tickp'}}\ \And\ \tickp'\ =\ \tickp +\ \tickoffp,\ \tickoffp\ =\ len(RT_v(V_d))$\\
%  %\begin{align*}
%  Proof for $\tickoffp +\ 1\ =\ len(RT_v(V_d))$, $RT_V(V_d) = V_y\ :\ l$
%  %$RT_V(V_d) = (V_x,\ k\ +\ 1,\ V_y\ :\ l)$\\
%  $where\ l\ = [U_1, ..., U_k]$\\
%  %\produce\\
%  then $m\ \in\ Q_{V_y}[\tickp']\ \tickp'\ =\ \tickp\ +\ 1$ By IH\\
%  $RT_{V_y}(V_d)\ =\  l$ By Fact1\\
%  %\produce\\
%  then $m_2\ \in\ Q_{V_d}[\tickp"]\ \tickp"\ =\ \tickp'\ +\ \tickoffp =\ \tickp\ +\ \tickoffp\ +\ 1$ By\ IH\\
%  %\end{align*}
%\end{proof}

%Each matrix entry will be a triplet consisting of the node of the next monitor ($V_x$) in the walk from source to destination, the length of the remaining list of nodes to reach the destination, and the list of those remaining nodes.  $RT_v (V_S, V_d) = (V_x, l, [U_1, ..., U_k])$.
%We assume a connected topology, otherwise if a subformula were assigned to some non connected part of the topology, their results could not be transmitted to the requiring nodes.
%
%Therefore, the routing table at a node is a $\topo : Monitor_{dst} \produce Monitor_{next}$.
%
%Such a table can be computed statically by applying Dijkstra's algorithm, for example.
%
%  \begin{equation*}
%  Topology~::~Map~Monitor~Monitor
%  \end{equation*}
%
The syntactical decomposition of the formula $\form$ in subformulas $\subform$ and their assignment to nodes is stored in $\deploy$.
%
This assignment is made statically at the setup of the monitors and must ensure that for every $\subform$ it is deployed in some node. 
%
\begin{fact}[Deployment function]
  \label{fact:deployment}
  For every $s$ subformula contained in $\form$ there is a Node tasked of resolving it.
  This relation is provided by the function $\deploy$ :
  $\deploy(\subform_i)\ =\ V_j$
  where $i,\ j\ \in\ \Nat$
\end{fact}
\begin{fact}[Deployment independence]
  \label{fact:deployment-independence}
  Using a different $\deploy$ function does not change the output of the formula $\form$ but it could change its efficiency.
\end{fact}

%
%Thus, deploying in some (if not all) the system nodes the corresponding monitors that will be tasked with computing subformulae.
%
%$\deploy : \subform \produce Monitor$.
%  \begin{equation*}    %  \deploy~::~Map~\subform~(Monitor,~\{eager,~lazy\})%      \deploy~::~Map~\subform~Monitor%  \end{equation*}
Information about the nodes that require the result of a given subformula is stored in $\depend$ which is useful for the Eval mode of operation (see Section~\ref{eval}).
%
%This is useful for the Eval mode of operation of the streams (see Section~\ref{eval}).
%$\depend : \subform \produce [Monitor]$.
%
%EXAMPLE depend

The node will decide based on the input whether it must instantiate equations or use their default values in those cases where the times shifts get out of the trace
boundaries.
%
%These default values are used for those cases where an instantiated expression gets out of the trace length, that is, lesser than 0 or greater than the trace length.
%
The node needs to know which streams should be treated as Eval in order to communicate them properly (see Section~\ref{eval}).
%send the responses as soon as the value of those expressions are obtained, since other nodes will not request Eval streams.
%
%Also, this will be needed in order not to create any request messages by the nodes that need the result of those streams (see Section~\ref{eval}).
%
The node needs to know which streams should be treated as triggers in order to behave as described in Section~\ref{trigger}.

\paragraph{Datatypes}
\label{datatypes}
% from thesis, too long
%We use many-sorted first order logic to describe data domains.
%
%A signature $\Sigma:\tupleof{\calS,\calF}$ consist on a finite collection of sorts $\calS$, and function symbols $\calF$ (where each argument of a function has a sort, and the resulting term also has
% a sort).
%
%A simple theory, \BoolName, has only one sort\footnote{We use sort and type interchangeably in the rest of the paper.}, \BoolT, two constants $\truesym$ and $\falsesym$, binary functions $\And$ and
%$\Or$, unary function $\Not$, etc.
%%
%A more sophisticated signature is \NatName{} that consists of two
%sorts (\NatT{} and \BoolT{}), with constant symbols \sym{0}, \sym{1},
%\sym{2}\ldots of sort \NatT{}, binary symbols $\sym{+}$, $\sym{*}$,
%etc (of sort $\NatT\times \NatT\Into \NatT$) as well as predicates
%$\sym{<}$, $\sym{\leq}$, etc of sort $\NatT\times\NatT\Into\BoolT$,
%with their usual interpretation.
%%
%All theories have equality and are typically (e.g. \NatName{},
%\BoolName, \textit{Queues}, \textit{Stacks}, etc) equipped with a
%ternary symbol $\sym{if}\cdot\sym{then}\cdot\sym{else}\cdot$.
%%
%In the case of \NatName{}, the $\sym{if}\cdot\sym{then}\cdot\sym{else}\cdot$
%symbol has sort $\BoolT\times \NatT \times \NatT \Into \NatT$.
%
% %
% We use many-sorted first order logic to describe data domains.
% %
% A many-sorted first-order signature is a tuple
% $\Sigma:\tupleof{\calS,\calF}$ where $\calS$ is a finite collection of
% distinct sorts, and $\calF$ is a collection of function symbols, each
% associated with a first-order \emph{type}.
% %
% For example, a functional symbol $\symf$ that describes a function
% that takes values from $S_1$ and $S_2$ and returns a value in $\Sres$
% has type $S_1\times S_2\Into \Sres$, where $S_1$, $S_2$ and $\Sres$
% are sorts in $\calS$.
% %
% The arity of a function is the number of its arguments, each of the
% appropriate sort.
% %
% In the example above, $\symf$ has arity $2$. 
% % Functions of arity $0$ represent constants. Examples of sorts are shown in Fig.~\ref{fig:domains}.
%
%
%%\begin{figure}[bth!]
%%\begin{center}
%%  \ExampleTypesFig
%%\end{center}
%%\caption{Examples of domains: \BoolName, \NatName, \StackName, \SetName}
%%\label{fig:domains}
%%\end{figure}
%
%Our theories are interpreted, so each sort $S$ is associated with a
%domain $D_S$ (a concrete set of values), and each function symbol
%$\symf$ is interpreted as a total computable function $\domf$, with
%the given arity and that produces values of the domain of the result
%given elements of the arguments' domains.
%%
%We omit the sort $S$ when it is clear from the context.
%
%We will use \emph{stream variables} with an associated sort, but from the
%point of view of the theories, these stream variables are atoms.
%%
%As usual, given a set of sorted atoms $A$ and a theory, terms are the
%smallest set containing $A$ and closed under the use of function
%symbol in the theory as a constructor (respecting sorts).
%
Supported datatypes for the specifications are Boolean, Floating point numbers, Maps and Sets.
%
Also in order to semantically represent undefined verdicts for logical formulas we use Trivalued logic.
%
In order to represent inconclusive verdicts that tend to either true or false we use the Tetravalued Logic.

\subsection{Communication Strategies}
\label{commstrategies}
In this section we explain the different strategies about how partial results are communicated among different nodes to obtain the final verdict and what are their advantages and disadvantages.
%
%There are different strategies to when to communicate the result of a recently resolved equation, or, seen from the other side, when a node that needs the result of a subexpression that is computed in
%another node gets its result.
%
Lets first establish when we consider a specification and a trace to meet what we call best and worst scenarios.
%
Worst case is such that the whole expression must be processed for computing a verdict, that is, as if there were no simplifier at all and every subexpression deployed in every node must be computed in
order to obtain the final verdict.
%
Best case is that when for computing a verdict the node that produces the verdict (root node for the AST of the formula) has all the variables needed to resolve the whole equation and consequently,
move it to R.
%
In this case no other nodes are needed nor other messages containing partial results.
\paragraph{Eval evaluation}
\label{eval}
As soon as an expression is resolved, its result is sent to those nodes that need it.
%
In this evaluation strategy no request-type  message will ever be sent.
%
%Therefore, the delay for a given formula will always be the height of the specification tree (AST) and the number of messages will be the $num(edges)$ of that tree in the case of a clique topology.
%
This strategy minimizes delay and messages sent in the worst case (compared to lazy) but consumes more bandwidth in the best case (compared to lazy).
%
As a rule of thumb, Eval evaluation is suitable when the probability of needing to compute the formula is high.
%EXAMPLE eval

\paragraph{Lazy evaluation}
\label{lazy}
In this strategy whenever a subexpression is needed a request-type message will be sent to the appropiate node in order to perform the actions needed to obtain the result of that subexpression and emit a response. 
%
Therefore, no expression result is ever transmitted over the network unless requested. 
%
This ensures that only strictly needed messages (considering simplification rules) travel over the network. 
%
On the one hand in the best case the root node emits the verdict with 0 delay and sending a total of 0 messages. 
%
On the other hand, in the worst case for any subexpression there will be two messages sent: request and response. 
%
%So for any monitoring tree in the worst case the number of messages sent will be $2*num(edges)$ and consequently the delay will be $2*depth(tree)$. 
%
That is, just the double than using Eval strategy.
%EXAMPLE lazy

\paragraph{Hybrid evaluation}
Analyzing the subformulas of the specification one could find some subexpressions that will be needed no matter the input so the monitor tasked with that subexpression could treat them as Eval, and
some other subexpressions that may or may not be needed depending on the input, so the monitor tasked with that subexpression could treat them as Lazy.
%
%This requires the expressions to be marked appropiately.
%
This way, an intermediate solution could be achieved in which just the necessary messages are sent and the delay is kept at a minimum, 
%
%Thus, effectively tailoring the way the monitors treat each subexpression to the specific needs of the problem at hand and
obtaining the benefits of both strategies.
%EXAMPLE hybrid

\subsection{Computation duration}
Monitors can compute in the following ways that differ in when to halt and emit the verdict.
\paragraph{Stream Request}
\label{stream-request}
The monitors run until they resolve \textbf{all} requested streams in Pen in every node.% [and empties Q, Out and I].
%EXAMPLE stream-req
\paragraph{Trigger}
\label{trigger}
The monitors run until they resolve \textbf{any} of the Trigger streams and emit it as the verdict.
\paragraph{Combination}
The two modes above can be combined in the following way: independently of whether there are remaining requested streams or other triggers in $Pen$ in any monitor, as soon as one Trigger in the
whole topology is resolved, the monitors will halt yielding the value of that Trigger as final verdict.
%if a trigger is specified and also there are streams requested in Pen, the system will halt as soon as the trigger is resolved but will compute the requested streams meanwhile. 
%
%Namely, it will stop if the trigger value is obtained or if all the requested streams in Pen are resolved, whatever happens first and will yield the corresponding final verdict. 
%
%REVISE (the trigger is stored in PEN and if it is not emptied the system will not halt) DONE explained as it is now

\subsection{Local Algorithm: Operational Semantics}
Every node $V_x$ will execute Algorithm~\ref{alg:local-algo}.

\paragraph{Incoming messages processing} Lines 1-17 deal with incoming message processing. 
%
In this phase the forwarding of messages ocurrs. 
%
%Also, the responses to those requests or triggers of streams that are already in R.
%
Requests and Triggers are stored in Pen. In addition, every response is stored in R.

\paragraph{Reading Input} Line 18 all observations are received as inputs for the monitors, so they are added to the Resolved set of equations.

\paragraph{Instantiation of equations} Line 19 describes how the subformulas assigned to the node are instantiated and added to U.

\paragraph{Simplification} Line 20 shows how with the knowledge in R the equations in U are simplified, those that get resolved will be moved from U to R. See section~\ref{simplification}.

\paragraph{Send responses} Lines 21-28 show how responses are sent for the newly resolved equations considering the communication strategies described in~\ref{commstrategies}: send Lazy streams that were
in Pen(received a request previously) send Eval streams to all those nodes that require it and send triggers.

\paragraph{Send and record requests} Lines 29 and 30 show how requests are sent for those substreams that are treated as Lazy and are also in Pen. Also, remember already requested streams in order not
to duplicate requests.

\paragraph{Prune R} Line 31 show how the values of the instanced streams in R can be safely removed when they are no lonoger useful.

\begin{algorithm}
  \caption{Local algorithm for monitor $V_x$ at time $\tick$}\label{alg:local-algo}
  \begin{algorithmic}[1]
    \ForAll {$m \in Q_t$} \Comment{Process incoming messages}
    \State $Q_t \gets Q_t / {m}$
    \If { $m.dst \neq V_x$}
    \State $route(m);$
    \ElsIf {$m.dst = V_x$}
    \If {$m.type = req \Or m.type = trigger$}
    \State $Pen_t \gets Pen_t + {m}$
    \ElsIf {$m.type = res$}
    \State $R_t \gets R_t + (m.stream[\tick], m.res)$
    \EndIf
    \EndIf
    \EndFor
    \State $R_t \gets R_t + (i[\tick],\ val(i[\tick]))$ for all $i[\tick]\ \in\ I_t$ \Comment{Read input}
    \State $U_t \gets U_t + (\subform[\tick],\ \expr(\subform[\tick]))$ for all $\subform$\ .\ $\deploy(\subform) = V_x$ \Comment{Generate equations}
    \State $U, R \Union newR \gets Simplify\ (U,\ R)$       \Comment{Substitute \& Simplify}
    \State $newEval \gets newR \cap Eval$
    \ForAll{$r \in newEval$} \Comment{Send Eval responses}
    \ForAll{$V_j \in \depend(r)$}
    \State $route (res\{r.str, r.val, V_x, V_y\})$  
    \EndFor
    \EndFor
    \ForAll{$m \in Pen$}
    \If{$m.str \in R$}
    \If {$m.type = Lazy$} \Comment{Lazy streams}
    \State $Pen_t \gets Pen_t\ /\ {m};route(res\{r.str, r.val, V_x, m.src\})$ 
    \ElsIf {$m.type = Trigger$} \Comment{Trigger streams}
    \State $Pen_t \gets Pen_t\ /\ {m};trigger(res\{r.str,r.val, V_x, m.src\})$ 
    \EndIf
    \EndIf
    \EndFor
    \State $timedSubstreams \gets \substr(\form[\tick]) . \form[\tick]\ \in\ Pen_t \cap Lazy \And \subform_{i} \notin Requested$% \And \deploy(\subform_{i}) = V_i\ .\ i \neq x$
    \ForAll{$substream \in timedSubstreams$} \Comment{Request needed subexpressions}
    \State $route(req\{substream, V_x, V_y\})$
    \State $Requested \gets Requested + {substream}$ \Comment{Remember requested streams}
    \EndFor
    \State $R_t \gets R_t - {r_{ttl = 0}} \text{for all}\ r\ \text{whose ttl is zero}$ \Comment{Prune R}
  \end{algorithmic}
\end{algorithm}

\subsection{Proofs}
\label{proofs}
Proof that the decentralised algorithm is correct.
%
Missing proofs can be found in the appendix.
%DONE FOR LAZY ONLY.
%\subsection{Main Lemma} Let $\si[0,\ T]$ be an input and let $O[0,\ T]$ be the centralised version of LOLA.\\
%Let $o[0,\ T] =\ \varphi$ be the decentralised version of LOLA
%then $O[0,\ T]\ =\ o[0,\ T]$.

%\begin{fact}[Well-?formedness?]
%  For any given $s[\tick]$ subexpression of $\varphi$, the expression of $s[\tick]$ will only contain subexpressions $r$ that meet $r < s[\tick]$:
%  \[   \left\{
%  \begin{array}{ll}
%    past\  h(r) < h(s[\tick]) \Or (h(r) = h(s[\tick]) \And t_r < t_s) \\
%    future\ h(r) < h(s[\tick]) \Or (h(r) = h(s[\tick]) \And t_r > t_s) 
%  \end{array} 
%  \right. \]
%  see Convergence III
%\end{fact}

\newcounter{thm-convergence}
\setcounter{thm-convergence}{\value{theorem}}
\begin{theorem} [Convergence]%V
  \label{thm:convergence}
  Every request produces a response and every $\subform[\tick]$ is eventually resolved and every time a response is sent then $\subform[\tick]$ is resolved to $c$, $(\subform[\tick], c)\ \in R_v$
  Formally, let $s[\tick]$ be a timed stream and let $V = \deploy(s)$ and $V_{src}$ be an arbitrary node and
  \begin{compactitem}
  \item{(1)}  let $req\{\subform[\tick], V_{src}, V\}$ be a msg in state $\Si_t$
  then, for some $t' > t$ there is a $c$ and a msg $res\{\subform[\tick], c, V, V_{src}\}$ in state $\Si_{t'}$
  \item{(2)} Also, for every $t"$ for which $\subform[\tick] \in U_V$ there is $t''' > t"$ for which $\subform[\tick] \in R_V$
  \end{compactitem}
  The proof will proceed by structural induction, with a well-ordering over $\rank$.
\end{theorem}
%\begin{proof}
%  By induction on $\rank$ based on previous lemmas and the lines of the algorithm.
%  \textbf{Base case}  Let us show that (1) holds for inputs:\\
%  Let $req\{i_{i}[\tick-x_i],\ V_s,\ V\}\ \in\ Q_V[t']$ and $\deploy(i_i) = V,\ x_i\ \in\ \Int $By Lemma~\ref{L4}\\
%  $\rank(i_i[\tick]) = 0$
%  As it is an input, $(i_{i}[\tick-x_i], v_i)\ \in\ R_V[t"]\, t" = t-x_i$ By line 10\\%READ INPUT
%  Then $res\{ i_{i}[\tick-x_i],\ v_i,\ V,\ V_s\}$ will be sent by line 20\\
%  Then $res\{ i_{i}[\tick-x_i],\ v_i,\ V,\ V_s\}\ \in\ Q_{V_s}[t'''] $ By Lemma~\ref{L4}  
%  
%  Proof (2) holds for $\rank(\subform_i[\tick]) = 0$:\\
%  $\subform[\tick]\ =\ f\ (\subform[\tick-y|d],\ i_1[\tick-x_1|d],...,\ i_i[\tick-x_i|d],\ r_{1}[\tick-k_{1}|d_1],..., \ r_{j}[\tick-k_{j}|d_j])$\\
%  As $\rank(\subform[\tick]) = 0$ then $\rank(r_1) = ... = \rank(r_{j}[\tick-k_{j}|d_j]) = 0$\\
%  But $\subform[\tick]$ can only depend on subexpressions $r_1, ..., r_j$ such that \\
%  $r_{1}[\tick-k_{1} | d_1],..,\ r_{j}[\tick-k_{j} | d_j] < \subform[\tick]$ in the given well-founded order.\\
%  Thus, they are either inputs or streams whose all subexpressions are simplified to default values, to comply with the order.\\
%  Those that will be simplified are those that meet $t+k < 0\ or\ t+k > N$ 
%  Then $\ r_{1}[\tick-k_{1} | d_1],..., \ r_{j}[\tick-k_{j} | d_j] = d_1, ..., d_j$ By line 12\\%SIMPL
%  Note that V need not send messages to know the default values $d_1, ..., d_j$\\\
%  If an input it is resolved in V\\
%  $i_1[\tick-x_1],...,\ i_i[\tick-x_i]\ \in\ R_{v}[t"]$ by line 10\\%READ INPUT
%  If it is resolved to default values $\subform[\tick]$ is resolved, so:\\
%  $\subform[\tick]\ \in\ R_V[t"]$ By line 12\\%19 -> 12 SIMPL 
%  (2) holds.
%  
%  Proof (1) holds based on (2) holds:\\
%  let $msg =req\{\subform[\tick], V, V_s\},\ \deploy(\subform) = V_s,\ msg\ \in\ Q_{V_s}[t'],\ t' <= t + d$ By Lemma~\ref{L4}\\
%  and $\rank(\subform) = 0$\\
%  Then $\subform[\tick]$ is resolved at some time in the future\\
%  $\subform[\tick]\ \in R_{V_s}[t"] t" > t'$ By (2)\\
%  Then a response is sent back to $V$ $res\{\subform[\tick],v, V_s, V\}$ By line 20\\%RES Lazy
%  which is received at $t'''$ $res\{\subform[\tick],v, V_s, V\} \in Q_V[t'''],\ t''' <= t" + d$ By Lemma~\ref{L4}\\
%  (1) and (2) hold for base case.\\
%  
%  \textbf{Induction Hypothesis (IH)}  
%  Assuming the theorem holds for all $\rank(r[\tick]) < \rank(\subform[\tick])$ for an arbitrary $\tick$\\
%  Proof of (2) assuming (1) holds for the IH\\
%  let $\subform[\tick]\ =\ f\ (\subform[\tick-y],\ i_1[\tick-x_1],...,\ i_i[\tick-x_i],\ r_{1}[\tick-k_{1} | d_1],..., \ r_{j}[\tick-k_{j} | d_j])$\\
%  And considering \\
%  $x_{1..i}\ \in\ \Int$, $k_{1..j}\ \in\ \Int$, $y\ \in\ \Nat$ and $\rank(r_{1..j}) < \rank(\subform[\tick])$\\
%  Then requests are sent to the corresponding nodes\\
%  $req\{ r_{1}[\tick-k_{1} | d_1],..., \ r_{j}[\tick-k_{j} | d_j], V, V_{1..j}\}$ By line 25\\%21 -> 25 Req streams
%  Those requests produce responses that return\\
%  $res\{ r_{1}[\tick-k_{1} | d_1],..., \ r_{j}[\tick-k_{j} | d_j],c_1, ..., c_j, V_{1..j}, V\} \in\ Q_V[t"]$ by (1) \\
%  So, both subexpressions and inputs are resolved waiting enough:\\
%  $(r_{1..j}, c_{1..j})\ \in\ R_V[t"]$\\
%  $(i_{1..i}, v_{1..i})\ \in\ R_V[t'''],\ t''' = t + max_{i=1..i}(t-x_i)$\\
%  So, $\subform[\tick]$ is resolved eventually in the future\\
%  $\subform[\tick]\ \in\ R_V[t^{IV}],\ t^{IV} = max(t", t''') = max (t", t + max_{i=1..i}(t-x_i))$\\
%  This proves that(2) holds assuming (1).
%  
%  Proof (1) assuming (2)\\
%  Let $msg = req\{ \subform[\tick],V, V_s\}\ \in\ Q_{V_s}$ By Lemma~\ref{L4}\\
%  let   $\subform[\tick]\ =\ f\ (\subform[\tick-y],\ i_1[\tick-x_1],...,\ i_i[\tick-x_i],\ r_{1}[\tick-k_{1} | d_1],..., \ r_{j}[\tick-k_{j} | d_j])$\\
%  then $\subform[\tick]$ is eventually resolved\\
%  $(\subform[\tick], c)\ \in\ R_{V_s}[t'], t' > t$ By (2)\\
%  then a response can be emitted\\
%  $res\{ \subform[\tick], c, V, V_s\}$ By line 20\\
%  at last, the response arrives at its destination\\
%  $res\{ \subform[\tick], c, V, V_s\}\ \in\ Q_{V}[t"], t" <= t' + d$ By Lemma~\ref{L4}\\
%  We have proved that (1) and (2) hold for the inductive case.
%\end{proof}

\begin{fact}
  \label{fact:streams-resolved}
  Convergence provides a value for every stream in a certain time $t'$.
\end{fact}


\section{Simplification}
\label{simplification}
In this section we discuss the use of simplifiers in our algorithm.
%
We describe the properties that we desire for our simplifiers and provide formal proofs of their correctness.
%
Simplifiers are important in practice because they provide performance enhancements.
%
Simplifiers are based on the principle that sometimes an expression can be correctly evaluated without knowing all their parameters.
%
The simplification algorithm is based in the simplification used in Lola~\cite{dangelo05lola}.
%
We are interested in showing that the decentralized algorithm that we propose (using simplifiers) is correct.
%
In order to do this we will proceed as follows: we will show the correctness of the algorithm ignoring the presence of simplifiers, showing a proof by comparing with the output of Lola without simplifiers.
%
Then we prove that the simplifiers preserve the equivalence under evaluation and prove that the centralized Lola without simplifiers is correct by comparing to Lola (which uses simplifiers).
%
At the end we will show that Lola produces the same outputs that our proposed algorithm, that is decentralized and uses simplifiers.
%
By transitivity we can also conclude that our algorithm is equivalent (produces the same outputs) as the decentralized algorithm without simplifiers.

\begin{algorithm}
  \label{alg:simplify}
  \caption{Simplification algorithm}
  \begin{algorithmic}[1]
    \ForAll {$\si\{r[t] \gets a_i\} \in R_V new$}
    \State $\in_{new} \gets simpl(\in, \si)$
    \If {$\in_{new} \text{is val}$ }
    \State $U'\ \gets U - \{(s[t], \in)\}$
    \State $R'\ \gets R + \{(s[t], \in_{new}\}$
    \Else
    \State $U'\ \gets (U - \{(s[t], \in)\} + \{(s[t], \in_{new})\})$
    \EndIf
    \EndFor
  \end{algorithmic}
\end{algorithm}

\begin{definition}[Strict Simplification]
  \label{def:strict-simpl}
  Let us define a special simplification function which will not simplify anything until it has all the parameters of the stream expression and then evaluates it.
  %
  It meets both simplification properties, namely P1 and P2.
  %
  P1: is trivial
  %
  P2: the partial evaluation occurs only when $Y = X$ so $X\ \setminus Y is\ \EmptySet$
  %
  Then the partial application (with all the parameters) yields the same result as applying the function with all its parameters. 
\end{definition}

%\begin{definition}[Simplification function properties OVERRIDEN]
%  Substitution of variables $x\ \in\ X$ by values $a_i\ \in\ \si $\\
%  $Dom(\si) = Dom(f)\ \produce\ simpl(f(x_1, ..., x_n), \si) = f(x_1 \si,..., x_n\si )$ (P1)\\
%  If the value of simplifying the function $f$ with all its parameters results in the value $u$,\\
%  then for every partial application of f with the values in $Y \subseteq X$ -that is, with fewer parameters-  the resulting value is $u$\\
%  $simpl(f(x_1, ..., x_n), \si) = u\ \produce\ \A X \setminus Y\ .\ f(x_1, ..., x_n) . \si = u$ (P2)\\
%  Then if we feed all remaining parameters to this transformation it will yield the same result as the original expression applying all the parameters at once.
%\end{definition}


\newcounter{thm-correctness-c-d-eval}
\setcounter{thm-correctness-c-d-eval}{\value{theorem}}
\begin{theorem} [Correctness of decentralized and centralized with strict simplification]
\label{thm:correctness-cent-decent-eval}
The centralized and decentralized algorithms using the Strict Simplification~\ref{def:strict-simpl} yield the same outputs for any input.
%
Let $\form$ be a well defined specification and $I$ an input of size $N$.
%
Let $O_{cst}$ be the outputs of the centralized strict and $O_{dst}$ the outputs of the decentralized strict with the
topology $\topo$. Then $O_{cst} = O_{dst}$.
\end{theorem}

%\begin{proof}
%  Let $E$ be the evaluation graph of $\form$, let $I$ be the input and let $\rank$ be the evaluation distance of $E$.
%  %
%  We show by induction on $\rank(\subform[\tick])$ that $O_{cst}(\subform[\tick]) = O_{dst}(\subform[\tick])$
%  \textbf{Base case}$\rank(\subform[\tick]) = 0$\\
%  Let $\subform[\tick]\ =\ f\ (\subform[\tick-y|d],\ i_1[\tick-x_1|d],...,\ i_i[\tick-x_i|d],\ r_{1}[\tick-k_{1}|d_1],..., \ r_{j}[\tick-k_{j}|d_j])$ be the stream expression\\
%  And this expression is the same for the centralized and decentralized algorithms.
%  As $\rank(\subform[\tick]) = 0$ then $\rank(r_1) = ... = \rank(r_{j}[\tick-k_{j}|d_j]) = 0$\\
%  But $\subform[\tick]$ can only depend on subexpressions $r_1, ..., r_j$ such that \\
%  $r_{1}[\tick-k_{1} | d_1],..,\ r_{j}[\tick-k_{j} | d_j] < \subform[\tick]$ in the given well-founded order.\\
%  Thus, they are either inputs or streams whose all subexpressions are simplified to default values, to comply with the order.\\
%  Those that will be simplified are those that meet $t+k < 0\ or\ t+k > N$ 
%  Then $\ r_{1}[\tick-k_{1} | d_1],..., \ r_{j}[\tick-k_{j} | d_j] = d_1, ..., d_j$ By line 12\\
%  Note that V need not send messages to know the default values $d_1, ..., d_j$
%  
%  If an input:\\
%  if it will be resolved in a remote node, a request is sent by line 25\\
%  that request will arrive at its destination by Lemma~\ref{L4}\\
%  then it is processed and as it is an input at some time t' it will be resolved\\
%  then a response can be emitted with the value in R by line 20\\
%  then the response arrives at V with the pair $(i[\tick], c)$ by Lemma~\ref{L4}\\
%  so it is resolved in V\\
%  Alternatively, the input is received at some time in V.
%  
%  Either case :\\
%  $i_1[\tick-x_1],...,\ i_i[\tick-x_i]\ \in\ R_{v}[t"]$ with their respective values by line 10 or by Convergence (Theorem~\ref{thm:convergence})\\
%  So, by applying all its parameters, $\subform[\tick]$ is resolved in the decentralized strict version:
%  $(\subform[\tick], c)\ \in\ R_{V_d}[t"]$ By line 12\\
%  
%  On the other hand the centralized with strict algorithm will resolve $\subform[\tick]$ at instant $t'$
%  where $t' = max_i (t-x_i)$. At said moment both the default values $d_1, ..., d_j$ and the inputs $(i_1,c_1), ..., (i_i, c_i)$ are available to evaluate the expression of $\subform[\tick]$.
%  $(\subform[\tick], c)\ \in\ R_{V_d}[t"]$ By line 12\\
%  Because applying the same expression (function) over the same arguments yield the same result.\\
%  %
%  \textbf{IH :$\rank(r[\tick]) < \rank(\subform[\tick])$}  
%  Assuming that for $\rank(r[\tick]) < \rank(\subform[\tick])$ the value of $r[\tick]_{cst}$ is equal to $r[\tick]_{dst}$ for an arbitrary $t$\\
%  Prove $\subform[\tick]_{cst} = \subform[\tick]_{dst}$ assuming their subexpressions are resolved and equal for all $r$ s.t. $\rank(r[\tick]) < \rank(\subform[\tick])$\\
%  let $\subform[\tick]\ =\ f\ (\subform[\tick-y],\ i_1[\tick-x_1],...,\ i_i[\tick-x_i],\ r_{1}[\tick-k_{1} | d_1],..., \ r_{j}[\tick-k_{j} | d_j])$\\
%  And considering $x_{1..i}\ \in\ \Int$, $k_{1..j}\ \in\ \Int$, $y\ \in\ \Nat$,  $\rank(r_{1..j}) < \rank(\subform[\tick])$\\
%  all params are resolved to the same values as in the centralized strict algorithm by IH\\
%  So, $\subform[\tick]$ is resolved eventually in the future to a constant $c$ by Convergence (Theorem~\ref{thm:convergence})\\
%  $\subform[\tick]\ \in\ R_V[t^{IV}],\ t^{IV} = max(t", t''') = max (t", t + max_{i=1..i}(t-x_i))$
%  
%  On the other hand the centralized version will resolve it by evaluating the expression of $\subform[\tick]$ applying all its parameters, both inputs and subexpressions.  Thus,
%  $\subform[\tick]\ \in\ R_V$. As the inputs for the expression are equal to those of the decentralized version, and all the subexpressions with lesser $\rank$ are resolved to the same values in
%  both algorithms, we can conclude that the value of $\subform[\tick]$ obtained by the centralized strict and decentralized strict algorithms are equal for every $\subform[\tick]$.
%\end{proof}

\begin{definition}[Eval]
  \label{def:eval}
  $Eval :: Term (\EmptySet) \produce Const $ is given/fixed in each theory.
  Simply bottom eval of each function of the corresponding datatype see Section~\ref{datatypes}.
\end{definition}
\begin{definition}[Val substitution]
  \label{def:val-subs}
  $\subs$ Set of substitutions of the form $x \gets c$ where $c$ is a constant for some subset of the variables of the streams.
\end{definition}

\begin{definition}[Function simpl does not introduce variables]
  \label{def:simpl-variables}
  simpl is a function from a term to another term which does not add variables to the term so that the new term has less or the same variables as the original term.
  $simpl : Term \produce Term$
  $simpl(t) = t'$ where $Vars(t')\ \subseteq\ Vars(t)$
\end{definition}
\begin{definition}[Term equivalence]
  \label{def:term-eq}
  Let t and t' be two terms. We say that $t$ and $t'$ are ``equivalent under evaluation'', and we write $t \eqval t'$ See definition~\ref{def:eval}. 
  whenever
  $\A \subs\ .\ Vars(t) \Union Vars(t') \in \subs\ .\ Eval(t \subs) = Eval(t'\subs)$
\end{definition}

\begin{definition}[Admissible simplifiers]
  \label{def:good-simpl}
  %Overrides \ref{def:simpl}.
  We capture ``admissible'' simplifiers as follows:
  \begin{enumerate}
  \item Simpl does not add variables \ref{def:simpl-variables} 
  \item $t \eqval simpl(t)$ for every $\tick$ \ref{def:term-eq}
  \end{enumerate}
\end{definition}

\begin{fact}[Simplification preserves equivalence]
  \label{fact:simpl-eq}
%  \begin{equation}
%    \text{if $t \eqval t' $ then $t \eqval \simpl t' $}
%    \label{eq:Atwo}
  %  \end{equation}
  if $t \eqval t' $ then $t \eqval \simpl(t') $
    \label{eq:Atwo}
\end{fact}

\begin{note}
  \label{note:eq-properties}
  It is easy to show that $\eqval$ is reflexive, simmetric and transitive.
  Note that if $t \eqval t'$ then $t \eqval simpl\ t'$ by reflexivity $(t \eqval t)$
  and transitivity $t \eqval t'\ and\ t' \eqval simpl\ t'$ then $t \eqval simpl\ t'$ of $\eqval$
\end{note}
%
We are interested in showing that the chain of substitution followed by simplification preserves the equivalence (Lemma \ref{lem:simpl-distr} below).
%
We need first an auxiliary lemma.
%
\newcounter{lem-simpl-two}
\setcounter{lem-simpl-two}{\value{lemma}}
\begin{lemma}
  \label{lem:simpl-two}
  For every $t, \subs_1$ and $\subs_2$
  $t \subs_1 \subs_2 \eqval \simpl(\simpl(t\subs_1)\subs_2)$
\end{lemma}
%\begin{proof}
%  We first show that
%  \begin{equation}
%    \text{if $t \eqval t'$ then for every $\subs$ such that $t\subs \eqval t'\subs$}
%    \label{eq:sigma-eqval}
%  \end{equation}
%  Let $\subs_2$ be an arbitrary substitution from $Val(Vars(t\subs) \Union Vars(t'\subs))$.\\That is a substitution of the remaining variables after substituting $\subs$\\
%  then ($\subs\subs_2$) is a substitution from $Val(Vars(t) \Union Vars(t'))$, all variables present in $t$ or $t'$.\\
%  Since $t \eqval t'$, then\\
%  $Eval(t\subs\subs_2) = Eval (t'\subs\subs_2)$, or in other words\\
%  $Eval((t\subs)\subs_2) = Eval ((t'\subs)\subs_2)$ this implies $t\subs \eqval t'\subs$.
%  Hence, (\ref{eq:sigma-eqval}) holds.
%  
%  Now, first $t\subs_1 \eqval t\subs_1$ by reflexivity.\\
%  Then $t\subs_1 \eqval simpl\ t\subs_1$ by definition of admissible simplifiers\\
%  It follows that $t\subs_1\subs_2 \eqval (simpl t\subs_1)\subs_2.$\\
%  Then by Fact \ref{eq:Atwo} $t\subs_1\subs_2 \eqval\ simpl((simpl\ t\subs_1)\subs_2)$ as desired.
%\end{proof}

\newcounter{lem-simpl-distr}
\setcounter{lem-simpl-distr}{\value{lemma}}
\begin{lemma} [Simplification distributive property]
  \label{lem:simpl-distr}
  Let $t$ be a term,  let $\subs_0, ..., \subs_n$ be substitutions from $Val(Vars(t))$,
  Let $t_0, ...,t_n$ be defined as follows: $t_0 = t,\ t_{i+1} = simpl(t_i\subs_i)$
  then
  $t_n \eqval simpl(t\subs_1...\subs_n)$
  then 
  $t_n \eqval simpl(t\subs_0 ... \subs_{n-1})$
\end{lemma}
%\begin{proof}
%  We show by induction on $n$ that $t_n \eqval t\subs_0, ..., \subs_{n-1}$.\\
%  \textbf{IH:} $t_{n-1} \eqval t\subs_0, ..., \subs_{n-2}$\\
%  Now by ``simpl preserves equivalence'' (Lemma~\ref{eq:Atwo}) and by ``substitution to both members preserves equivalence'' (Lemma~\ref{eq:sigma-eqval}) then
%  $simpl (t_{n-1}\subs_{n-1}) \eqval t\subs_0, ..., \subs_{n-2}\subs_{n-1}$\\
%  Now $t_n = simpl(t_{n-1}\subs_{n-1})$ and by reflexivity $t_n \eqval simpl(t_{n-1}\subs_{n-1})$\\
%  Hence, $t_n \eqval t\subs_0, ..., \subs_{n-1}$ follows.
%  %
%  Now applying ``simpl preserves equivalence'' we obtain the desired result.
%\end{proof}

\newcounter{lem-subs-simpl-ground}
\setcounter{lem-subs-simpl-ground}{\value{lemma}}
\begin{lemma}Let $t[x_1,...,x_n]$ be a term, and simpl a simplifier.
  \label{lem:subs-simpl-ground}
  Let $\subs$ be a partial substitution of $X$ such that $simpl(t\subs) = c$. Then, for every $\subs_{rest}, simpl(t\subs\subs_{rest}) = c$
  In particular if $t\subs\subs_{rest}$ is ground, $Eval(t\subs\subs_{rest}) = c$
\end{lemma}
%\begin{proof}
%  $t\subs \eqval simpl(t\subs) \eqval c$\\
%  Consequently,     $t\subs\subs_{rest} \eqval simpl(t\subs\subs_{rest}) \eqval c\subs_{rest}$, and $c\subs_{rest} \eqval c$\\
%  Finally, since $t\subs\subs_{rest}$ is ground $Eval(t\subs\subs_{rest}) = d$, which satisfies $d \eqval c$
%\end{proof}

\newcounter{thm-correctness-c-simpl-c-strict}
\setcounter{thm-correctness-c-simpl-c-strict}{\value{theorem}}
\begin{theorem}[Theorem correctness of centralized with simplification and centralized strict]
  \label{thm:correctness-cent-simpl-cent-strict}
  The centralized with evaluation and the centralized with simplification algorithms yield the same outputs for any input.
  Let $\form$ be a well defined specification and $I$ an input of size $N$. Let $O_{cst}$ be the outputs of the centralized strict and $O_{cs}$ the outputs of the centralized with simplification. Then $O_{cst} = O_{cs}$.
\end{theorem}

%\begin{proof}
%  Let $E$ be the evaluation graph of $\form$ and $I$ and let $\rank$ be evaluation distance of $E$. We show by induction on $\rank(\subform[\tick])$ that for all $O_{ce}(\subform[\tick]) = O_{cs}(\subform[\tick])$
%  \textbf{Base case}[$\rank = 0$]
%  let $\subform[\tick]\ =\ f\ (\subform[\tick-y|d],\ i_1[\tick-x_1|d],...,\ i_i[\tick-x_i|d],\ r_{1}[\tick-k_{1}|d_1],..., \ r_{j}[\tick-k_{j}|d_j])$ be the stream expression\\
%  And this expression is the same for both algorithms.\\
%  As $\rank(\subform[\tick]) = 0$ then $\rank(r_1) = ... = \rank(r_{j}[\tick-k_{j}|d_j]) = 0$\\
%  But $\subform[\tick]$ can only depend on subexpressions $r_1, ..., r_j$ such that \\
%  $r_{1}[\tick-k_{1} | d_1],..,\ r_{j}[\tick-k_{j} | d_j] < \subform[\tick]$ in the given well-founded order.\\
%  Thus, they are either inputs or streams whose all subexpressions are simplified to default values, to comply with the order.\\
%  Those that will be simplified are those that meet $t+k < 0\ or\ t+k > N$ \\
%  Then $\ r_{1}[\tick-k_{1} | d_1],..., \ r_{j}[\tick-k_{j} | d_j] = d_1, ..., d_j$ By line 12\\
%  Note that V need not send messages to know the default values $d_1, ..., d_j$\\
%  If an input it is received at some time in V.\\
%  $i_1[\tick-x_1],...,\ i_i[\tick-x_i]\ \in\ R_{v}[t"]$\\
%  As both inputs and the default values are resolved, so by applying all its parameters to its expression, $\subform[\tick]$ is resolved in the centralized with evaluation to a value $c$.\\
%  $(\subform[\tick], c)\ \in\ R_{V_d}[t"]$ By line 12\\
%  
%  But, at some time $t'''$ such that $t''' \leq t"$ the centralized with simplification simplifies the expression of $\subform[\tick]$ to its value $d$.\\
%  Then by lemma \ref{lem:subs-simpl-ground} we could substitute the remaining parameters $\subs_{rest}$ in the expression on $\subform[\tick]$ at $t'''$ and evaluate the expression, obtaining the same output $c$, thus we can conclude that $c = d$.
%  
%  \textbf{IH}
%  Assuming centralized with evaluation and centralized with simplification yield the same outputs for $\rank(r[\tick]) < \rank(\subform[\tick])$ for an arbitrary $\tick$\\
%  Prove $\subform[\tick]_{cs} = \subform[\tick]_{ce} $ assuming their subexpressions are resolved and equal for $\rank(r[\tick]) < \rank(\subform[\tick]$\\
%  let $\subform[\tick]\ =\ f\ (\subform[\tick-y],\ i_1[\tick-x_1],...,\ i_i[\tick-x_i],\ r_{1}[\tick-k_{1} | d_1],..., \ r_{j}[\tick-k_{j} | d_j])$\\
%  And considering $x_{1..i}\ \in\ \Int$, $k_{1..j}\ \in\ \Int$, $y\ \in\ \Nat$ and $\rank(r_{1..j}) < \rank(\subform[\tick])$\\
%  So, $\subform[\tick]$ is resolved eventually in the future to a constant $c$\\
%  $\subform[\tick]\ \in\ R_V[t^{IV}],\ t^{IV} = max(t", t''') = max (t", t + max_{i=1..i}(t-x_i))$\\
%  On the one hand the centralized version will resolve it by evaluating the expression of $\subform[\tick]$ applying all its parameters, both inputs and subexpressions. As follows :
%  $Eval(t, s1, ...,sn) = c$ where $s_1, ..., s_n$ are pairs of substitutions of the form $(stream, const)$
%  Thus, $\subform[\tick]\ \in\ R_V,$
%  
%  Nevertheless, the centralized with simplification algorithm may obtain the output of the expression in some time $t' \leq t$ by applying some of the parameters of the expression. As follows:
%  $simpl(t\subs) = d$.
%  Then by Lemma \ref{lem:subs-simpl-ground} we could substitute the remaining parameters $\subs_{rest}$ in the expression on $\subform[\tick]$ at $t'''$ and evaluate the expression, obtaining the same output $c$, thus we can conclude that $c = d$.
%  
%\end{proof}

\newcounter{thm-correctness-d-simpl-d-strict}
\setcounter{thm-correctness-d-simpl-d-strict}{\value{theorem}}
\begin{theorem}[Theorem correctness of decentralized with simplification and decentralized with strict]
  \label{thm:correctness-decent-simpl-decent-strict}
  The decentralized strict and the decentralized with simplification algorithms yield the same outputs for any input.
  Let $\form$ be a well defined specification and $I$ an input of size $N$ and let $\Tau$ be the topology for both algorithms. Let $O_{dst}$ be the outputs of the decentralized with evaluation and $O_{ds}$ the outputs of the decentralized with simplification. Then $O_{dst} = O_{ds}$.
\end{theorem}
%\begin{proof}
%  Let $E$ be the evaluation graph of $\form$ and $I$ and let $\rank$ be evaluation distance of $E$. We show by induction on $\rank(\subform[\tick])$ that $O_{ds}(\subform[\tick]) = O_{dst}(\subform[\tick])$\\
%  \textbf{Base case}[$\rank = 0$]
%  let $\subform[\tick]\ =\ f\ (\subform[\tick-y|d],\ i_1[\tick-x_1|d],...,\ i_i[\tick-x_i|d],\ r_{1}[\tick-k_{1}|d_1],..., \ r_{j}[\tick-k_{j}|d_j])$ be the stream expression\\
%  And this expression is the same for the decentralized with simplification and decentralized strict algorithms.\\
%  As $\rank(\subform[\tick]) = 0$ then $\rank(r_1) = ... = \rank(r_{j}[\tick-k_{j}|d_j]) = 0$\\
%  But $\subform[\tick]$ can only depend on subexpressions $r_1, ..., r_j$ such that \\
%  $r_{1}[\tick-k_{1} | d_1],..,\ r_{j}[\tick-k_{j} | d_j] < \subform[\tick]$ in the given well-founded order.\\
%  Thus, they are either inputs or streams whose all subexpressions are simplified to default values, to comply with the order.\\
%  Those that will be simplified are those that meet $t+k < 0\ or\ t+k > N$ \\
%  Then $\ r_{1}[\tick-k_{1} | d_1],..., \ r_{j}[\tick-k_{j} | d_j] = d_1, ..., d_j$ By line 12\\
%  Note that V need not send messages to know the default values $d_1, ..., d_j$\\
%  If an input it is resolved in V\\
%  if it will be resolved in a remote node then a request is sent by line 25\\
%  that request will arrive at its destination by     \ref{L4}\\
%  then it is processed and as it is an input at some time t' it will be resolved\\
%  then a response can be emitted with the value in R by line 20\\
%  then the response arrives at V with the pair $(i[\tick], c)$\\
%  so it is resolved in V\\
%  Alternatively, the input is received at some time in V.\\
%  Either case :\\
%  $i_1[\tick-x_1],...,\ i_i[\tick-x_i]\ \in\ R_{v}[t"]$ by line 10\\
%  If it is resolved to default values $\subform[\tick]$ is resolved, so by applying all its parameters, $\subform[\tick]$ is resolved in decentralized with evaluation as follows
%  $Eval(t\subs) = c$ where $\subs$ are pairs of substitutions of the form $(stream, const)$
%  Then $(\subform[\tick], c)\ \in\ R_{V_d}[t"]$ By line 12\\
%  
%  Nevertheless, the decentralized with simplification algorithm may obtain the output of the expression in some time $t' \leq t$ by applying some of the parameters of the expression.
%  As follows: $simpl(t\subs) = d$.
%  Then by lemma \ref{lem:subs-simpl-ground} we could substitute the remaining parameters $\subs_{rest}$ in the expression on $\subform[\tick]$ at $t'''$ and evaluate the expression, obtaining the same output $c$, thus we can conclude that $c = d$.
%  
%  \textbf{IH :$\rank(r[\tick]) < \rank(\subform[\tick])$}
%  Prove $\subform[\tick]_d = \subform[\tick]_c $ assuming their subexpressions are resolved and equal for $\rank(r[\tick]) < \rank(\subform[\tick]$\\
%  let $\subform[\tick]\ =\ f\ (\subform[\tick-y],\ i_1[\tick-x_1],...,\ i_i[\tick-x_i],\ r_{1}[\tick-k_{1} | d_1],..., \ r_{j}[\tick-k_{j} | d_j])$\\
%  And considering $x_{1..i}\ \in\ \Int$, $k_{1..j}\ \in\ \Int$, $y\ \in\ \Nat$, $\rank(r_{1..j}) < \rank(\subform[\tick])$
%  $r_{1..j}$ will be resolved eventually to the same values that in the decentralized with simplification by IH\\
%  So, $\subform[\tick]$ is resolved eventually in the future to a constant $c$ by applying all its parameters.\\
%  $\subform[\tick]\ \in\ R_V[t^{IV}],\ t^{IV} = max(t", t''')$ % = max (t", t + max_{i=1..i}(t-x_i))$????\\ 
%  
%  On the other hand the decentralized with simplification version will resolve it by evaluating the expression of $\subform[\tick]$ applying some its parameters but will yield the same result by Lemma~\ref{lem:subs-simpl-ground}.\\
%  Thus, $\subform[\tick]\ \in\ R_V$. Considering that the needed inputs for the expression are equal as those of the decentralized version with evaluation, and all the needed subexpressions with lesser $\rank$ are resolved to the same values in both algorithms by IH. Then $simpl(t\subs) = d$ follows.
%  Then by lemma \ref{lem:subs-simpl-ground} we could substitute the remaining parameters $\subs_{rest}$ in the expression on $\subform[\tick]$ at $t'''$ and evaluate the expression, obtaining the same output $c$, thus we can conclude that $c = d$.
%\end{proof}

\newcounter{lem-oracle}
\setcounter{lem-oracle}{\value{lemma}}
\begin{lemma}[Oracle]
  \label{lem:oracle}
  Let there be an Oracle which injects the value of a stream in $R_V$ for a given node $V$.
  The value injected by the oracle is the same as the value that the algorithm would obtain applying the expression of the stream to all its parameters.
  Just as in the centralized Lola.
\end{lemma}
%\begin{proof}
%  By contradiction.\\
%  Suppose there is a stream for which the value guessed by the Oracle differs from that obtained by the system.\\
%  Given that all its substreams are well calculated and that the Oracle guesses the correct value of the stream.\\
%  Then, the only possibility is that the application of the stream expression with all its parameters performed by the algorithm was incorrect. This is a contradiction.
%\end{proof}


\newcounter{def-back-ref}
\setcounter{def-back-ref}{\value{definition}}
\begin{definition}[Back Reference Function]
  \label{def:back-ref}
  Let $bref : Stream \produce Nat$ be a function defined for every stream in the specification:  
  $bref(s)  = Max(0, Max({-w | r_i \xrightarrow{w} s} + dist(\delta(r_i), \delta(s))))$
\end{definition}

\newcounter{lem-back-ref}
\setcounter{lem-back-ref}{\value{lemma}}
\begin{lemma}[Back Reference (TTL)]
  \label{lem:back-ref}
  Let $s[t]$ be and instanced stream $s$ at time $\tick$, then
  there will be no Request message for $s[t]$ received at $\delta(s)$ after $t+bref(s)$
\end{lemma}
%\begin{proof}
%Let $r_i$, $s$ be streams s.t. $r_i \xrightarrow{w_i} s$ then\\
%  at $t_i' = t - w$ $r_i \in U_{\delta(r_i)}$ By Instantiation phase (line 19) and\\
%  at $t_i'' = t_i' + dist(\delta(r_i), \delta(s))$ a $Msg\{Req, s, \delta(r_i), \delta(s)\}$ arrives at $\delta(s)$ By lemma \ref{L4} and\\
%  at $t_{max} = Max(0, Max(t_i''))$ the last request message for $s$ arrives at $\delta(s)$.
%\end{proof}

\newcounter{cor-back-ref}
\setcounter{cor-back-ref}{\value{corollary}}
\begin{corollary}[R Pruning]
  \label{cor:r-prune}
  Let $n$ be a node  s.t. $n = \delta(s)$ and $s \in Lazy$ then n can remove $s[t]$ from its R in the pruning phase at $t + bref(s)$ or after.
\end{corollary}

%%% Local Variables:
%%% TeX-master: "main.tex"
%%% TeX-PDF-mode: t
%%% End:


==> preamble.tex <==
%for ieee
%\newcommand{\TheTitle}{Decentralized Stream Runtime Verification for Timed Asynchronous networks}
%\newcommand{\Thanks}{\thanks{This work was funded in part by FPU Grant
%    FPU18/04362 granted by the Spanish Ministry of Science, Innovation
%    and Universities. OTHER FUNDING}}
%\newcommand{\email}[1]{\textit{#1}}
%\title{\TheTitle}



\title{Decentralized Stream Runtime Verification for Timed Asynchronous Networks}
\author{\uppercase{Luis Miguel Danielsson}\authorrefmark{1,2} and \uppercase{C\'esar S\'anchez}\authorrefmark{2},\IEEEmembership{Senior, IEEE}}
\address[1]{Universidad Polit\'ecnica de Madrid, Madrid, Spain}
\address[2]{IMDEA Software Institute, Madrid, Spain email: {lm.danielsson@imdea.org} email:{cesar.sanchez@imdea.org}}
%\tfootnote{\Thanks}
%\footnotetext{\Thanks}
\markboth
{Author \headeretal: Preparation of Papers for IEEE TRANSACTIONS and JOURNALS}
{Author \headeretal: Preparation of Papers for IEEE TRANSACTIONS and JOURNALS}

%\corresp{*Luis Miguel Danielsson, IMDEA Software Institute. \email{lm.danielsson@imdea.org}}
%\corresp{Luis Miguel Danielsson, IMDEA Software Institute. email: lm.danielsson@imdea.org}

%\presentaddress{Present address}


==> quantitative.tex <==
\section{More Examples}
\label{sec:app:quantitative}

%\begin{example}
%  \label{ex:msgs}
%  %solution.tex
%  In this example we explain how the message sending happens with the topology of the network connecting monitors.
%  %
%  As we can see in Fig.~\ref{Re_msgs}, a message takes 1 cycle to
%  reach the next hop in the path from source to destination.
%  %
%  Therefore the distance between source and destination will be the time that a message needs to arrive from source to destination.
%  %
%\qed
%%
%  \begin{figure}
%    \centering
%  \includegraphics[scale=0.60]{RE_msgs}
%  \caption{Autosar example message sending}
%  \label{fig:RE_msgs}
%\end{figure}
%\end{example}
%
%\begin{example}
%  \label{ex:msgs}
%  %in solution.tex
%  In this example we describe the message passing of Request messages
%  (in red) and Response messages (in green) in
%  Fig.~\ref{fig:msgs-needed}.
%  %
%  The need of an instanced stream value arises from its presence in
%  the right side of an expression in U.
%  %
%  Therefore a needed value is one such that it is needed to simplify
%  that expression, whereas one that is not needed does not appear in
%  any expression in U.
%  %
%  Eval streams always send the Response message to those monitors that
%  compute streams that may need their values.
%  %
%  Lazy streams need to be requested in order to be sent, this way only
%  when it is actually needed a Request and matching Response will
%  traverse the network.
%  %
%\qed
%
%\begin{figure}
%  \begin{tabular}{cc}
%    \includegraphics[scale=1.00]{RE_eval} & 
%    \includegraphics[scale=1.00]{RE_lazy_needed}\\
%    \text{(a) Eval, all streams are needed} & 
%    \text{(b) Lazy, all streams are needed}\\
%    \includegraphics[scale=1.00]{RE_eval} & 
%    \includegraphics[scale=1.00]{RE_lazy_notneeded}\\
%    \text{(c) Eval, rarely the streams are needed} & 
%    \text{(d) Lazy, rarely the streams are needed}
%  \end{tabular}
%  \caption{Messages needed (lazy vs eval)}
%  \label{fig:msgs-needed}
%\end{figure}
%%
%\end{example}
%
%\begin{example}
%  \label{ex:simplification}
%  %solution.tex
%  In this example we explain how the simplifications of some expressions work.
%  \begin{tabular}{ccc}
%    & Expression & Simplified\\
%    a & if true then s[0] else t[1] & s[0]\\
%    b & if false then s[0] else t[1] & t[0]\\
%    c & 0 + 7 & 7\\
%    d & 1 * s[0] & s[0]\\
%    e & true or s[0] & true\\
%    f & false or s[0] & s[0]\\
%    g & false and s[0] & false\\
%    h & true and s[0] & s[0]\\
%      %a & \lolalang{if true then s[0] else t[1]} & \lolalang{s[0]}\\
%  \end{tabular}
%
%\qed
%%
%\end{example}

\begin{example}
  \label{ex:full-autosar}
  In this example we propose our solution to the problem of decentralized stream runtime verification in a car that uses the Autosar standard over the CAN network.
  %
  This example is inspired by the Electronic Stability Program (ESP) and models the under steering to the left scenario in an attempt to avoid an obstacle.
  %
  In such a case the ESP must detect the sudden turn of the steering wheel and the deviation produced with the actual movement of the car (yaw).
  %
  When this deviation is perceived and maintained over a period of time, the ESP must act on the brakes, the torque distribution and the engine in order produce the desired movement without any lose of control over the vehicle.
  %
  We define the following streams:
  %
  \begin{compactitem}
  \item $dir\_dev$ which represents the direction of the deviation between the yaw and the steering
  %
  \item $u\_st\_l$ represents the detection of an under steering to the left
  %
  \item $c\_u\_st\_l$ represent the duration of the under steering as a count.
  \end{compactitem}
  {\small\begin{lstlisting}[language=LOLA]
 
clique
@Chassis{
const num dir_tol = 0.2
input num yaw //real wheel direction 100, 100 in percentage
input num steering //driver desired direction 100, 100
input bool drive_wheel_slip 
input num b1 //brakes front left
input num b2 //brakes front right
input num b3 //brake rear left
input num b4 //brakes rear right
const num persistent_threshold = 25
define num dir_dev = steering - yaw //this way we know the direction of the dev

//steering left but car is not moving enough to the left, to avoid an obstacle
define bool u_st_l = dir_dev > 0 and dir_dev > dir_tol 
define num count_u_st_l = if u_st_l then count_u_st_l[-1|0] + 1 else 0
define bool persistent_u_st_l = count_u_st_l > persistent_threshold
define num effective_brake_l_rear = if persistent_u_st_l then count_u_st_l else 0

//other cases: under steering right, and over steering to both sides
output bool ESP_on = u_st_l or drive_wheel_slip //or other cases
//act on throttle
output num req_throttle = if ESP_on then req_throttle[-1|0] - dir_dev else 0
//act on torque distribution
output num req_torque_d = if ESP_on then req_torque_d[-1|0] - dir_dev else 0 
}

@Engine{
input num throttle 
const num throttle_tol = 0.1
output bool correct_throttle = req_throttle[-1|0]/throttle <= throttle_tol
}

@Transmission{
input num torque_d 
const num torque_d_tol = 0.1
output bool correct_torque_d = req_torque_d[-1|0]/torque_d <= torque_d_tol
}

@PowerTrainCoordinator{
output bool all_correct = correct_throttle and correct_torque_d
output bool always_correct = all_correct and always_correct[-1|true]
}

  \end{lstlisting}}

\qed
%

\end{example}


\begin{example}{Quantitative LTL semantics}
\label{quantitative-sem-ltl}
In this section we describe a quantitative semantics for LTL that preserves the commutative, associative, distributive, De Morgan laws and double negation.
This is the semantics for the most used operators:
\begin{compactitem}
\item $(\pi,i) \models Once\ \form = \form + \form[-1|0]$ iff $\exists j \leq i . (\pi,j) \models p \ne 0 $
\item $(\pi,i) \models Historically\ \form = \form * \form[-1|0]$ iff $\forall j \leq i . (\pi,j) \models p \ne 0 $
\item $(\pi,i) \models Previously strict\ \form = \form[-1|0]$ iff $i > 0 \And (\pi,j) \models p \ne 0 $
\item $(\pi,i) \models Previously\ \form = \form[-1|1]$ iff $i = 0 \Or (\pi,j) \models p \ne 0 $
\item $(\pi,i)\ \form \models \alpha Since \beta = \alpha + (\beta * \form[-1|1]$ iff $\exists j \leq i\ (\pi,j) \models \beta \ne 0$ and\\ $\forall k, j < k \leq i\ (pi,k) \models \alpha \ne 0$
\item $(\pi,i) \models InvCounter \form = if \form then 1 else 1 + InvCounter[-1|0]$
\item $(\pi,i) \models Once\ \form = 1/invCounter$
  \end{compactitem}
\end{example}

\begin{example}
  \label{ex:lola-two}
  Lets consider the previous example deployed in an isolated monitor that receives as an input the streams $i$ and $reset$.
  %
  Both streams are received at each corresponding cycle, so $i[0]$ and
  $reset[0]$ will be received at $n = 0$ and stored in Resolved and so on for all $n$.

  Starting at $\tick = 0$, the expression will be instantiated with the current value of $\tick$, replacing $\tick$ with its actual value in the expression, in this case $acc[0] = i[0] + root[0-1|0] = i[0] +
  root[-1|0]$. 
  %
  As $root[-1|0]$ is an invalid position in the stream $root$, then the default value for $root$ will be used, that is, $0$. 
  %
  So, the expression will simplify to $acc[0] = i[0] + 0 = i[0]$
  which is in R and has a certain value $c$. 
  %
  This value will be substituted in the expression for $acc[0]$. 
  %
  As it is now resolved, it will be moved from Unresolved to Resolved. 
  %
  The instantiation of $root$ is analogous: $root[0] = if\ reset[0]\ then\ 0\ else\ acc[0]$, lets consider that $reset[0] = False$ so $root[0] = acc[0]$ and as $acc[0]$ is already resolved, so
  $root[0] = c$ and it is moved to R.

  Then, at $\tick = 1$ the equation is instantiated again $acc[1] = i[1] + root[1-1|0] = i[1] + root[0]$.
  %
  This time, the required streams for the evaluation of $acc[1]$ are $i[1]$ and $root[0]$(which is a correct position of the stream $root$ because it is inside the trace limits $0 <= \tick < N$) and
  will be searched in Resolved.
  %
  If the value of the pair $(stream,time)$ is found in Resolved, then it is used to replace all references in every expression in Unresolved.
  %
  In this case the value of $root[0]$ will be used to substitute in the appropiate place in the expression resulting in $acc[1] = i[1] + c = e$.
  %
  As it is resolved it will be moved to Resolved. 
  %
  The instantiation of $root$ is the following: $root[1] = if\ reset[1]\ then\ 0\ else\ acc[1]$.
  %
  Lets consider this time that $reset[1] = True$, then the expression is resolved to $root[0] = 0$ and moved to R.
  %
  If the values of the needed timed streams were not found in Resolved, then the expression could not be simplified any further and would be left in Unresolved awaiting for a new tick in which the
  needed streams are in R (maybe coming from other nodes) so the expression can be simplified.
%
\qed
%
\end{example}

\begin{example}
  \phantomsection
  \label{ex:placement}
Lets continue with the same example, with the following placement: Monitor1 is assigned the stream $root$ and receives the input stream $reset$ while $acc$ will be computed by Monitor2 which also
receives the input stream $i$.
%
As Monitor1 needs the value of $acc$, it will send the message $req\{acc[t], Mon1, Mon2\}$ which can be read as "Monitor1 requests the value of $acc[t]$ at time $t$ to Monitor2".
%
Then at time $t+1$ Monitor2 receives this message and responds with the message $res\{acc[t] = c, Mon2, Mon1\}$ which analogously can be read as "Monitor2 responds $acc[t] = c$ to Monitor1".
%
At last, at time $t+2$ Monitor1 receives the message with the value of $acc[t] = c$, stores this value in R and proceeds to simplify the equation for $root[t]$.

Meanwhile at $t+1$ Monitor2 has the expression $acc[t+1] = i[t+1] + root[t]$ so it needs the value of $root[t]$ and will send the message $req\{root[t], Mon2, Mon1\}$ which arrives at Monitor 1 in
$t+2$.
%
At that time the value of $root[t]$ is already in R, so Monitor1 sends the message $res\{root[t]=c, Mon1, Mon2\}$ which in turn arrives at $t+3$ at Monitor2.
%
This value is stored in R and used to resolve the value of $acc[t+1]$. This process is repeated for all $t$ in the trace length.

This is an example of Lazy communication(see Section~\ref{lazy}) without any simplifier (see Section ~\ref{simplifiers}).
%
\qed
%
\end{example}

\begin{example}
  \label{ex:depend}
  %Let $\form~=~f(\subform)~\Or~g(\subform)$, and $\form$ is distributed in the following way: let $A~=~f(\subform)$ and $B~=~g(\subform)$ if $A$ is assigned to Monitor1 and $B$ is assigned to
  %Monitor2, and $\subform$ is assigned to Monitor3, then once Monitor3 resolves the value of $\subform$ it will communicate it to those nodes which require it, namely Monitor1 and Monitor2.  This is
  %possible because of $\depend~=~{\subform~\Impl~[Monitor1,~Monitor2]}$
  
  Lets consider Example 4 but using the Eval communication strategy (see Section~\ref{eval}).
  %
  Once Monitor2 resolves the value of $acc$ it will communicate it to those nodes which require it, namely Monitor1.
  %
  Analogously, Monitor1 will communicate the values of $root$ to Monitor1 as soon as they are resolved.
  %
  This is possible because of $\depend~=~\{acc~\Impl~[Monitor1], root~\Impl~[Monitor2]\}$.
%
\qed
%
\end{example}

\begin{example}
  \label{ex:eval}
%  Let $s[0] = r[0] + 1$ be a formula, and let $\deploy(s) = N1$ and $\deploy(r) = (N2, Eager)$, then as soon as $r_t$ for any $t$ is resolved and stored in $R$, a response message (without request)
  %will be sent to those nodes that require it, namely $N1$.

  Considering example 3 but with the Eval communication strategy, as soon as a Monitor2 resolves the value of $acc[t]$ the message $res{acc[t] = c, Monitor2, Monitor1}$ will be sent without the need
  of a request message.
%
  Analogously, as soon as Monitor1 resolves $root[t]$ the message $res\{root[t] = c, Monitor1, Monitor2\}$ will be sent.
%
\qed
%
\end{example}

\begin{example}
  \label{ex:lazy}
  %Let $\form_{t1} = a_{t2} \Impl b_{t3}$ where the root node emits the verdict and knows that $a_{t2} = \False$ because it has the pair $<a_{t2}, False>$ stored in $R$, given that $b_{t3}$ is computed
  %in another node, then by the use of a simplifier the node will know that $\form_{t1} = \True$ and there is no need to know the value of $b_{t3}$, nor to communicate it via network. This is an
  %example of a best case scenario.

  Considering the example 3, when we considered that $reset[t] = False$, in this case if we have a simplifier the expression $root[0] = if\ reset[0]\ then\ 0\ else\ acc[0]$ can be resolved to $root[0]
  = 0$.
%
Therefore there is no need to send a request message nor the corresponding response in order to get a value that is in fact not needed.
%
This is an example of a best case scenario.
%
\qed
%
\end{example}

%\begin{example}
% \label{ex:lazy2}
%  Let $\form[t] = true \lor \subform[t]$ be deployed at $N1$ amd $\subform[t]$ be deployed at $N2$, then the simplifier could simplify it to just $\form[t] = true$ and there will be no need to send
%  the request of $\subform$ and follow the whole protocol to get a value that is in fact not needed. However, if this situation arises using Eval for $\subform$, then $N2$ will compute $\subform$
%  which may require computation and messages sent. Then, as soon as the monitor obtains the subformula value, it will send a response message to $N1$ with the pair $,\subform_t, result.$, without
%  knowing that the computation and the message sent were useless, since the value is not really needed.
  %?regardless of whether the computations performed and messages sent were useful, resulting in a waste of resources in this case.
%\end{example}

\begin{example}
  \label{ex:hybrid}
  Considering our example the optimal way of configuring it is to treat the $root$ stream as Eval and the $acc$ stream as Lazy. 
%
This is due to the fact that $acc$ will always need the value of $root$ independetly of the inputs whereas the stream $root$ only needs $acc$ in some cases. 
%
\qed
%
\end{example}

\begin{example}
  \label{stream-req}
  Consider a trace of 100 elements and the specification of our example 1, if we want the monitors to compute the specification at each point in time, then we will request $root[0], ...,root[99]$.
%
Thus, the monitors will continue computing until they obtain all the values of $root[t]$ for every $t$. 
%
Depending on the trace and the specification itself, this situation may arise in a time before, at or after 99. 
%
This is how we could compute a specification at every point of a given trace.
%
\qed
%
\end{example}




==> solution-both.tex <==
\subsection{Problem description}
\subsubsection{Network.} 
Now we need these two msgs:
\begin{compactitem}
%REQUESTS ARE USED FOR LAZY ONLY, see LAZY section in efficient.tex
\item \textbf{Requests} messages: $(\REQ,s[k],n_s,n_d)$ where $s[k]$
  is an instant variable, $n_s$ is the source node and $n_d$ is the
  destination node of the message.
\item \textbf{Response} messages: $(\RESP,s[k],c,n_s,n_d)$ where
  $s[k]$ is an instant variable, $c$ is a value, $n_s$ is the source
  node and $n_d$ is the destination node.
\end{compactitem}
%
Let $\MSG=(\RESP,s[k],c,n_s,n_d)$, then $\MSG.\SRC=n_s$,
$\MSG.\DST=n_d$, $\MSG.\TYPE=\RESP$, $\MSG.\STREAM=s[k]$ and
$\MSG.\VAL=c$ (the analogous definitions apply for a request message
except that $\MSG.\VAL$ is not applicable).
%
\subsubsection{Stream Assignment and Communication Strategy}
Additionally, each stream variable $v$ can be assigned one of the
following two \emph{communication strategies} to denote whether an
instant value $v[k]$ is automatically communicated to all potentially
interested nodes, or whether its value is obtained on request only.
%
Let $v$ and $u$ be two stream variables such that $v$ appears in the
equation of $u$ and let $n_v=\mu(v)$ and $n_u=\mu(u)$.
\begin{compactitem}
\item \textbf{Eager communication}: the node $n_v$ informs $n_u$ of
  every value $v[k]=c$ that it resolves by sending a message
  $(\RESP,v[k],c,n_v,n_u)$.
\item \textbf{Lazy communication}: node $n_u$ requests $n_v$ the value
  of $v[k]$ (in case $n_u$ needs it to resolve $u[k']$ for some
  $k'$) by sending a message $(\REQ,v[k],n_u,n_v)$. When $n_u$ receives
  this message and resolves $v[k]$ to a value $c$, $n_u$ will respond
  with $(\RESP,v[k],c,n_v,n_u)$.
\end{compactitem}
%
Each stream variable can be independently declared as eager or lazy.
%
We use two predicates $\ISEAGER(u)$ and $\ISLAZY(u)$ (which is defined
as $\neg \ISEAGER(u)$) to indicate the communication strategy of
stream variable $u$.
%
Note that the lazy strategy involves two messages and eager only one,
but eager sends every instant variable resolved, while lazy will only
sends those that are requested.
%
In case the values are almost always needed, eager is preferable while
if values are less frequently required lazy is preferred.
%
We now need to add the communication strategy to the definition of the decentralized SRV problem.
%
\begin{definition}
  A decentralized SRV problem $\tupleof{\varphi,\topo,\mu, \ISEAGER}$
  is characterized by a specification $\varphi$, a topology $\topo$, a
  stream assignment $\mu$ and a communication strategy for every
  stream variable.
\end{definition}

\subsection{DSRV for Timed Asynchronous Networks: monitor and algorithm}
Our solution consists of a collection of local monitors, one for each
network node $n$.
%
A local monitor $\tupleof{\QUEUE_n, U_n, R_n, \PEN_n,\WAIT_n}$ for  $n$
consists of an input queue $\QUEUE_n$ and five storages:
\begin{compactitem}
\item \textbf{Resolved} storage $R_n$, where $n$ stores resolved
  instant variables $(v[k],c)$.
\item \textbf{Unresolved} storage $U_n$, where $n$ stores unresolved
  equations $v[k]=e$ where $e$ is not a value, but an expression that
  contains other instant variables.
\item \textbf{Pending} requests $\PEN_n$, where $n$ records instant
  variables that have been requested from $n$ by other monitors but that
  $n$ has not resolved yet.
\item \textbf{Waiting} for responses $\WAIT_n$, where $n$ records
  instant variables that $n$ has requested from other nodes but has
  received no response yet.
\end{compactitem}

When $n$ receives a response from remote nodes, the information is
added to $R_n$, so future local requests for the same value can be
resolved immediately.
%
The storage $\WAIT_n$ is used to prevent $n$ from requesting the same
value twice while waiting for the first request to be responded.
%
An entry in $\WAIT_n$ is removed when the value is received, since the
value will be subsequently fetched directly from $R_n$ and not
requested through the network.
%
The storage $\PEN_n$ is used to record that a value that $n$ is
responsible for has been requested, but $n$ does not know the answer
yet.
%
When $n$ computes the answer, then $n$ sends the corresponding response
message and removes the entry from $\PEN_n$.
%
Informally, in each cycle, the local monitor for $n$ processes the
incoming messages from its input queue $\QUEUE_n$.
%
Then $n$ reads the values for input streams assigned to it and also
instantiates for the current instant the output stream variables that
$n$ is responsible for.
%
After that, the equations obtained are simplified using the knowledge
acquired so far by $n$.
%
Finally, new response and request messages are generated and inserted
in the queues of the corresponding neighbors.

\AlgorithmTADLola

More concretely, every node $n$ will execute the procedure \Monitor\
shown in Algorithm~\ref{alg:local-algo}, which invokes \Step\ in every
clock tick until the input terminates.
%
The procedure \Finalize\ is used to resolve the pending values at the
end of the trace to their default.
%
The procedure \Step\ executes the following steps:
%
\begin{enumerate}
\item \textbf{Process Messages}: Lines $7$ invokes \ProcessMessages procedure
  in lines $23$-$28$ that deal with the processing of incoming messages.
%
%  First, Lines $13$-$14$ route messages with a different destination.
%
  Lines $26$ annotate requests in $\PEN_n$, which will be later
  resolved and responded.
  %
  Lines $27$-$28$ handle response arrivals, adding them to $R_n$ and
  removing them from $\WAIT_n$.
\item \textbf{Read Inputs and Instantiate Outputs:} Line $8$ reads new inputs
  for current time $k$, and line $9$ instantiates the equation of
  every output stream that $n$ is responsible for.
\item \textbf{Evaluate:} Line $10$ invokes the procedure \Evaluate, in lines $14-22$
  which evaluates the unresolved equations.
\item \textbf{Send Responses:} Line $11$ invokes \SendResponses, in lines $29$-$36$.
  First lines $30$-$32$ send messages for all newly resolved eager variables.
  %
  Lines $33$-$36$ deal with pending lazy variables.
  %
  If a pending instant variable is now resolved, the response message
  is sent and the entry is removed from $\PEN_n$.
\item \textbf{Send new Requests:} Lines $37$-$41$ send new request
  messages for all lazy instant streams that are now needed, to the
  corresponding responsible nodes.
\item \textbf{Prune:} Line $42$-$44$ prunes the set $R$ from information
  that is no longer needed. See section~\ref{sec:efficient}.
  %
\end{enumerate}

\subsection{Formal Correctness}
\label{subsec:correctness-complete}
\summary{formal proof of convergence and correctness}
We now show that our solution is correct by proving that the output
computed is the same as in the denotational semantics, and that every
output is eventually computed.

\newcounter{thm-convergence-complete}
\setcounter{thm-convergence-complete}{\value{theorem}}
\begin{theorem}
  \label{thm:convergence-complete}
  All of the following hold for every instant variable $u[k]$:
  \begin{compactenum}
    \item[\textup{(1)}] The value of $u[k]$ is eventually resolved.
    \item[\textup{(2)}] The value of $u[k]$ is $c$ if and only if $(u[k],c)\in R$ at
      some instant.
    \item[\textup{(3)}] If $\ISEAGER(u)$ then a response message for
      $u[k]$ is eventually sent.
    \item[\textup{(4)}] If $\ISLAZY(u)$ then all request messages for $u[k]$
      are eventually responded.

  \end{compactenum}
\end{theorem}
%
%%%% PROOF IN APPENDIX
\noindent The proof proceeds by induction in the evaluation graph, showing
simultaneously in the induction step $(1)$-$(4)$ as these depend on
each other (in the previous inductive steps).
\begin{proof}
  Let $M$ be a length of a computation and $\sigma_I$ be an input of
  length $M$.
%
  Note that $(1)$ to $(4)$ above are all statements about instant
  variables $u[k]$, which are the nodes of the evaluation graph
  $G_{\varphi,M}$.
%
  We proceed by induction on $G_{\varphi,M}$ (which is acyclic because
  $D_\varphi$ is well-formed).
%
  \begin{itemize}
  \item \textbf{Base case}: The base case are vertices of the
    evaluation graph that have no outgoing edges, which are either
    instant variables that correspond to inputs or to defined
    variables whose instant equation does not contain other instant
    variables.
    %
    Statement $(1)$ follows immediately for inputs because at instant
    $k$, $s[k]$ is read at node $\mu(k)$.
    % 
    For output equations that do not have variables, or whose
    variables have offsets that once instantiated become negative or
    greater than $M$, the value of its leafs is determined either
    immediately or at $M$ when the offset if calculated.
    %
    At this point, the value computed is inserted in $R$, so $(2)$
    also holds at $\mu(u)$.
    % 
    Note that $(2)$ also holds for other nodes because the response
    message contains $u[k]=c$ if and only if $(u[k],c)\in R_n$, where
    $\mu(u)=n$.
    %
    %If $s$ is eager,
    Then the response message is inserted exactly at
    the point it is resolved, so $(1)$ implies $(3)$.
    %
    Finally, $(4)$ also holds at the time of receiving the request
    message or resolving $u[k]$ (whatever happens later).
%
  \item \textbf{Inductive case}: Consider an arbitrary $u[k]$ in the
    evaluation graph $G_{\varphi,M}$ and let
    $u_1[k_1],\ldots,u_l[k_l]$ the instant variables that $u[k]$
    depends on.
    % 
    These are nodes in $G_{\varphi,M}$ that are lower than $u[k]$ so
    the inductive hypothesis applies, and $(1)$-$(3)$ hold for these.
    %
    Let $n=\mu(u)$.
    %
    At instant $k$, $u[k]$ is instantiated and inserted in $U_n$. 
    %
    At the end of cycle $k$, lazy variables among $u_1[l_1]\ldots
    u_l[ul]$ are requested.
    %
    By induction hypothesis, at some instant all these requests are
    responded by $(1)$.
    %
    Similarly, the values of all eager variables are calculated and
    sent as well (by $(1)$ and $(3)$).
    %
    At the latest time of arrival, the equation for $u[k]$ has no more
    variables and it is evaluated to a value, so $(1)$ holds and $(2)$
    holds at $n$.
    %
    At this point, if $\ISEAGER(u)$ then the response message is sent
    (so $(1)$ holds for $u[k]$) and if $\ISLAZY(u)$ then all requests
    (previously received in $\PEN_n$ or future requests) are answered,
    so $(1)$ also holds.
  \end{itemize}
%
  This finishes the proof.
\end{proof}


==> todo-no.tex <==
%\usepackage{todonotes}
\usepackage[disable]{todonotes}


==> todo-yes.tex <==
\usepackage{todonotes}
%\usepackage[disable]{todonotes}


==> uses.tex <==
\section{Uses} 
\label{sec:uses}
%do not tell my tool can be deployed
In this chapter we will present a motivating example based on industry standards for automotive. Namely, the CAN bus and the AUTOSAR framework.

\subsection{CAN Network}
The CAN network is implemented with a CAN bus which is a type of asynchronous BUS in the sense that computation nodes need not share the BUS clock internally. However, whenever a node wants to send a message, it is synchronized to the clock of the BUS. So, in the end a CAN BUS provide a synchronization mechanism that is shared across the network. Multiple computation nodes, usually ECUs, can be connected to the CAN BUS.
\paragraph{Versions}
In the standard ISO 11898-2 a high rate CAN bus is presented which can only have the topology of a BUS. Logically, this is equivalent as a clique topology because every node is directly connected to any other one. But, in the standard ISO 11898-3 a low-rate fault-tolerant CAN BUS is presented which admits either star or multiple stars connected by a central BUS topologies.

%\paragraph{Colission detection}
%In addition, the CAN BUS establishes a colission detection mechanism in the case of multiple nodes sending a message at the same time.
%Any message consist of the identifier of the sender node and the payload itself as the most important fields. Any number of nodes will try to put their messages in the BUS, but the bus performs and AND of the bits in the bus. So, a 0 has a higher precedence than a 1. Using this mechanism, the BUS effectively establishes a priority order among the messages. As the messages contain the identifier of the sender, engineers can adjust the priority of each sender using these identifiers, making their messages get through the network before messages of senders with lower priority. 
%\paragraph{Provides}Regarding the assumptions we made, the CAN network provides the following properties: Global clock \ref{ass:global-clock}, Multiple computation nodes \ref{ass:decent-obs} \ref{ass:monitors}, arbitrary topologies (Restricted in CAN) \ref{ass:routing-table}.

%\begin{itemize}
%\item Global clock \ref{ass:global-clock}\\
%\item Multiple computation nodes \ref{ass:decent-obs} \ref{ass:monitors}\\
%\item arbitrary topologies (Restricted in CAN) \ref{ass:routing-table}\\
%\end{itemize}

\subsection{AUTOSAR}
AUTOSAR is an industry standard framework for automotive applications and provides services such as scheduling or communication. The AUTOSAR framework is organized in several layers and can support different communication infrastructures such as CAN BUS, Lin or FlexRay. All these communication infrastructures are used in the automotive industry. -

%The AUTOSAR Runtime Environment provides the following properties: msgs of arbitrary size (contain lists)  (CAN TP, RTE can send arrays of variable number of elements) and routing determined statically at initialization \ref{ass:routing-table}
%\begin{itemize}
%\item msgs of arbitrary size (contain lists)  (CAN TP, RTE can send arrays of variable number of elements)\\
%\item routing determined statically at initialization \ref{ass:routing-table}\\
%\end{itemize}

\subsection{Assumptions of our solution}
We have identified the following assumptions:
\begin{itemize}
\item Global clock \ref{ass:global-clock}
\item Multiple computation nodes \ref{ass:decent-obs} \ref{ass:monitors}
\item Arbitrary topologies (Restricted in CAN) \ref{ass:routing-table}
\item Messages of arbitrary size (contain lists)  (CAN TP, RTE can send arrays of variable number of elements)
\item Static routing \ref{ass:routing-table}
\item Msgs are reliable and arrive in a tick
\item All nodes can send a bounded number of msgs in a tick
\end{itemize}
The first three properties are provided by the CAN network and the next two are provided by the AUTOSAR framework. In this setting we could build on top of these a service that could provide the last two properties. 

%Needed properties
%\begin{itemize}
%\item Msgs are reliable and arrive in a tick\\
%\item all nodes can send a bounded number of msgs in a tick\\
%\end{itemize}

Rewrite this saying that the assumptions we made are realistic enough.

%\includegraphics{figures/use_figure1}
%\includegraphics[scale=0.1]{figures/use_figure1}
%  \includegraphics[width=5cm]{figs/figure1}


